QUEST Eclipsing Binaries and ELLISA: Eclipsing binary search in the QUEST low latitude catalogue and the ELLISA light curve simulator

The realistic simulation of variable star populations is fundamental to determine the selection function and contamination in existing and upcoming multi-epoch surveys. We present \ellisa, a simulator that produces an ensemble of mock light curves for a population of eclipsing binaries obtained from physical and orbital parameters consistent with different galactic populations, and which considers user-supplied time sampling and photometric errors to represent any given survey. We carried out a search for eclipsing binaries in the QUEST low-galactic latitude catalogue of variable stars, spanning an area of 476 sq. deg at $-25^\circ \la b \la 30^\circ$ and $190^ \circ \leqslant l \leqslant 230^ \circ$ towards the galactic anti-centre, and use \ellisa~to characterise the completeness of the resulting catalogue in terms of amplitudes and periods of variation as well as eclipsing binary type. The resulting catalogue consists of $1,125$ eclipsing binaries, out of which $179$, $60$ and $886$ are EA, EB and EW types respectively. We estimate, on average, $30\%$ completeness in the period range $0.25 \la P/d \la 1$ for EB+EW binaries and $15\%$ completeness for EA binaries with periods $2 \la P/d \la 10$, being the time sampling the primary factor determining the completeness of each type of eclipsing binary. This is one of few eclipsing binary catalogues reported with an estimate of the selection function. Mock eclipsing binary light curve libraries produced with \ellisa~can be used to estimate the selection function and optimise eclipsing binary searches in upcoming multi-epoch surveys such as Gaia, the Panoramic Survey Telescope and Rapid Response System, the Zwicky Transient Factory or the Large Synoptic Survey Telescope.

==> light_curves_table.onlineonly.tex <==
\begin{tabular}{cccccccccccc}
\hline
ID & $\alpha$ & $\delta$ & ($N_V$,$N_R$,$N_I$) & Period & AmpV & AmpR & AmpI & Type & V & R & I\\
	& ($^{\circ}$) & ($^{\circ}$) &	& (d)	& (mag) & (mag) & (mag) &	& (mag) & (mag) & (mag) \\
\hline
40430964 & 73.3967 & 1.21155 & (23,24,26) & 0.36275 & 0.48 & 0.50 & 0.45 & ew & 16.52 $\pm$ 0.02 & 16.04 $\pm$ 0.01 & 15.66 $\pm$ 0.01 \\
40440270 & 73.5137 & 1.10068 & (26,25,26) & 0.62019 & 0.41 & 0.46 & 0.41 & eb & 14.85 $\pm$ 0.01 & 14.69 $\pm$ 0.00 & 14.52 $\pm$ 0.01 \\
40451647 & 73.6484 & 1.19106 & (19,25,25) & 0.26241 & 0.62 & 0.62 & 0.64 & ew & 17.52 $\pm$ 0.04 & 17.12 $\pm$ 0.01 & 16.76 $\pm$ 0.02 \\
40507509 & 74.3014 & 1.23649 & (24,25,27) & 0.43003 & 0.21 & 0.26 & 0.28 & ew & 16.56 $\pm$ 0.02 & 16.24 $\pm$ 0.01 & 15.95 $\pm$ 0.01 \\
40536826 & 74.6461 & 1.44519 & (20,24,21) & 0.31963 & 0.27 & 0.27 & 0.27 & ew & 17.03 $\pm$ 0.02 & 16.68 $\pm$ 0.01 & 16.35 $\pm$ 0.02 \\
40321878 & 71.8874 & 0.38869 & (20,5,0) & 0.55484 & 0.38 & 0.22 & 0.0 & ew & 14.31 $\pm$ 0.01 & 13.87 $\pm$ 0.00 & 0.0 $\pm$ 0.0 \\
40392956 & 72.8747 & 0.69226 & (19,11,21) & 0.26941 & 0.67 & 0.69 & 0.66 & ew & 17.71 $\pm$ 0.02 & 17.25 $\pm$ 0.01 & 16.79 $\pm$ 0.03 \\
40367482 & 72.5838 & -0.1034 & (33,25,23) & 0.28221 & 0.55 & 0.48 & 0.44 & ew & 16.31 $\pm$ 0.02 & 15.96 $\pm$ 0.01 & 15.62 $\pm$ 0.02 \\
40379942 & 72.7493 & -0.2977 & (15,12,17) & 2.00070 & 0.2 & 0.15 & 0.32 & ea & 16.42 $\pm$ 0.02 & 15.73 $\pm$ 0.01 & 15.18 $\pm$ 0.01 \\
40430447 & 73.3903 & -0.1010 & (31,23,20) & 0.30083 & 0.52 & 0.27 & 0.34 & ew & 18.13 $\pm$ 0.05 & 17.82 $\pm$ 0.04 & 17.62 $\pm$ 0.06 \\
40448224 & 73.6073 & 0.11906 & (0,18,16) & 0.22906 & 0.0 & 0.77 & 0.75 & ew & 0.0 $\pm$ 0.0 & 17.70 $\pm$ 0.03 & 17.10 $\pm$ 0.04 \\
40452311 & 73.6561 & -0.1555 & (35,23,21) & 1.02585 & 0.43 & 0.41 & 2.34 & ea & 17.34 $\pm$ 0.03 & 17.30 $\pm$ 0.03 & 17.30 $\pm$ 0.04 \\
40494852 & 74.1566 & 0.20654 & (23,14,13) & 0.36438 & 0.44 & 0.43 & 0.35 & ew & 16.60 $\pm$ 0.02 & 16.02 $\pm$ 0.01 & 15.64 $\pm$ 0.02 \\
40544320 & 74.7337 & -0.1355 & (28,24,23) & 0.32177 & 0.35 & 0.37 & 0.36 & ew & 16.78 $\pm$ 0.02 & 16.31 $\pm$ 0.02 & 15.89 $\pm$ 0.02 \\
40546984 & 74.7647 & 0.26690 & (13,9,10) & 0.28372 & 0.60 & 0.37 & 0.52 & ew & 16.36 $\pm$ 0.02 & 15.88 $\pm$ 0.01 & 15.46 $\pm$ 0.02 \\
50009152 & 75.1007 & 1.05505 & (20,24,21) & 0.41207 & 0.46 & 0.31 & 0.29 & ew & 15.82 $\pm$ 0.01 & 15.89 $\pm$ 0.01 & 15.75 $\pm$ 0.03 \\
50034168 & 75.3621 & 1.30209 & (26,23,24) & 0.35347 & 0.45 & 0.38 & 0.43 & ew & 16.25 $\pm$ 0.02 & 15.91 $\pm$ 0.01 & 15.59 $\pm$ 0.02 \\
50085350 & 75.8903 & 1.36489 & (16,18,22) & 0.20933 & 0.49 & 0.53 & 0.53 & ew & 18.66 $\pm$ 0.09 & 17.72 $\pm$ 0.03 & 17.05 $\pm$ 0.04 \\
50104299 & 76.0793 & 1.31239 & (26,20,21) & 0.92090 & 0.68 & 0.59 & 0.60 & ea & 17.02 $\pm$ 0.03 & 16.67 $\pm$ 0.02 & 16.38 $\pm$ 0.03 \\
50122594 & 76.2716 & 1.34513 & (28,23,23) & 0.22927 & 0.41 & 0.20 & 0.20 & ew & 15.94 $\pm$ 0.02 & 15.38 $\pm$ 0.01 & 15.02 $\pm$ 0.02 \\
50182919 & 76.9175 & 1.21323 & (26,27,27) & 0.74998 & 0.26 & 0.28 & 0.23 & ea & 15.50 $\pm$ 0.01 & 15.3 $\pm$ 0.01 & 15.12 $\pm$ 0.02 \\
50207034 & 77.1704 & 1.21934 & (43,25,46) & 0.33794 & 0.35 & 0.50 & 0.45 & ew & 17.12 $\pm$ 0.03 & 16.83 $\pm$ 0.02 & 16.21 $\pm$ 0.03 \\
50274583 & 77.8076 & 1.44248 & (29,15,0) & 0.63141 & 0.52 & 0.36 & 0.0 & ea & 16.71 $\pm$ 0.03 & 16.32 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50286491 & 77.9184 & 1.26471 & (56,25,47) & 0.57669 & 0.38 & 0.30 & 0.33 & eb & 15.25 $\pm$ 0.01 & 15.10 $\pm$ 0.01 & 14.93 $\pm$ 0.02 \\
50292673 & 77.9723 & 1.37036 & (39,20,0) & 0.30735 & 0.66 & 0.63 & 0.0 & ew & 18.21 $\pm$ 0.07 & 17.77 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
50309293 & 78.1179 & 1.04332 & (31,25,0) & 0.20645 & 0.45 & 0.32 & 0.0 & ea & 18.41 $\pm$ 0.08 & 18.09 $\pm$ 0.04 & 0.0 $\pm$ 0.0 \\
50356379 & 78.5482 & 1.31961 & (52,18,81) & 0.43845 & 0.39 & 0.26 & 0.36 & ew & 14.76 $\pm$ 0.01 & 14.24 $\pm$ 0.01 & 13.85 $\pm$ 0.02 \\
50382864 & 78.7867 & 1.16932 & (49,26,93) & 0.25924 & 0.33 & 0.18 & 0.39 & ew & 17.37 $\pm$ 0.04 & 16.74 $\pm$ 0.02 & 16.15 $\pm$ 0.03 \\
50392149 & 78.8680 & 1.25570 & (53,24,99) & 0.37125 & 0.24 & 0.22 & 0.35 & ew & 15.25 $\pm$ 0.01 & 14.81 $\pm$ 0.01 & 14.45 $\pm$ 0.02 \\
50427699 & 79.1881 & 1.26213 & (38,36,0) & 9.93552 & 0.54 & 0.52 & 0.0 & ew & 18.28 $\pm$ 0.07 & 17.82 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
50428744 & 79.1973 & 1.18625 & (0,43,59) & 1.04558 & 0.0 & 0.61 & 0.46 & ea & 0.0 $\pm$ 0.0 & 16.11 $\pm$ 0.01 & 15.82 $\pm$ 0.03 \\
50449876 & 79.3957 & 1.25477 & (23,47,87) & 0.25043 & 0.74 & 0.62 & 1.91 & ew & 18.74 $\pm$ 0.09 & 18.03 $\pm$ 0.04 & 17.63 $\pm$ 0.06 \\
50515851 & 80.0095 & 1.47764 & (39,39,60) & 0.26237 & 0.42 & 0.18 & 0.39 & ew & 17.02 $\pm$ 0.03 & 16.30 $\pm$ 0.01 & 15.53 $\pm$ 0.02 \\
50557720 & 80.3869 & 1.16904 & (55,52,124) & 0.31315 & 0.19 & 0.22 & 0.25 & ew & 15.73 $\pm$ 0.01 & 15.31 $\pm$ 0.01 & 14.94 $\pm$ 0.02 \\
50566490 & 80.4670 & 1.35626 & (58,55,118) & 0.54049 & 0.52 & 0.30 & 0.42 & ew & 16.10 $\pm$ 0.02 & 15.87 $\pm$ 0.01 & 15.61 $\pm$ 0.02 \\
50571345 & 80.5107 & 1.24244 & (51,53,127) & 0.32809 & 0.42 & 0.24 & 0.32 & ew & 17.40 $\pm$ 0.04 & 16.99 $\pm$ 0.02 & 16.62 $\pm$ 0.03 \\
50576340 & 80.5552 & 1.14432 & (2,36,114) & 0.65728 & 0.01 & 0.98 & 0.94 & ea & 19.76 $\pm$ 0.15 & 18.85 $\pm$ 0.07 & 17.58 $\pm$ 0.06 \\
50598499 & 80.7493 & 1.40037 & (50,45,104) & 0.04713 & 0.51 & 0.25 & 0.27 & ea & 17.63 $\pm$ 0.05 & 17.00 $\pm$ 0.02 & 16.38 $\pm$ 0.03 \\
50624681 & 80.9706 & 1.48941 & (13,26,0) & 0.26503 & 0.31 & 0.38 & 0.0 & ew & 19.15 $\pm$ 0.11 & 18.39 $\pm$ 0.05 & 0.0 $\pm$ 0.0 \\
50634198 & 81.0483 & 1.39875 & (47,40,0) & 0.20820 & 0.56 & 0.36 & 0.0 & ew & 18.24 $\pm$ 0.07 & 17.29 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
50641455 & 81.1071 & 1.42375 & (40,43,89) & 0.27210 & 0.69 & 0.82 & 0.76 & ew & 17.84 $\pm$ 0.06 & 17.35 $\pm$ 0.02 & 17.01 $\pm$ 0.04 \\
50747963 & 81.9680 & 1.02630 & (30,47,117) & 0.41397 & 0.24 & 0.39 & 0.50 & ew & 16.55 $\pm$ 0.02 & 16.02 $\pm$ 0.01 & 15.86 $\pm$ 0.03 \\
50775468 & 82.1883 & 1.33601 & (32,29,98) & 0.36841 & 0.25 & 0.71 & 0.35 & ew & 15.88 $\pm$ 0.02 & 15.35 $\pm$ 0.01 & 14.91 $\pm$ 0.02 \\
50812538 & 82.4938 & 1.03397 & (23,44,0) & 0.08673 & 0.48 & 0.33 & 0.0 & ea & 14.32 $\pm$ 0.01 & 13.97 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50814991 & 82.5151 & 1.34493 & (26,45,118) & 0.33311 & 0.38 & 0.35 & 0.34 & ew & 17.95 $\pm$ 0.06 & 17.62 $\pm$ 0.03 & 17.13 $\pm$ 0.04 \\
50839106 & 82.7165 & 1.31434 & (24,51,107) & 0.40117 & 0.33 & 0.49 & 0.43 & ew & 18.06 $\pm$ 0.07 & 17.91 $\pm$ 0.04 & 17.34 $\pm$ 0.05 \\
50847483 & 82.7867 & 0.96692 & (0,38,102) & 0.46822 & 0.0 & 0.33 & 0.48 & ew & 0.0 $\pm$ 0.0 & 14.68 $\pm$ 0.01 & 14.11 $\pm$ 0.02 \\
50876465 & 83.0322 & 1.06996 & (26,53,107) & 0.32780 & 0.73 & 0.71 & 0.91 & ew & 15.79 $\pm$ 0.01 & 15.25 $\pm$ 0.01 & 14.75 $\pm$ 0.02 \\
50879736 & 83.0609 & 1.12765 & (6,41,93) & 0.22775 & 0.46 & 0.77 & 1.19 & ew & 19.39 $\pm$ 0.13 & 18.28 $\pm$ 0.05 & 17.47 $\pm$ 0.06 \\
50960726 & 83.7520 & 1.39177 & (15,37,81) & 0.33318 & 0.51 & 0.72 & 0.53 & ew & 18.65 $\pm$ 0.09 & 17.91 $\pm$ 0.04 & 17.46 $\pm$ 0.06 \\
51017040 & 84.2193 & 1.47695 & (22,29,53) & 0.35276 & 0.61 & 0.49 & 0.55 & ew & 17.09 $\pm$ 0.03 & 16.28 $\pm$ 0.01 & 15.87 $\pm$ 0.03 \\
51038050 & 84.3959 & 1.35742 & (15,26,88) & 0.39176 & 0.58 & 0.56 & 0.60 & ew & 18.15 $\pm$ 0.07 & 17.67 $\pm$ 0.03 & 17.16 $\pm$ 0.04 \\
51059196 & 84.5706 & 0.99350 & (8,14,85) & 0.42834 & 0.33 & 0.4 & 0.57 & ew & 17.86 $\pm$ 0.06 & 17.60 $\pm$ 0.03 & 16.81 $\pm$ 0.04 \\
51062290 & 84.5958 & 1.14174 & (21,24,92) & 0.22574 & 0.39 & 0.23 & 0.27 & ew & 18.16 $\pm$ 0.07 & 17.19 $\pm$ 0.02 & 16.43 $\pm$ 0.03 \\
51069538 & 84.6570 & 1.43906 & (21,23,66) & 0.42379 & 0.45 & 0.44 & 0.41 & ew & 16.15 $\pm$ 0.02 & 15.48 $\pm$ 0.01 & 14.83 $\pm$ 0.02 \\
51118146 & 85.0644 & 1.19038 & (20,23,80) & 0.55887 & 0.4 & 0.36 & 0.52 & ew & 17.44 $\pm$ 0.04 & 17.16 $\pm$ 0.02 & 16.90 $\pm$ 0.04 \\
51121206 & 85.0902 & 0.92738 & (0,15,67) & 0.19301 & 0.0 & 0.49 & 0.59 & ew & 0.0 $\pm$ 0.0 & 17.50 $\pm$ 0.03 & 16.82 $\pm$ 0.04 \\
51121235 & 85.0904 & 1.46939 & (21,23,50) & 0.26659 & 0.37 & 0.31 & 0.26 & ew & 16.80 $\pm$ 0.03 & 16.41 $\pm$ 0.01 & 15.78 $\pm$ 0.03 \\
51173465 & 85.5528 & 1.20459 & (21,21,64) & 0.26649 & 0.54 & 0.55 & 0.59 & ew & 16.92 $\pm$ 0.03 & 16.28 $\pm$ 0.01 & 15.73 $\pm$ 0.02 \\
51202001 & 85.7940 & 1.41953 & (12,25,60) & 0.23664 & 0.43 & 0.36 & 0.33 & ew & 18.50 $\pm$ 0.08 & 17.66 $\pm$ 0.03 & 17.07 $\pm$ 0.04 \\
51207122 & 85.8384 & 1.25810 & (25,24,77) & 0.54230 & 0.85 & 0.9 & 0.92 & ew & 15.67 $\pm$ 0.01 & 15.12 $\pm$ 0.01 & 14.62 $\pm$ 0.02 \\
51240102 & 86.1177 & 1.00150 & (12,16,62) & 0.49067 & 0.37 & 0.3 & 0.42 & ew & 16.89 $\pm$ 0.03 & 16.48 $\pm$ 0.01 & 16.36 $\pm$ 0.03 \\
51242452 & 86.1374 & 1.10341 & (26,26,62) & 0.55299 & 0.61 & 0.63 & 0.64 & ew & 15.74 $\pm$ 0.01 & 15.24 $\pm$ 0.01 & 14.74 $\pm$ 0.02 \\
51259955 & 86.2853 & 1.09864 & (25,25,56) & 0.43804 & 0.28 & 0.29 & 0.57 & ew & 15.03 $\pm$ 0.01 & 14.49 $\pm$ 0.01 & 14.01 $\pm$ 0.02 \\
51260907 & 86.2935 & 1.33281 & (26,21,55) & 0.30364 & 0.68 & 0.66 & 0.88 & ew & 15.21 $\pm$ 0.01 & 14.58 $\pm$ 0.01 & 13.95 $\pm$ 0.02 \\
51261471 & 86.2983 & 1.31221 & (3,19,48) & 0.53199 & 0.20 & 0.68 & 0.69 & ea & 19.32 $\pm$ 0.12 & 18.37 $\pm$ 0.05 & 17.39 $\pm$ 0.05 \\
51264421 & 86.3234 & 1.42840 & (19,19,43) & 0.36808 & 0.37 & 0.28 & 0.51 & ew & 17.02 $\pm$ 0.03 & 16.14 $\pm$ 0.01 & 15.52 $\pm$ 0.02 \\
51337163 & 86.9628 & 1.03958 & (8,22,42) & 0.27668 & 0.34 & 0.30 & 0.38 & ew & 19.02 $\pm$ 0.11 & 17.84 $\pm$ 0.03 & 16.79 $\pm$ 0.03 \\
51382182 & 87.3288 & 1.12144 & (11,22,40) & 0.32965 & 0.68 & 0.37 & 0.41 & ew & 18.40 $\pm$ 0.08 & 17.47 $\pm$ 0.03 & 16.78 $\pm$ 0.03 \\
51471204 & 88.0096 & 1.25829 & (23,17,18) & 0.34374 & 0.54 & 1.11 & 0.47 & ew & 15.22 $\pm$ 0.01 & 14.59 $\pm$ 0.01 & 13.89 $\pm$ 0.02 \\
51494267 & 88.1935 & 1.02860 & (22,22,0) & 0.86054 & 0.42 & 0.55 & 0.0 & ea & 16.2 $\pm$ 0.02 & 15.54 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51560357 & 88.7187 & 1.19401 & (16,23,24) & 0.16679 & 0.52 & 0.59 & 0.56 & ea & 18.15 $\pm$ 0.07 & 17.03 $\pm$ 0.02 & 15.39 $\pm$ 0.02 \\
51616583 & 89.2040 & 1.00725 & (12,13,21) & 0.31365 & 0.41 & 0.32 & 0.40 & ew & 17.65 $\pm$ 0.05 & 16.99 $\pm$ 0.02 & 16.24 $\pm$ 0.03 \\
51714505 & 89.8523 & 1.28579 & (12,20,21) & 0.27421 & 0.89 & 0.66 & 0.76 & ew & 18.64 $\pm$ 0.09 & 17.59 $\pm$ 0.03 & 16.48 $\pm$ 0.03 \\
50079404 & 75.8340 & 0.35163 & (15,19,19) & 0.54460 & 0.42 & 0.32 & 0.35 & ew & 17.92 $\pm$ 0.04 & 18.07 $\pm$ 0.04 & 17.87 $\pm$ 0.07 \\
50091440 & 75.9537 & 0.48042 & (17,18,20) & 0.31705 & 0.61 & 0.93 & 0.59 & ew & 15.13 $\pm$ 0.01 & 14.79 $\pm$ 0.01 & 14.41 $\pm$ 0.02 \\
50097045 & 76.0097 & 0.66442 & (17,19,22) & 0.26560 & 0.60 & 0.56 & 0.55 & ew & 17.09 $\pm$ 0.02 & 16.64 $\pm$ 0.01 & 16.23 $\pm$ 0.02 \\
50336458 & 78.3785 & 0.79091 & (63,21,87) & 0.33454 & 0.42 & 0.45 & 0.48 & ew & 16.10 $\pm$ 0.01 & 15.51 $\pm$ 0.01 & 14.95 $\pm$ 0.02 \\
50430702 & 79.2277 & 0.39224 & (68,47,95) & 0.24035 & 0.90 & 0.87 & 0.83 & ew & 15.04 $\pm$ 0.01 & 14.54 $\pm$ 0.01 & 14.07 $\pm$ 0.02 \\
50480134 & 79.6920 & 0.83641 & (51,39,70) & 0.31049 & 0.84 & 0.72 & 0.75 & ew & 17.21 $\pm$ 0.03 & 16.78 $\pm$ 0.02 & 16.38 $\pm$ 0.03 \\
50490529 & 79.7905 & 0.41429 & (52,49,102) & 3.05266 & 0.27 & 0.25 & 0.47 & ea & 16.39 $\pm$ 0.02 & 16.05 $\pm$ 0.01 & 15.74 $\pm$ 0.02 \\
50505329 & 79.9269 & 0.34777 & (57,43,90) & 0.38486 & 0.61 & 0.55 & 0.82 & ew & 16.70 $\pm$ 0.02 & 16.34 $\pm$ 0.01 & 15.97 $\pm$ 0.02 \\
50529660 & 80.1504 & 0.53485 & (32,0,62) & 0.17806 & 0.56 & 0.0 & 0.53 & ew & 14.06 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 13.28 $\pm$ 0.02 \\
50620504 & 80.9532 & 0.80220 & (63,45,107) & 0.50492 & 0.49 & 0.42 & 0.8 & ew & 15.42 $\pm$ 0.01 & 15.05 $\pm$ 0.01 & 14.74 $\pm$ 0.02 \\
50643673 & 81.1420 & 0.77247 & (66,47,0) & 0.79506 & 0.70 & 0.33 & 0.0 & ew & 17.40 $\pm$ 0.03 & 16.23 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50656194 & 81.2428 & 0.42669 & (43,42,126) & 0.48731 & 0.48 & 0.38 & 0.39 & ew & 16.57 $\pm$ 0.02 & 16.11 $\pm$ 0.01 & 15.64 $\pm$ 0.02 \\
50666065 & 81.3251 & 0.63866 & (70,48,124) & 0.22086 & 0.22 & 0.22 & 0.22 & ew & 16.48 $\pm$ 0.02 & 15.96 $\pm$ 0.01 & 15.22 $\pm$ 0.02 \\
50707857 & 81.6711 & 0.83741 & (37,36,85) & 0.32759 & 0.45 & 0.48 & 0.43 & ew & 14.54 $\pm$ 0.01 & 14.15 $\pm$ 0.01 & 13.76 $\pm$ 0.02 \\
50737943 & 81.9094 & 0.38449 & (47,47,110) & 3.08496 & 0.39 & 0.28 & 0.24 & ew & 15.53 $\pm$ 0.01 & 14.80 $\pm$ 0.01 & 13.49 $\pm$ 0.02 \\
50765935 & 82.1312 & 0.80539 & (50,35,0) & 1.26327 & 0.43 & 0.43 & 0.0 & ew & 14.70 $\pm$ 0.01 & 13.88 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50815970 & 82.5466 & 0.67769 & (46,40,123) & 1.17342 & 0.81 & 0.75 & 0.84 & ea & 18.19 $\pm$ 0.05 & 17.77 $\pm$ 0.03 & 17.28 $\pm$ 0.05 \\
50829485 & 82.6600 & 0.61037 & (50,44,127) & 0.35452 & 0.26 & 0.32 & 0.38 & ew & 17.07 $\pm$ 0.02 & 16.60 $\pm$ 0.01 & 16.28 $\pm$ 0.03 \\
50842025 & 82.7655 & 0.43021 & (18,41,107) & 0.27968 & 0.53 & 0.44 & 0.43 & ew & 19.22 $\pm$ 0.09 & 18.08 $\pm$ 0.04 & 17.09 $\pm$ 0.04 \\
50860953 & 82.9249 & 0.49040 & (42,47,98) & 1.23314 & 0.48 & 0.44 & 0.46 & ew & 16.80 $\pm$ 0.02 & 16.48 $\pm$ 0.01 & 16.09 $\pm$ 0.02 \\
50863250 & 82.9445 & 0.82397 & (46,41,83) & 0.37269 & 0.27 & 0.31 & 0.33 & ew & 16.97 $\pm$ 0.02 & 16.64 $\pm$ 0.01 & 16.47 $\pm$ 0.03 \\
51019368 & 84.2709 & 0.74591 & (55,25,100) & 0.41481 & 0.47 & 0.47 & 0.81 & ew & 14.66 $\pm$ 0.01 & 14.43 $\pm$ 0.01 & 14.16 $\pm$ 0.02 \\
51073077 & 84.7208 & 0.61407 & (50,21,91) & 0.54208 & 0.32 & 0.28 & 0.36 & ew & 15.83 $\pm$ 0.01 & 15.36 $\pm$ 0.01 & 14.85 $\pm$ 0.02 \\
51077029 & 84.7551 & 0.65543 & (51,20,82) & 0.46476 & 0.32 & 0.25 & 0.28 & ew & 14.67 $\pm$ 0.01 & 14.26 $\pm$ 0.01 & 13.84 $\pm$ 0.02 \\
51090576 & 84.8656 & 0.87777 & (32,15,69) & 6.55593 & 0.54 & 0.51 & 0.53 & ea & 16.17 $\pm$ 0.02 & 15.53 $\pm$ 0.01 & 14.89 $\pm$ 0.02 \\
51105789 & 84.9954 & 0.80321 & (43,19,81) & 0.51306 & 0.48 & 0.16 & 0.27 & ew & 17.03 $\pm$ 0.02 & 16.77 $\pm$ 0.02 & 16.30 $\pm$ 0.03 \\
51125983 & 85.1690 & 0.53848 & (24,19,69) & 0.36613 & 0.37 & 0.34 & 0.37 & ew & 14.69 $\pm$ 0.01 & 14.2 $\pm$ 0.01 & 13.99 $\pm$ 0.02 \\
51127358 & 85.1814 & 0.32892 & (24,20,58) & 0.24513 & 0.68 & 0.58 & 0.72 & ew & 18.50 $\pm$ 0.06 & 17.85 $\pm$ 0.03 & 17.09 $\pm$ 0.04 \\
51155526 & 85.4334 & 0.52826 & (24,18,73) & 0.81525 & 0.40 & 0.30 & 0.25 & ew & 15.89 $\pm$ 0.01 & 15.55 $\pm$ 0.01 & 15.15 $\pm$ 0.02 \\
51217112 & 85.9638 & 0.47876 & (21,18,55) & 0.29431 & 0.61 & 0.60 & 0.65 & ew & 18.59 $\pm$ 0.06 & 18.00 $\pm$ 0.04 & 17.47 $\pm$ 0.05 \\
51219660 & 85.9869 & 0.88851 & (20,9,45) & 0.33854 & 0.77 & 0.62 & 0.82 & ew & 17.32 $\pm$ 0.03 & 16.79 $\pm$ 0.02 & 16.27 $\pm$ 0.03 \\
51410418 & 87.5909 & 0.39051 & (20,19,27) & 0.24968 & 0.37 & 0.25 & 0.30 & ew & 18.81 $\pm$ 0.07 & 17.51 $\pm$ 0.03 & 16.41 $\pm$ 0.03 \\
51430194 & 87.7429 & 0.60328 & (30,20,32) & 0.45668 & 0.21 & 0.18 & 0.21 & ew & 17.39 $\pm$ 0.03 & 16.96 $\pm$ 0.02 & 16.23 $\pm$ 0.02 \\
51440211 & 87.8195 & 0.45440 & (19,12,22) & 0.35948 & 0.24 & 0.21 & 0.25 & ew & 15.73 $\pm$ 0.01 & 14.93 $\pm$ 0.01 & 14.13 $\pm$ 0.02 \\
51451030 & 87.9037 & 0.66596 & (25,18,33) & 0.36015 & 0.27 & 0.26 & 0.26 & ew & 16.26 $\pm$ 0.02 & 15.66 $\pm$ 0.01 & 14.98 $\pm$ 0.02 \\
51494370 & 88.2505 & 0.43529 & (11,12,21) & 0.33671 & 0.21 & 0.18 & 0.23 & ew & 15.85 $\pm$ 0.01 & 15.04 $\pm$ 0.01 & 14.22 $\pm$ 0.02 \\
51497683 & 88.2771 & 0.82040 & (25,19,34) & 1.41798 & 0.31 & 0.32 & 0.31 & ea & 16.56 $\pm$ 0.02 & 15.81 $\pm$ 0.01 & 15.05 $\pm$ 0.02 \\
51684045 & 89.6566 & 0.36318 & (14,19,16) & 0.67007 & 0.43 & 0.47 & 0.36 & ew & 18.56 $\pm$ 0.06 & 17.84 $\pm$ 0.03 & 17.06 $\pm$ 0.04 \\
50061732 & 75.6504 & -0.0194 & (39,22,23) & 1.26323 & 1.02 & 0.8 & 0.86 & ea & 15.58 $\pm$ 0.01 & 15.38 $\pm$ 0.01 & 15.14 $\pm$ 0.02 \\
50283698 & 77.9037 & -0.1194 & (82,23,42) & 0.29090 & 0.42 & 0.40 & 0.38 & ew & 15.50 $\pm$ 0.01 & 15.22 $\pm$ 0.01 & 14.88 $\pm$ 0.02 \\
50310388 & 78.1413 & -0.2459 & (59,25,65) & 0.78669 & 0.28 & 0.28 & 0.38 & ew & 16.70 $\pm$ 0.02 & 16.5 $\pm$ 0.02 & 16.22 $\pm$ 0.02 \\
50322296 & 78.2524 & -0.2611 & (53,21,62) & 0.30358 & 0.78 & 0.30 & 0.39 & ew & 17.95 $\pm$ 0.06 & 17.82 $\pm$ 0.04 & 17.22 $\pm$ 0.05 \\
50324694 & 78.2744 & -0.1908 & (53,13,73) & 2.31837 & 0.67 & 0.27 & 0.21 & ew & 15.86 $\pm$ 0.02 & 15.07 $\pm$ 0.01 & 13.43 $\pm$ 0.02 \\
50330409 & 78.3274 & -0.0292 & (71,21,0) & 0.21070 & 0.76 & 0.79 & 0.0 & ea & 16.52 $\pm$ 0.02 & 16.16 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
50334073 & 78.3610 & 0.04899 & (85,22,70) & 0.32612 & 0.57 & 0.49 & 0.69 & ew & 16.49 $\pm$ 0.02 & 16.53 $\pm$ 0.02 & 15.85 $\pm$ 0.02 \\
50355158 & 78.5506 & -0.1190 & (77,23,69) & 2.36550 & 0.83 & 0.35 & 0.57 & ea & 17.84 $\pm$ 0.05 & 17.53 $\pm$ 0.03 & 17.15 $\pm$ 0.04 \\
50420666 & 79.1396 & -0.0098 & (129,53,74) & 0.81775 & 0.30 & 0.15 & 0.28 & ew & 15.99 $\pm$ 0.02 & 15.84 $\pm$ 0.01 & 15.61 $\pm$ 0.02 \\
50443729 & 79.3552 & 0.22752 & (48,32,45) & 0.45376 & 0.31 & 0.15 & 0.41 & ew & 16.32 $\pm$ 0.02 & 16.15 $\pm$ 0.02 & 16.02 $\pm$ 0.02 \\
50480790 & 79.7037 & 0.20591 & (63,23,46) & 0.62229 & 0.23 & 0.18 & 0.25 & ew & 16.00 $\pm$ 0.02 & 15.89 $\pm$ 0.01 & 15.75 $\pm$ 0.02 \\
50498753 & 79.8715 & 0.21624 & (63,26,44) & 0.36736 & 0.53 & 0.47 & 0.48 & ew & 16.61 $\pm$ 0.02 & 15.91 $\pm$ 0.01 & 15.92 $\pm$ 0.02 \\
50513325 & 80.0061 & -0.2178 & (78,48,81) & 3.44526 & 0.25 & 0.14 & 0.68 & ea & 17.74 $\pm$ 0.05 & 17.03 $\pm$ 0.02 & 16.46 $\pm$ 0.03 \\
50544388 & 80.2889 & 0.22404 & (57,26,66) & 0.28456 & 0.45 & 0.33 & 0.23 & ew & 14.87 $\pm$ 0.01 & 14.45 $\pm$ 0.01 & 13.99 $\pm$ 0.02 \\
50584049 & 80.6449 & -0.2394 & (42,71,64) & 0.23280 & 0.92 & 0.76 & 4.08 & ew & 19.09 $\pm$ 0.11 & 18.44 $\pm$ 0.06 & 18.04 $\pm$ 0.08 \\
50673060 & 81.3887 & -0.3737 & (50,56,26) & 0.28796 & 0.68 & 0.48 & 0.39 & ew & 18.34 $\pm$ 0.07 & 17.77 $\pm$ 0.04 & 17.33 $\pm$ 0.05 \\
50676364 & 81.4155 & 0.16131 & (92,0,86) & 0.69032 & 1.51 & 0.0 & 0.57 & ew & 17.70 $\pm$ 0.05 & 0.0 $\pm$ 0.0 & 17.16 $\pm$ 0.04 \\
50683023 & 81.4710 & 0.10805 & (103,68,0) & 0.34021 & 0.94 & 1.29 & 0.0 & eb & 18.04 $\pm$ 0.06 & 17.39 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
50727050 & 81.8284 & -0.3491 & (58,58,71) & 0.30334 & 0.84 & 0.44 & 0.45 & ew & 17.07 $\pm$ 0.03 & 16.77 $\pm$ 0.02 & 16.42 $\pm$ 0.03 \\
50756757 & 82.0631 & -0.0806 & (114,84,143) & 0.39778 & 0.49 & 0.52 & 0.5 & ew & 15.91 $\pm$ 0.02 & 15.56 $\pm$ 0.01 & 15.18 $\pm$ 0.02 \\
50757340 & 82.0678 & 0.09310 & (114,59,119) & 0.29263 & 0.32 & 0.15 & 0.26 & ew & 14.69 $\pm$ 0.01 & 14.17 $\pm$ 0.01 & 13.65 $\pm$ 0.02 \\
50780658 & 82.2562 & -0.3036 & (34,37,46) & 0.23934 & 0.69 & 0.98 & 0.93 & ew & 18.42 $\pm$ 0.07 & 17.38 $\pm$ 0.03 & 16.59 $\pm$ 0.03 \\
50795523 & 82.3797 & 0.00649 & (117,82,136) & 0.23281 & 0.33 & 0.39 & 0.40 & ew & 17.08 $\pm$ 0.03 & 16.57 $\pm$ 0.02 & 16.00 $\pm$ 0.02 \\
50818266 & 82.5716 & 0.18022 & (63,39,97) & 0.22359 & 0.39 & 0.28 & 0.31 & ew & 17.69 $\pm$ 0.05 & 16.93 $\pm$ 0.02 & 16.20 $\pm$ 0.02 \\
50826518 & 82.6414 & -0.0794 & (61,61,138) & 0.24529 & 0.64 & 0.57 & 0.60 & ew & 18.08 $\pm$ 0.06 & 17.75 $\pm$ 0.04 & 17.34 $\pm$ 0.05 \\
50833701 & 82.7006 & -0.2538 & (59,69,95) & 0.29088 & 1.13 & 0.87 & 0.80 & ew & 18.10 $\pm$ 0.06 & 17.63 $\pm$ 0.04 & 17.09 $\pm$ 0.04 \\
50848129 & 82.8222 & 0.01436 & (0,43,75) & 0.25232 & 0.0 & 1.09 & 0.64 & ew & 0.0 $\pm$ 0.0 & 18.38 $\pm$ 0.06 & 17.67 $\pm$ 0.07 \\
50888755 & 83.1723 & -0.2245 & (64,78,115) & 0.24308 & 0.16 & 0.29 & 0.67 & ew & 14.88 $\pm$ 0.01 & 14.38 $\pm$ 0.01 & 13.81 $\pm$ 0.02 \\
50889721 & 83.1808 & -0.3864 & (38,50,0) & 0.55089 & 0.27 & 0.48 & 0.0 & ew & 16.44 $\pm$ 0.02 & 15.99 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
50928290 & 83.5171 & 0.04270 & (112,87,121) & 0.39011 & 0.44 & 0.48 & 0.41 & eb & 17.14 $\pm$ 0.03 & 16.64 $\pm$ 0.02 & 16.05 $\pm$ 0.02 \\
50988311 & 84.0164 & -0.2356 & (76,71,90) & 1.62168 & 0.56 & 0.22 & 0.38 & ew & 15.94 $\pm$ 0.02 & 14.96 $\pm$ 0.01 & 13.84 $\pm$ 0.02 \\
51046225 & 84.5039 & 0.11369 & (82,45,99) & 0.38781 & 0.58 & 0.52 & 2.78 & ew & 17.94 $\pm$ 0.06 & 17.58 $\pm$ 0.03 & 17.22 $\pm$ 0.05 \\
51052067 & 84.5522 & -0.1524 & (94,63,0) & 14.1434 & 0.38 & 0.29 & 0.0 & ew & 16.02 $\pm$ 0.02 & 15.06 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51053661 & 84.5651 & -0.0561 & (108,57,0) & 9.49618 & 0.43 & 0.20 & 0.0 & ew & 15.03 $\pm$ 0.01 & 13.94 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51055174 & 84.5773 & -0.0665 & (64,51,76) & 9.93892 & 0.51 & 0.53 & 0.36 & ea & 16.73 $\pm$ 0.02 & 16.21 $\pm$ 0.02 & 15.56 $\pm$ 0.02 \\
51058771 & 84.6075 & -0.2638 & (62,43,86) & 0.37251 & 0.86 & 0.83 & 0.7 & eb & 18.40 $\pm$ 0.07 & 18.2 $\pm$ 0.05 & 17.81 $\pm$ 0.07 \\
51062956 & 84.6428 & 0.13942 & (70,25,93) & 0.25749 & 0.94 & 0.79 & 0.68 & ew & 17.70 $\pm$ 0.05 & 17.04 $\pm$ 0.02 & 16.26 $\pm$ 0.03 \\
51082306 & 84.8049 & -0.3455 & (48,38,48) & 0.38792 & 0.44 & 0.42 & 0.38 & ew & 17.58 $\pm$ 0.04 & 17.21 $\pm$ 0.03 & 16.82 $\pm$ 0.04 \\
51111613 & 85.0533 & -0.1689 & (72,53,84) & 0.28116 & 0.85 & 0.95 & 1.16 & ew & 15.77 $\pm$ 0.02 & 15.20 $\pm$ 0.01 & 14.58 $\pm$ 0.02 \\
51121835 & 85.1407 & 0.03056 & (81,56,105) & 4.9217 & 0.54 & 0.41 & 0.40 & ew & 18.45 $\pm$ 0.07 & 17.28 $\pm$ 0.03 & 15.32 $\pm$ 0.02 \\
51164830 & 85.5268 & -0.2175 & (51,51,76) & 3.76931 & 0.56 & 0.51 & 0.55 & ea & 16.67 $\pm$ 0.02 & 16.27 $\pm$ 0.02 & 15.79 $\pm$ 0.02 \\
51196677 & 85.7984 & -0.2112 & (52,52,74) & 0.31437 & 0.89 & 0.86 & 1.56 & ew & 17.53 $\pm$ 0.04 & 16.87 $\pm$ 0.02 & 16.20 $\pm$ 0.02 \\
51201203 & 85.8377 & -0.2905 & (42,43,74) & 2.12710 & 0.25 & 0.16 & 1.23 & ea & 17.66 $\pm$ 0.05 & 16.94 $\pm$ 0.02 & 16.36 $\pm$ 0.03 \\
51201286 & 85.8383 & 0.16269 & (29,21,60) & 0.29437 & 0.48 & 0.53 & 0.50 & ew & 18.98 $\pm$ 0.10 & 18.67 $\pm$ 0.07 & 17.85 $\pm$ 0.07 \\
51218147 & 85.9810 & -0.1832 & (34,41,68) & 4.01596 & 0.85 & 0.32 & 0.99 & ea & 18.82 $\pm$ 0.09 & 18.26 $\pm$ 0.06 & 17.65 $\pm$ 0.06 \\
51384454 & 87.4008 & -0.3330 & (25,40,0) & 0.31280 & 0.36 & 0.24 & 0.0 & ew & 16.49 $\pm$ 0.02 & 15.89 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51390224 & 87.4444 & -0.2128 & (29,43,49) & 11.8651 & 2.10 & 0.35 & 0.68 & ea & 16.30 $\pm$ 0.02 & 15.39 $\pm$ 0.01 & 14.55 $\pm$ 0.02 \\
51395714 & 87.4854 & -0.3091 & (17,42,37) & 0.28988 & 0.50 & 0.50 & 0.47 & ew & 17.41 $\pm$ 0.04 & 16.61 $\pm$ 0.02 & 15.74 $\pm$ 0.02 \\
51463995 & 88.0127 & -0.2561 & (31,48,46) & 0.26397 & 0.21 & 0.21 & 0.54 & ew & 16.59 $\pm$ 0.02 & 15.99 $\pm$ 0.02 & 14.98 $\pm$ 0.02 \\
51508185 & 88.3688 & 0.08144 & (36,28,53) & 0.33010 & 0.88 & 0.69 & 0.64 & ew & 18.15 $\pm$ 0.06 & 17.31 $\pm$ 0.03 & 16.38 $\pm$ 0.03 \\
51514187 & 88.4164 & 0.16317 & (33,11,32) & 0.58808 & 0.62 & 0.37 & 0.35 & ew & 18.24 $\pm$ 0.07 & 17.53 $\pm$ 0.03 & 16.89 $\pm$ 0.04 \\
51526365 & 88.5142 & -0.2411 & (25,27,47) & 0.99256 & 0.65 & 0.45 & 1.21 & ew & 17.51 $\pm$ 0.04 & 17.06 $\pm$ 0.02 & 16.58 $\pm$ 0.03 \\
51537167 & 88.6027 & -0.2166 & (16,0,40) & 1.94564 & 1.39 & 0.0 & 0.44 & ea & 17.07 $\pm$ 0.03 & 0.0 $\pm$ 0.0 & 15.52 $\pm$ 0.02 \\
51558377 & 88.7717 & -0.0586 & (39,28,47) & 0.32434 & 0.62 & 0.43 & 0.44 & ew & 17.49 $\pm$ 0.04 & 16.80 $\pm$ 0.02 & 16.08 $\pm$ 0.02 \\
51589474 & 89.0089 & 0.22665 & (35,12,25) & 0.47504 & 0.58 & 0.57 & 0.48 & ew & 17.29 $\pm$ 0.04 & 16.68 $\pm$ 0.02 & 15.95 $\pm$ 0.02 \\
51601335 & 89.0987 & -0.1014 & (29,23,45) & 2.07525 & 0.52 & 0.49 & 0.48 & ea & 15.62 $\pm$ 0.01 & 15.30 $\pm$ 0.01 & 14.83 $\pm$ 0.02 \\
51719466 & 89.8908 & 0.18493 & (34,11,19) & 0.33332 & 0.37 & 0.31 & 0.28 & ew & 14.65 $\pm$ 0.01 & 13.96 $\pm$ 0.01 & 13.49 $\pm$ 0.02 \\
60040746 & 90.3370 & 1.23762 & (16,23,21) & 0.52630 & 0.22 & 0.24 & 0.17 & ew & 15.85 $\pm$ 0.01 & 15.08 $\pm$ 0.01 & 14.53 $\pm$ 0.01 \\
60086778 & 90.6875 & 1.27025 & (10,22,0) & 0.40429 & 0.23 & 0.30 & 0.0 & ew & 17.35 $\pm$ 0.01 & 16.72 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
60163631 & 91.2495 & 1.35438 & (0,21,11) & 0.29907 & 0.0 & 0.38 & 0.32 & ew & 0.0 $\pm$ 0.0 & 17.08 $\pm$ 0.01 & 16.75 $\pm$ 0.02 \\
60014948 & 90.1332 & 0.78874 & (24,16,22) & 1.54527 & 0.27 & 0.12 & 0.25 & ew & 18.70 $\pm$ 0.05 & 18.09 $\pm$ 0.02 & 17.46 $\pm$ 0.02 \\
60030021 & 90.2551 & 0.34106 & (0,13,15) & 0.69705 & 0.0 & 0.28 & 0.30 & ew & 0.0 $\pm$ 0.0 & 19.19 $\pm$ 0.05 & 18.33 $\pm$ 0.04 \\
60045464 & 90.3729 & 0.50934 & (0,17,18) & 0.26076 & 0.0 & 0.73 & 0.68 & eb & 0.0 $\pm$ 0.0 & 18.45 $\pm$ 0.03 & 17.63 $\pm$ 0.03 \\
60084881 & 90.6732 & 0.80028 & (14,16,22) & 0.33973 & 0.31 & 0.34 & 0.69 & ew & 15.49 $\pm$ 0.02 & 14.61 $\pm$ 0.01 & 14.07 $\pm$ 0.01 \\
60104075 & 90.8170 & 0.38005 & (4,16,15) & 0.26682 & 0.21 & 0.38 & 0.56 & ew & 19.00 $\pm$ 0.06 & 18.33 $\pm$ 0.03 & 17.59 $\pm$ 0.03 \\
60136127 & 91.0494 & 0.73901 & (16,18,0) & 0.33851 & 0.31 & 0.28 & 0.0 & ew & 14.92 $\pm$ 0.03 & 14.40 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
60149072 & 91.1430 & 0.60206 & (15,18,14) & 0.25300 & 0.42 & 0.27 & 0.23 & ew & 18.42 $\pm$ 0.04 & 17.37 $\pm$ 0.01 & 16.5 $\pm$ 0.01 \\
60149784 & 91.1482 & 0.51487 & (8,19,13) & 0.53281 & 0.24 & 0.22 & 0.20 & ew & 16.26 $\pm$ 0.02 & 15.91 $\pm$ 0.01 & 15.46 $\pm$ 0.01 \\
60315084 & 92.3349 & 0.80855 & (0,19,12) & 0.27506 & 0.0 & 0.38 & 0.35 & ew & 0.0 $\pm$ 0.0 & 17.26 $\pm$ 0.01 & 16.55 $\pm$ 0.01 \\
60038923 & 90.3234 & 0.00796 & (37,15,0) & 0.36884 & 0.30 & 0.26 & 0.0 & ew & 17.72 $\pm$ 0.03 & 17.21 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80090435 & 121.139 & -0.2374 & (14,30,0) & 1.02099 & 0.64 & 0.67 & 0.0 & ea & 15.82 $\pm$ 0.01 & 15.50 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80151225 & 121.941 & -0.2886 & (19,32,0) & 0.37830 & 0.33 & 0.33 & 0.0 & ew & 16.89 $\pm$ 0.02 & 16.28 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80318882 & 124.385 & -0.4143 & (21,28,0) & 2.00126 & 0.43 & 0.42 & 0.0 & ew & 17.9 $\pm$ 0.04 & 17.64 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
80462097 & 126.817 & -0.1955 & (20,29,0) & 0.32715 & 0.48 & 0.47 & 0.0 & eb & 15.95 $\pm$ 0.01 & 15.51 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80562200 & 128.723 & -0.3592 & (22,31,0) & 0.31745 & 0.26 & 0.30 & 0.0 & ew & 15.64 $\pm$ 0.01 & 15.29 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80563452 & 128.748 & -0.0042 & (19,27,0) & 0.22656 & 0.76 & 0.83 & 0.0 & eb & 18.47 $\pm$ 0.06 & 17.76 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
80574709 & 128.974 & -0.1744 & (24,30,0) & 0.26524 & 0.47 & 0.38 & 0.0 & ew & 18.09 $\pm$ 0.04 & 17.63 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
80683482 & 131.307 & -0.2591 & (24,33,0) & 1.29114 & 1.37 & 0.46 & 0.0 & ew & 17.09 $\pm$ 0.02 & 16.97 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
80737637 & 132.621 & -0.0771 & (23,23,0) & 0.38783 & 0.31 & 0.24 & 0.0 & ew & 14.50 $\pm$ 0.01 & 14.09 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
40402872 & 73.0023 & 3.38271 & (14,19,8) & 0.36267 & 0.31 & 0.29 & 0.24 & ew & 16.79 $\pm$ 0.03 & 16.45 $\pm$ 0.01 & 16.34 $\pm$ 0.02 \\
40489784 & 74.0605 & 3.19718 & (20,12,25) & 0.26456 & 0.59 & 0.50 & 0.41 & ew & 17.63 $\pm$ 0.06 & 17.11 $\pm$ 0.02 & 16.22 $\pm$ 0.02 \\
40344206 & 72.2112 & 2.68232 & (18,20,11) & 0.37520 & 0.30 & 0.22 & 0.22 & ew & 16.82 $\pm$ 0.02 & 16.56 $\pm$ 0.01 & 16.41 $\pm$ 0.02 \\
40370918 & 72.5839 & 2.70197 & (21,25,11) & 0.47370 & 0.26 & 0.30 & 0.18 & ew & 15.75 $\pm$ 0.01 & 15.57 $\pm$ 0.01 & 15.30 $\pm$ 0.01 \\
40391814 & 72.8605 & 2.55094 & (17,24,9) & 0.32707 & 0.44 & 0.44 & 0.29 & ew & 17.71 $\pm$ 0.03 & 17.30 $\pm$ 0.02 & 16.80 $\pm$ 0.03 \\
40399642 & 72.9594 & 2.46405 & (20,20,9) & 0.61908 & 0.33 & 0.30 & 0.25 & ew & 15.00 $\pm$ 0.01 & 14.83 $\pm$ 0.01 & 14.80 $\pm$ 0.01 \\
40509333 & 74.2827 & 2.52446 & (30,28,23) & 0.27700 & 0.79 & 0.71 & 0.65 & ew & 16.57 $\pm$ 0.02 & 16.13 $\pm$ 0.01 & 15.61 $\pm$ 0.01 \\
40516110 & 74.3621 & 2.76515 & (30,28,28) & 0.27456 & 0.46 & 0.44 & 0.41 & ew & 18.34 $\pm$ 0.04 & 17.46 $\pm$ 0.02 & 16.73 $\pm$ 0.03 \\
40529087 & 74.5168 & 2.80532 & (30,26,27) & 0.23091 & 0.50 & 0.46 & 0.59 & ew & 18.43 $\pm$ 0.05 & 17.97 $\pm$ 0.04 & 17.23 $\pm$ 0.04 \\
40560950 & 74.8897 & 2.84968 & (20,26,25) & 0.34680 & 0.28 & 0.29 & 0.29 & ew & 16.86 $\pm$ 0.02 & 16.61 $\pm$ 0.01 & 16.28 $\pm$ 0.02 \\
40279847 & 71.2474 & 2.00222 & (48,23,14) & 0.33302 & 0.42 & 0.36 & 0.25 & ew & 15.55 $\pm$ 0.01 & 15.14 $\pm$ 0.01 & 14.64 $\pm$ 0.01 \\
40295540 & 71.4922 & 1.94554 & (46,24,15) & 0.35198 & 0.49 & 0.43 & 0.39 & ew & 17.33 $\pm$ 0.02 & 16.95 $\pm$ 0.01 & 16.55 $\pm$ 0.02 \\
40400407 & 72.9692 & 1.94483 & (45,33,16) & 2.28585 & 0.57 & 0.55 & 0.22 & ea & 15.78 $\pm$ 0.01 & 15.03 $\pm$ 0.01 & 14.21 $\pm$ 0.01 \\
40428207 & 73.3190 & 1.81286 & (34,34,30) & 0.34619 & 0.35 & 0.36 & 0.34 & ew & 16.68 $\pm$ 0.01 & 16.28 $\pm$ 0.01 & 15.82 $\pm$ 0.01 \\
40441101 & 73.4827 & 1.90929 & (44,46,29) & 0.24229 & 0.65 & 0.43 & 0.39 & ew & 18.02 $\pm$ 0.04 & 17.49 $\pm$ 0.02 & 16.89 $\pm$ 0.02 \\
40473866 & 73.8732 & 1.96774 & (48,0,8) & 0.32671 & 0.66 & 0.0 & 0.43 & ew & 13.70 $\pm$ 0.01 & 0.0 $\pm$ 0.0 & 13.08 $\pm$ 0.01 \\
40487622 & 74.0356 & 1.63777 & (25,27,10) & 0.39355 & 0.62 & 0.81 & 0.52 & ew & 16.71 $\pm$ 0.02 & 16.31 $\pm$ 0.01 & 15.84 $\pm$ 0.01 \\
40492182 & 74.0870 & 1.85216 & (50,32,0) & 0.26796 & 0.45 & 0.76 & 0.0 & ew & 17.74 $\pm$ 0.03 & 17.41 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
40497160 & 74.1439 & 1.56737 & (20,0,9) & 0.35847 & 0.46 & 0.0 & 0.42 & ew & 17.40 $\pm$ 0.03 & 0.0 $\pm$ 0.0 & 17.11 $\pm$ 0.03 \\
40516319 & 74.3647 & 1.97854 & (55,47,25) & 0.32600 & 0.48 & 0.47 & 0.41 & ew & 16.82 $\pm$ 0.02 & 16.44 $\pm$ 0.01 & 15.99 $\pm$ 0.01 \\
40538170 & 74.6218 & 2.03775 & (52,46,22) & 1.79369 & 0.24 & 0.25 & 0.13 & ew & 16.02 $\pm$ 0.01 & 14.94 $\pm$ 0.01 & 13.61 $\pm$ 0.01 \\
40543399 & 74.6830 & 2.01325 & (53,45,27) & 0.42386 & 1.08 & 0.67 & 1.05 & eb & 18.54 $\pm$ 0.07 & 17.94 $\pm$ 0.03 & 17.42 $\pm$ 0.04 \\
40562332 & 74.9061 & 1.81458 & (45,37,27) & 1.95616 & 0.36 & 0.33 & 0.34 & ea & 16.58 $\pm$ 0.01 & 16.50 $\pm$ 0.01 & 16.31 $\pm$ 0.02 \\
40566273 & 74.9523 & 2.23040 & (23,0,11) & 0.38583 & 0.52 & 0.0 & 0.47 & ew & 13.81 $\pm$ 0.01 & 0.0 $\pm$ 0.0 & 13.13 $\pm$ 0.01 \\
50001970 & 75.0220 & 3.07039 & (30,24,26) & 0.34006 & 0.49 & 0.39 & 0.36 & ew & 17.22 $\pm$ 0.04 & 16.60 $\pm$ 0.01 & 16.06 $\pm$ 0.02 \\
50019583 & 75.2123 & 3.01894 & (26,20,28) & 0.54692 & 0.41 & 0.33 & 0.42 & ew & 15.58 $\pm$ 0.01 & 15.44 $\pm$ 0.01 & 15.25 $\pm$ 0.01 \\
50030975 & 75.3317 & 3.34329 & (0,19,20) & 0.24515 & 0.0 & 0.52 & 0.53 & ew & 0.0 $\pm$ 0.0 & 17.94 $\pm$ 0.03 & 17.49 $\pm$ 0.05 \\
50074895 & 75.7866 & 3.03537 & (24,24,27) & 0.23399 & 0.56 & 0.45 & 0.37 & ew & 18.36 $\pm$ 0.08 & 17.53 $\pm$ 0.02 & 17.16 $\pm$ 0.04 \\
50108832 & 76.1290 & 3.09999 & (31,15,0) & 0.29669 & 0.61 & 0.51 & 0.0 & ew & 16.17 $\pm$ 0.02 & 15.67 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50126841 & 76.3222 & 3.38252 & (24,24,29) & 1.98794 & 0.54 & 0.59 & 0.55 & ea & 16.84 $\pm$ 0.03 & 16.26 $\pm$ 0.01 & 15.58 $\pm$ 0.02 \\
50294747 & 77.9964 & 3.34801 & (25,18,23) & 0.40155 & 0.48 & 0.40 & 0.44 & ew & 14.60 $\pm$ 0.01 & 14.14 $\pm$ 0.01 & 13.63 $\pm$ 0.01 \\
50407530 & 79.0142 & 3.35493 & (25,24,25) & 1.92633 & 0.73 & 0.79 & 0.71 & ea & 18.11 $\pm$ 0.07 & 17.49 $\pm$ 0.02 & 16.99 $\pm$ 0.04 \\
50421522 & 79.1423 & 2.94260 & (21,19,30) & 0.60265 & 0.42 & 0.29 & 0.47 & ew & 16.64 $\pm$ 0.03 & 16.16 $\pm$ 0.01 & 15.69 $\pm$ 0.02 \\
50473729 & 79.6313 & 3.17644 & (33,23,27) & 0.35386 & 0.34 & 0.27 & 0.59 & ew & 16.21 $\pm$ 0.02 & 15.90 $\pm$ 0.01 & 15.55 $\pm$ 0.02 \\
50487171 & 79.7585 & 3.03127 & (33,20,25) & 0.26771 & 0.3 & 0.20 & 0.21 & ew & 16.54 $\pm$ 0.02 & 16.30 $\pm$ 0.01 & 15.69 $\pm$ 0.02 \\
50491106 & 79.7959 & 3.32944 & (31,21,29) & 0.27748 & 0.41 & 0.33 & 0.36 & ew & 15.56 $\pm$ 0.01 & 15.19 $\pm$ 0.01 & 14.57 $\pm$ 0.01 \\
50493040 & 79.8130 & 2.93512 & (0,20,28) & 0.38654 & 0.0 & 0.21 & 0.23 & ew & 0.0 $\pm$ 0.0 & 15.57 $\pm$ 0.01 & 15.23 $\pm$ 0.01 \\
50510289 & 79.9732 & 3.30210 & (30,25,0) & 0.62033 & 0.30 & 0.30 & 0.0 & ew & 14.89 $\pm$ 0.01 & 14.73 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50563367 & 80.4553 & 3.31434 & (30,20,28) & 0.32137 & 0.50 & 0.34 & 0.39 & ew & 16.47 $\pm$ 0.02 & 16.29 $\pm$ 0.01 & 15.53 $\pm$ 0.02 \\
50613447 & 80.8942 & 3.22380 & (24,20,30) & 1.34611 & 1.05 & 1.00 & 0.93 & ea & 14.76 $\pm$ 0.01 & 14.55 $\pm$ 0.01 & 14.25 $\pm$ 0.01 \\
50617224 & 80.9265 & 3.11569 & (29,24,29) & 0.48999 & 0.33 & 0.34 & 0.32 & ew & 17.74 $\pm$ 0.06 & 17.22 $\pm$ 0.02 & 16.75 $\pm$ 0.03 \\
50664317 & 81.3106 & 3.09420 & (29,24,27) & 0.28164 & 0.58 & 0.52 & 0.64 & ew & 17.28 $\pm$ 0.04 & 16.92 $\pm$ 0.02 & 16.48 $\pm$ 0.03 \\
50673683 & 81.3886 & 3.01654 & (23,23,27) & 1.99692 & 0.23 & 0.71 & 0.60 & ea & 15.16 $\pm$ 0.01 & 14.55 $\pm$ 0.01 & 13.88 $\pm$ 0.01 \\
50763713 & 82.1134 & 3.10332 & (0,22,22) & 0.25404 & 0.0 & 0.63 & 0.63 & ew & 0.0 $\pm$ 0.0 & 18.12 $\pm$ 0.04 & 17.57 $\pm$ 0.05 \\
50904287 & 83.3021 & 3.48926 & (10,16,20) & 0.3454 & 0.24 & 0.17 & 0.24 & ew & 16.08 $\pm$ 0.02 & 15.69 $\pm$ 0.01 & 15.16 $\pm$ 0.01 \\
50908143 & 83.3357 & 3.35131 & (31,25,23) & 0.37549 & 0.50 & 0.46 & 0.42 & ew & 16.40 $\pm$ 0.02 & 16.02 $\pm$ 0.01 & 15.60 $\pm$ 0.02 \\
50918999 & 83.4303 & 3.02064 & (22,22,24) & 0.21059 & 0.23 & 0.22 & 0.22 & ew & 17.58 $\pm$ 0.05 & 16.85 $\pm$ 0.01 & 16.31 $\pm$ 0.02 \\
50924899 & 83.4818 & 3.17274 & (32,24,29) & 0.55331 & 0.62 & 0.34 & 0.56 & ew & 16.63 $\pm$ 0.03 & 16.38 $\pm$ 0.01 & 16.06 $\pm$ 0.02 \\
50001918 & 75.0213 & 2.73424 & (28,30,28) & 0.39597 & 0.23 & 0.21 & 0.20 & ew & 14.60 $\pm$ 0.01 & 14.42 $\pm$ 0.01 & 14.12 $\pm$ 0.01 \\
50002096 & 75.0233 & 2.76072 & (31,30,26) & 0.25787 & 0.85 & 0.76 & 0.64 & ew & 16.84 $\pm$ 0.02 & 16.27 $\pm$ 0.01 & 15.67 $\pm$ 0.01 \\
50023449 & 75.2536 & 2.50716 & (31,31,27) & 0.25727 & 0.29 & 0.26 & 0.25 & ew & 16.45 $\pm$ 0.01 & 15.92 $\pm$ 0.01 & 15.34 $\pm$ 0.01 \\
50085280 & 75.8929 & 2.69298 & (30,31,30) & 0.34734 & 0.65 & 0.65 & 0.66 & ew & 15.27 $\pm$ 0.01 & 14.96 $\pm$ 0.01 & 14.55 $\pm$ 0.01 \\
50167431 & 76.7629 & 2.86415 & (0,26,24) & 0.24829 & 0.0 & 0.23 & 0.21 & ew & 0.0 $\pm$ 0.0 & 15.16 $\pm$ 0.01 & 14.71 $\pm$ 0.01 \\
50170439 & 76.7955 & 2.73837 & (28,21,25) & 0.35154 & 0.44 & 0.45 & 0.48 & ew & 17.08 $\pm$ 0.02 & 16.83 $\pm$ 0.02 & 16.55 $\pm$ 0.03 \\
50208473 & 77.1926 & 2.34659 & (31,28,29) & 0.36719 & 0.64 & 0.39 & 0.42 & ew & 15.44 $\pm$ 0.01 & 15.15 $\pm$ 0.01 & 14.44 $\pm$ 0.01 \\
50344583 & 78.4499 & 2.72000 & (33,26,30) & 0.33166 & 0.71 & 0.67 & 0.75 & ew & 17.33 $\pm$ 0.02 & 16.96 $\pm$ 0.02 & 16.55 $\pm$ 0.03 \\
50429839 & 79.2198 & 2.38108 & (22,30,29) & 0.2737 & 0.54 & 0.49 & 0.53 & ea & 16.18 $\pm$ 0.01 & 16.11 $\pm$ 0.01 & 15.90 $\pm$ 0.02 \\
50431451 & 79.2348 & 2.86136 & (17,24,24) & 0.23865 & 0.47 & 0.37 & 0.33 & ew & 17.78 $\pm$ 0.03 & 17.20 $\pm$ 0.02 & 16.72 $\pm$ 0.03 \\
50472102 & 79.6157 & 2.58110 & (28,27,24) & 0.28632 & 0.61 & 0.45 & 0.43 & ew & 18.45 $\pm$ 0.05 & 18.37 $\pm$ 0.05 & 17.64 $\pm$ 0.06 \\
50500557 & 79.8832 & 2.68134 & (26,24,29) & 0.34646 & 0.54 & 0.50 & 0.57 & ew & 17.49 $\pm$ 0.03 & 17.23 $\pm$ 0.02 & 16.79 $\pm$ 0.03 \\
50517261 & 80.0367 & 2.76284 & (29,27,26) & 0.85298 & 0.88 & 0.83 & 0.65 & ea & 18.37 $\pm$ 0.05 & 18.1 $\pm$ 0.04 & 17.64 $\pm$ 0.06 \\
50544270 & 80.2823 & 2.77774 & (31,28,28) & 0.26412 & 0.36 & 0.23 & 0.31 & ew & 17.57 $\pm$ 0.03 & 17.05 $\pm$ 0.02 & 16.58 $\pm$ 0.03 \\
50563048 & 80.4525 & 2.44656 & (18,15,26) & 0.27322 & 0.60 & 0.69 & 0.84 & ew & 17.63 $\pm$ 0.03 & 17.08 $\pm$ 0.02 & 16.50 $\pm$ 0.02 \\
50601247 & 80.7892 & 2.61005 & (31,24,25) & 0.37609 & 0.46 & 0.36 & 0.44 & ew & 18.08 $\pm$ 0.04 & 17.56 $\pm$ 0.03 & 17.01 $\pm$ 0.04 \\
50638865 & 81.1031 & 2.64767 & (31,27,25) & 0.26721 & 0.44 & 0.45 & 0.37 & ew & 16.83 $\pm$ 0.02 & 16.47 $\pm$ 0.01 & 16.02 $\pm$ 0.02 \\
50729302 & 81.8410 & 2.59028 & (30,28,14) & 0.27340 & 0.82 & 0.76 & 0.67 & ew & 16.94 $\pm$ 0.02 & 16.47 $\pm$ 0.01 & 15.93 $\pm$ 0.02 \\
50762725 & 82.1055 & 2.65241 & (30,28,25) & 0.61516 & 0.67 & 0.90 & 0.64 & ea & 17.71 $\pm$ 0.03 & 17.55 $\pm$ 0.03 & 17.21 $\pm$ 0.04 \\
50764864 & 82.1227 & 2.50278 & (29,32,29) & 0.54361 & 0.34 & 0.33 & 0.29 & ew & 15.47 $\pm$ 0.01 & 15.37 $\pm$ 0.01 & 15.09 $\pm$ 0.01 \\
50769506 & 82.1606 & 2.61045 & (32,28,27) & 5.00102 & 0.41 & 0.44 & 0.46 & ea & 17.34 $\pm$ 0.02 & 17.03 $\pm$ 0.02 & 16.51 $\pm$ 0.02 \\
50820059 & 82.5809 & 2.67710 & (22,21,27) & 0.33118 & 0.35 & 0.41 & 0.41 & ew & 17.14 $\pm$ 0.02 & 16.93 $\pm$ 0.02 & 16.58 $\pm$ 0.03 \\
50830997 & 82.6729 & 2.56403 & (32,31,28) & 0.25834 & 0.46 & 0.43 & 0.41 & ew & 16.72 $\pm$ 0.01 & 16.29 $\pm$ 0.01 & 15.72 $\pm$ 0.01 \\
50842277 & 82.7673 & 2.74705 & (29,30,24) & 0.26461 & 0.63 & 0.56 & 0.43 & ew & 17.92 $\pm$ 0.04 & 17.14 $\pm$ 0.02 & 16.60 $\pm$ 0.03 \\
50896884 & 83.2375 & 2.49731 & (22,28,25) & 1.08586 & 0.31 & 0.26 & 0.17 & ew & 16.14 $\pm$ 0.01 & 15.30 $\pm$ 0.01 & 14.23 $\pm$ 0.01 \\
50963755 & 83.8056 & 2.47458 & (31,28,25) & 0.27831 & 0.35 & 0.34 & 0.39 & ew & 16.12 $\pm$ 0.01 & 15.81 $\pm$ 0.01 & 15.35 $\pm$ 0.01 \\
50977666 & 83.9200 & 2.47384 & (29,28,24) & 0.28052 & 0.48 & 0.49 & 0.41 & ew & 18.19 $\pm$ 0.04 & 17.79 $\pm$ 0.03 & 17.23 $\pm$ 0.04 \\
50982055 & 83.9573 & 2.31989 & (17,21,16) & 0.31742 & 0.52 & 0.43 & 0.49 & ew & 17.73 $\pm$ 0.03 & 17.41 $\pm$ 0.02 & 17.24 $\pm$ 0.04 \\
51010242 & 84.1946 & 2.78097 & (33,29,26) & 0.48121 & 0.83 & 0.79 & 0.82 & ea & 17.14 $\pm$ 0.02 & 16.82 $\pm$ 0.02 & 16.36 $\pm$ 0.02 \\
51037363 & 84.4230 & 2.48469 & (31,30,25) & 0.27289 & 0.65 & 0.54 & 0.54 & eb & 17.42 $\pm$ 0.02 & 16.94 $\pm$ 0.02 & 16.34 $\pm$ 0.02 \\
51054715 & 84.5667 & 2.73840 & (25,24,23) & 0.41048 & 0.47 & 0.52 & 0.59 & ew & 18.30 $\pm$ 0.05 & 18.12 $\pm$ 0.04 & 17.80 $\pm$ 0.07 \\
51057009 & 84.5854 & 2.69616 & (30,29,26) & 0.44212 & 0.68 & 0.44 & 0.46 & ew & 17.51 $\pm$ 0.03 & 17.25 $\pm$ 0.02 & 16.83 $\pm$ 0.03 \\
51075504 & 84.7416 & 2.61037 & (32,31,24) & 1.25733 & 0.47 & 0.42 & 0.37 & ea & 16.11 $\pm$ 0.01 & 15.50 $\pm$ 0.01 & 14.74 $\pm$ 0.01 \\
51111826 & 85.0475 & 2.43850 & (0,19,26) & 0.35800 & 0.0 & 1.65 & 0.62 & ea & 0.0 $\pm$ 0.0 & 15.61 $\pm$ 0.01 & 15.05 $\pm$ 0.01 \\
51142474 & 85.3157 & 2.45576 & (24,21,26) & 0.29996 & 0.60 & 0.55 & 0.50 & ew & 17.77 $\pm$ 0.03 & 17.22 $\pm$ 0.02 & 16.53 $\pm$ 0.02 \\
51186265 & 85.7029 & 2.38037 & (30,29,27) & 0.37308 & 0.33 & 0.33 & 0.30 & ew & 17.92 $\pm$ 0.04 & 17.50 $\pm$ 0.03 & 16.75 $\pm$ 0.03 \\
51219918 & 85.9890 & 2.52519 & (32,30,22) & 1.10577 & 0.46 & 0.44 & 0.42 & ea & 17.04 $\pm$ 0.02 & 16.79 $\pm$ 0.02 & 16.30 $\pm$ 0.02 \\
51271397 & 86.4312 & 2.64094 & (28,31,29) & 0.37926 & 0.24 & 0.25 & 0.20 & ew & 17.21 $\pm$ 0.02 & 16.38 $\pm$ 0.01 & 15.36 $\pm$ 0.01 \\
51277283 & 86.4836 & 2.66071 & (26,26,28) & 0.61916 & 0.26 & 0.26 & 0.25 & eb & 16.43 $\pm$ 0.01 & 16.10 $\pm$ 0.01 & 15.53 $\pm$ 0.01 \\
51343222 & 87.0639 & 2.67190 & (20,20,27) & 0.38899 & 0.46 & 0.36 & 0.43 & ew & 16.32 $\pm$ 0.01 & 15.67 $\pm$ 0.01 & 14.88 $\pm$ 0.01 \\
51377218 & 87.3381 & 2.71662 & (26,24,19) & 0.29853 & 0.32 & 0.35 & 0.46 & ew & 18.33 $\pm$ 0.05 & 17.68 $\pm$ 0.03 & 16.99 $\pm$ 0.03 \\
51389941 & 87.4350 & 2.74357 & (0,24,24) & 0.28463 & 0.0 & 0.25 & 0.41 & ea & 0.0 $\pm$ 0.0 & 13.93 $\pm$ 0.01 & 13.31 $\pm$ 0.01 \\
51400315 & 87.5132 & 2.78201 & (29,29,30) & 0.24458 & 0.57 & 0.52 & 0.49 & ew & 17.59 $\pm$ 0.03 & 16.94 $\pm$ 0.02 & 16.12 $\pm$ 0.02 \\
51448179 & 87.8811 & 2.42367 & (23,26,28) & 0.32214 & 0.35 & 0.33 & 0.30 & ew & 16.13 $\pm$ 0.01 & 15.31 $\pm$ 0.01 & 14.28 $\pm$ 0.01 \\
51496170 & 88.2651 & 2.78226 & (30,27,24) & 0.45666 & 0.29 & 0.24 & 0.25 & ew & 17.29 $\pm$ 0.02 & 16.14 $\pm$ 0.01 & 14.65 $\pm$ 0.01 \\
51588391 & 88.9926 & 2.70168 & (30,28,26) & 0.26680 & 0.45 & 0.38 & 0.33 & ew & 17.69 $\pm$ 0.03 & 16.68 $\pm$ 0.01 & 15.40 $\pm$ 0.01 \\
51616253 & 89.2016 & 2.81038 & (0,20,26) & 0.47059 & 0.0 & 0.29 & 0.27 & ew & 0.0 $\pm$ 0.0 & 15.52 $\pm$ 0.01 & 14.57 $\pm$ 0.01 \\
51702352 & 89.7741 & 2.41762 & (28,27,27) & 0.36504 & 0.58 & 0.38 & 0.54 & ew & 18.31 $\pm$ 0.05 & 17.84 $\pm$ 0.03 & 17.08 $\pm$ 0.04 \\
51705410 & 89.7942 & 2.87113 & (14,23,23) & 0.95472 & 0.29 & 0.57 & 0.37 & ea & 16.10 $\pm$ 0.01 & 15.25 $\pm$ 0.01 & 14.19 $\pm$ 0.01 \\
51724407 & 89.9153 & 2.43799 & (7,0,21) & 0.28776 & 0.51 & 0.0 & 0.44 & ea & 17.89 $\pm$ 0.03 & 0.0 $\pm$ 0.0 & 16.21 $\pm$ 0.02 \\
50051435 & 75.5408 & 1.56925 & (19,0,10) & 0.33245 & 0.37 & 0.0 & 0.50 & ew & 15.22 $\pm$ 0.01 & 0.0 $\pm$ 0.0 & 14.28 $\pm$ 0.01 \\
50158220 & 76.6616 & 1.59990 & (52,22,9) & 0.37686 & 0.39 & 0.32 & 0.24 & ew & 18.06 $\pm$ 0.05 & 17.79 $\pm$ 0.03 & 17.57 $\pm$ 0.06 \\
50188208 & 76.9821 & 1.67735 & (46,19,4) & 1.95659 & 0.58 & 0.21 & 0.19 & ea & 14.94 $\pm$ 0.01 & 14.65 $\pm$ 0.01 & 14.29 $\pm$ 0.01 \\
50217451 & 77.2834 & 1.66909 & (66,26,9) & 0.26853 & 0.75 & 0.65 & 0.54 & ew & 18.58 $\pm$ 0.08 & 18.27 $\pm$ 0.05 & 17.78 $\pm$ 0.07 \\
50239589 & 77.4986 & 1.62279 & (87,22,7) & 0.31293 & 0.64 & 0.50 & 0.46 & ew & 17.19 $\pm$ 0.03 & 16.82 $\pm$ 0.02 & 16.36 $\pm$ 0.02 \\
50266894 & 77.7429 & 1.57986 & (71,0,6) & 0.57148 & 0.78 & 0.0 & 0.37 & eb & 15.09 $\pm$ 0.01 & 0.0 $\pm$ 0.0 & 14.34 $\pm$ 0.01 \\
50295394 & 78.0016 & 1.95994 & (82,42,25) & 0.27413 & 1.19 & 0.86 & 0.98 & ew & 18.56 $\pm$ 0.08 & 18.03 $\pm$ 0.04 & 17.42 $\pm$ 0.05 \\
50339740 & 78.4073 & 1.82603 & (104,37,48) & 0.38384 & 0.88 & 0.87 & 0.61 & ea & 17.09 $\pm$ 0.03 & 16.53 $\pm$ 0.02 & 15.86 $\pm$ 0.02 \\
50435681 & 79.2740 & 2.24980 & (17,0,16) & 0.38572 & 0.49 & 0.0 & 0.43 & ew & 17.4 $\pm$ 0.03 & 0.0 $\pm$ 0.0 & 16.44 $\pm$ 0.02 \\
50457846 & 79.4831 & 2.18666 & (27,11,0) & 0.58613 & 0.56 & 0.38 & 0.0 & eb & 13.82 $\pm$ 0.01 & 13.89 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50484048 & 79.7289 & 1.67156 & (93,57,35) & 7.64886 & 0.49 & 0.45 & 0.42 & ew & 14.94 $\pm$ 0.01 & 14.63 $\pm$ 0.01 & 14.25 $\pm$ 0.01 \\
50545498 & 80.2933 & 1.63343 & (84,47,62) & 3.13879 & 0.30 & 0.26 & 0.29 & ea & 14.68 $\pm$ 0.01 & 14.49 $\pm$ 0.01 & 14.21 $\pm$ 0.01 \\
50565630 & 80.4760 & 1.91722 & (121,73,79) & 1.99514 & 0.35 & 0.36 & 0.21 & ew & 15.42 $\pm$ 0.01 & 14.51 $\pm$ 0.01 & 13.42 $\pm$ 0.01 \\
50569288 & 80.5088 & 1.82062 & (106,67,69) & 1.35162 & 0.48 & 0.47 & 0.44 & ea & 16.29 $\pm$ 0.02 & 15.71 $\pm$ 0.01 & 15.09 $\pm$ 0.01 \\
50583707 & 80.6370 & 2.00174 & (91,60,63) & 0.28797 & 1.97 & 0.60 & 0.62 & ew & 18.64 $\pm$ 0.08 & 18.07 $\pm$ 0.04 & 17.58 $\pm$ 0.06 \\
50599532 & 80.7748 & 1.64757 & (81,46,66) & 2.07147 & 0.36 & 0.38 & 0.55 & ew & 17.23 $\pm$ 0.03 & 16.15 $\pm$ 0.01 & 14.54 $\pm$ 0.01 \\
50600809 & 80.7857 & 1.89242 & (117,70,74) & 0.27557 & 0.23 & 0.22 & 0.42 & ew & 14.07 $\pm$ 0.01 & 13.69 $\pm$ 0.01 & 13.30 $\pm$ 0.01 \\
50602623 & 80.8017 & 2.18559 & (27,21,0) & 1.91986 & 0.60 & 0.92 & 0.0 & ea & 16.91 $\pm$ 0.02 & 16.45 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
50607212 & 80.8411 & 1.97623 & (114,74,85) & 22.1616 & 0.36 & 0.29 & 0.13 & ew & 15.78 $\pm$ 0.01 & 14.84 $\pm$ 0.01 & 13.77 $\pm$ 0.01 \\
50611629 & 80.8787 & 1.85522 & (111,62,50) & 2.48000 & 0.48 & 0.37 & 0.36 & ew & 14.84 $\pm$ 0.01 & 14.04 $\pm$ 0.01 & 13.19 $\pm$ 0.01 \\
50627432 & 81.0095 & 1.88931 & (123,66,73) & 14.3693 & 0.51 & 0.21 & 0.17 & ew & 16.51 $\pm$ 0.02 & 15.49 $\pm$ 0.01 & 14.10 $\pm$ 0.01 \\
50650756 & 81.1990 & 1.60795 & (80,51,60) & 0.97408 & 0.35 & 0.33 & 0.33 & ew & 15.64 $\pm$ 0.01 & 14.70 $\pm$ 0.01 & 13.60 $\pm$ 0.01 \\
50650776 & 81.1992 & 1.91576 & (112,74,84) & 11.9457 & 0.38 & 0.31 & 0.24 & ew & 16.53 $\pm$ 0.02 & 15.52 $\pm$ 0.01 & 14.17 $\pm$ 0.01 \\
50674665 & 81.3965 & 1.72800 & (108,67,77) & 9.98433 & 0.90 & 0.32 & 0.37 & ew & 17.38 $\pm$ 0.03 & 16.34 $\pm$ 0.01 & 14.6 $\pm$ 0.01 \\
60016997 & 90.1506 & 3.06212 & (24,17,0) & 1.00562 & 0.20 & 0.28 & 0.0 & ea & 14.72 $\pm$ 0.01 & 14.25 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
60055689 & 90.4507 & 3.25969 & (0,21,21) & 0.31577 & 0.0 & 0.52 & 0.46 & ew & 0.0 $\pm$ 0.0 & 18.14 $\pm$ 0.03 & 17.36 $\pm$ 0.03 \\
60067115 & 90.5383 & 3.18916 & (23,19,21) & 0.63306 & 0.57 & 0.55 & 0.54 & eb & 16.41 $\pm$ 0.02 & 15.93 $\pm$ 0.01 & 15.32 $\pm$ 0.01 \\
60108336 & 90.8491 & 3.47502 & (0,15,15) & 0.34461 & 0.0 & 0.31 & 0.30 & ew & 0.0 $\pm$ 0.0 & 16.44 $\pm$ 0.01 & 15.81 $\pm$ 0.01 \\
60122929 & 90.9556 & 3.43687 & (0,17,15) & 0.39478 & 0.0 & 0.4 & 0.42 & ew & 0.0 $\pm$ 0.0 & 17.13 $\pm$ 0.01 & 16.91 $\pm$ 0.02 \\
60125947 & 90.9776 & 3.35992 & (21,22,18) & 0.45069 & 0.19 & 0.26 & 0.20 & ea & 17.25 $\pm$ 0.03 & 16.76 $\pm$ 0.01 & 16.12 $\pm$ 0.01 \\
60140676 & 91.0821 & 3.31294 & (18,17,18) & 0.42413 & 0.32 & 0.26 & 0.26 & ew & 16.77 $\pm$ 0.02 & 16.33 $\pm$ 0.01 & 15.72 $\pm$ 0.01 \\
60141980 & 91.0912 & 3.04330 & (17,17,16) & 0.29966 & 0.44 & 0.20 & 0.27 & ew & 17.36 $\pm$ 0.03 & 16.87 $\pm$ 0.01 & 16.25 $\pm$ 0.01 \\
60170125 & 91.2970 & 3.00660 & (0,16,18) & 0.35536 & 0.0 & 0.37 & 0.36 & ew & 0.0 $\pm$ 0.0 & 14.92 $\pm$ 0.01 & 14.15 $\pm$ 0.01 \\
60198321 & 91.4935 & 3.18758 & (0,18,21) & 0.22044 & 0.0 & 0.49 & 0.39 & ew & 0.0 $\pm$ 0.0 & 18.08 $\pm$ 0.03 & 17.05 $\pm$ 0.02 \\
60239219 & 91.7774 & 3.02816 & (0,11,17) & 0.35990 & 0.0 & 0.21 & 0.25 & ew & 0.0 $\pm$ 0.0 & 16.17 $\pm$ 0.01 & 15.49 $\pm$ 0.01 \\
60256411 & 91.9039 & 3.38872 & (0,11,16) & 0.46948 & 0.0 & 0.21 & 0.22 & ew & 0.0 $\pm$ 0.0 & 15.16 $\pm$ 0.01 & 14.43 $\pm$ 0.01 \\
60066489 & 90.5334 & 2.59212 & (8,21,21) & 0.27957 & 0.40 & 0.42 & 0.34 & ew & 19.26 $\pm$ 0.07 & 18.51 $\pm$ 0.05 & 17.60 $\pm$ 0.05 \\
60085209 & 90.6758 & 2.60578 & (15,26,25) & 0.33191 & 0.60 & 0.66 & 0.71 & ew & 17.06 $\pm$ 0.02 & 16.51 $\pm$ 0.02 & 15.77 $\pm$ 0.02 \\
60184115 & 91.3959 & 2.77705 & (14,25,26) & 0.28060 & 0.36 & 0.33 & 0.32 & ew & 18.39 $\pm$ 0.04 & 17.74 $\pm$ 0.03 & 16.73 $\pm$ 0.03 \\
60199393 & 91.5010 & 2.35943 & (0,22,23) & 0.51922 & 0.0 & 0.20 & 0.27 & ew & 0.0 $\pm$ 0.0 & 16.56 $\pm$ 0.02 & 15.97 $\pm$ 0.02 \\
60205385 & 91.5415 & 2.59005 & (13,23,26) & 0.29903 & 0.36 & 0.36 & 0.33 & ew & 16.74 $\pm$ 0.02 & 16.07 $\pm$ 0.02 & 15.26 $\pm$ 0.02 \\
60208374 & 91.5614 & 2.7092 & (13,19,19) & 2.69334 & 0.45 & 0.45 & 0.46 & ea & 15.28 $\pm$ 0.02 & 14.76 $\pm$ 0.03 & 14.11 $\pm$ 0.02 \\
60247522 & 91.8371 & 2.75719 & (0,14,21) & 0.44978 & 0.0 & 0.25 & 0.27 & ew & 0.0 $\pm$ 0.0 & 16.90 $\pm$ 0.02 & 16.03 $\pm$ 0.02 \\
60011185 & 90.1015 & 1.92025 & (48,34,24) & 0.42394 & 0.61 & 0.56 & 0.45 & ew & 18.47 $\pm$ 0.05 & 17.85 $\pm$ 0.02 & 17.12 $\pm$ 0.02 \\
60039749 & 90.3296 & 1.71467 & (24,27,14) & 0.93261 & 0.41 & 0.60 & 0.63 & ea & 18.29 $\pm$ 0.04 & 17.85 $\pm$ 0.02 & 17.08 $\pm$ 0.02 \\
60042851 & 90.3526 & 1.59209 & (23,19,9) & 0.41589 & 0.26 & 0.21 & 0.19 & ew & 15.81 $\pm$ 0.02 & 15.14 $\pm$ 0.00 & 14.70 $\pm$ 0.01 \\
60043180 & 90.3553 & 2.04394 & (45,28,26) & 0.17691 & 0.12 & 0.28 & 0.22 & ea & 16.05 $\pm$ 0.02 & 15.49 $\pm$ 0.00 & 14.88 $\pm$ 0.01 \\
60056105 & 90.4540 & 1.85084 & (42,29,19) & 0.29621 & 0.50 & 0.26 & 0.27 & ew & 16.61 $\pm$ 0.02 & 16.09 $\pm$ 0.01 & 15.66 $\pm$ 0.01 \\
60070880 & 90.5672 & 2.04498 & (34,27,19) & 0.19346 & 0.28 & 0.34 & 0.31 & ew & 17.66 $\pm$ 0.03 & 16.79 $\pm$ 0.01 & 15.93 $\pm$ 0.01 \\
60096414 & 90.7601 & 1.98669 & (27,35,21) & 0.36306 & 0.73 & 0.93 & 0.64 & ew & 16.82 $\pm$ 0.02 & 16.31 $\pm$ 0.01 & 15.67 $\pm$ 0.01 \\
60101749 & 90.7996 & 1.93952 & (26,35,23) & 1.65653 & 0.37 & 0.34 & 0.40 & ea & 17.46 $\pm$ 0.02 & 17.20 $\pm$ 0.01 & 16.71 $\pm$ 0.02 \\
60120445 & 90.9378 & 1.89329 & (26,33,23) & 0.30214 & 0.32 & 0.33 & 0.34 & ew & 17.44 $\pm$ 0.02 & 16.92 $\pm$ 0.01 & 16.24 $\pm$ 0.01 \\
60122316 & 90.9513 & 1.93885 & (24,33,22) & 0.31013 & 0.24 & 0.34 & 0.23 & ew & 15.67 $\pm$ 0.02 & 15.21 $\pm$ 0.00 & 14.57 $\pm$ 0.01 \\
60174712 & 91.3297 & 1.89678 & (20,35,21) & 0.25731 & 0.19 & 0.25 & 0.20 & ew & 17.91 $\pm$ 0.03 & 17.31 $\pm$ 0.02 & 16.65 $\pm$ 0.02 \\
60180976 & 91.3742 & 2.08412 & (17,30,14) & 0.39277 & 0.41 & 0.49 & 0.41 & eb & 18.20 $\pm$ 0.04 & 17.76 $\pm$ 0.02 & 17.18 $\pm$ 0.02 \\
60207206 & 91.5533 & 2.03851 & (18,28,27) & 0.35500 & 0.56 & 0.31 & 0.27 & ew & 17.90 $\pm$ 0.03 & 17.39 $\pm$ 0.02 & 16.93 $\pm$ 0.02 \\
60259861 & 91.9296 & 1.75829 & (17,22,23) & 0.42056 & 0.43 & 0.38 & 0.49 & ew & 16.92 $\pm$ 0.02 & 16.15 $\pm$ 0.01 & 15.51 $\pm$ 0.01 \\
60260561 & 91.9347 & 1.99845 & (0,28,18) & 0.34525 & 0.0 & 0.30 & 0.24 & ew & 0.0 $\pm$ 0.0 & 17.78 $\pm$ 0.02 & 17.04 $\pm$ 0.02 \\
60277092 & 92.0544 & 2.05071 & (16,25,24) & 0.34487 & 0.37 & 0.44 & 0.32 & ew & 16.05 $\pm$ 0.02 & 15.48 $\pm$ 0.00 & 14.81 $\pm$ 0.01 \\
60277148 & 92.0548 & 2.07585 & (15,23,21) & 0.28537 & 0.32 & 0.36 & 0.39 & ew & 18.15 $\pm$ 0.04 & 17.48 $\pm$ 0.02 & 16.66 $\pm$ 0.02 \\
60287333 & 92.1283 & 2.00478 & (0,28,18) & 1.43244 & 0.0 & 0.62 & 0.51 & ea & 0.0 $\pm$ 0.0 & 17.08 $\pm$ 0.01 & 16.16 $\pm$ 0.01 \\
60289718 & 92.1464 & 1.88380 & (20,29,19) & 0.43683 & 0.25 & 0.29 & 0.30 & ew & 17.06 $\pm$ 0.02 & 16.35 $\pm$ 0.01 & 15.48 $\pm$ 0.01 \\
60382705 & 92.8234 & 1.95283 & (13,22,11) & 0.27962 & 0.67 & 0.60 & 0.44 & ew & 17.93 $\pm$ 0.03 & 17.15 $\pm$ 0.01 & 16.24 $\pm$ 0.01 \\
60490130 & 93.5863 & 1.75801 & (12,21,17) & 0.36854 & 0.27 & 0.43 & 0.39 & ea & 17.08 $\pm$ 0.02 & 16.62 $\pm$ 0.01 & 16.01 $\pm$ 0.01 \\
60567429 & 94.1764 & 2.06118 & (0,10,18) & 0.31540 & 0.0 & 0.33 & 0.32 & ew & 0.0 $\pm$ 0.0 & 18.29 $\pm$ 0.03 & 17.74 $\pm$ 0.04 \\
60578294 & 94.2563 & 1.90371 & (12,11,15) & 0.3151 & 0.23 & 0.23 & 0.25 & ew & 17.87 $\pm$ 0.03 & 17.36 $\pm$ 0.02 & 16.89 $\pm$ 0.02 \\
60585354 & 94.3064 & 1.83312 & (12,11,18) & 0.45623 & 0.59 & 0.49 & 0.54 & ew & 17.61 $\pm$ 0.02 & 17.29 $\pm$ 0.02 & 16.79 $\pm$ 0.02 \\
60615578 & 94.5177 & 1.88267 & (15,11,18) & 0.35255 & 0.51 & 0.35 & 0.32 & ew & 15.98 $\pm$ 0.02 & 15.51 $\pm$ 0.00 & 15.19 $\pm$ 0.01 \\
60618398 & 94.5368 & 1.90887 & (12,10,18) & 0.26625 & 0.55 & 0.26 & 0.46 & ew & 18.26 $\pm$ 0.04 & 17.51 $\pm$ 0.02 & 16.71 $\pm$ 0.02 \\
60840575 & 96.2376 & 1.80370 & (14,7,12) & 0.48379 & 0.28 & 0.31 & 0.41 & ew & 18.66 $\pm$ 0.05 & 18.08 $\pm$ 0.03 & 17.61 $\pm$ 0.03 \\
60878443 & 96.5251 & 1.95745 & (18,10,11) & 0.83775 & 0.68 & 0.60 & 0.57 & ea & 17.22 $\pm$ 0.02 & 16.80 $\pm$ 0.01 & 16.13 $\pm$ 0.01 \\
40508623 & 74.2748 & 5.33473 & (17,11,0) & 1.38830 & 0.32 & 0.32 & 0.0 & ew & 18.31 $\pm$ 0.06 & 17.91 $\pm$ 0.04 & 0.0 $\pm$ 0.0 \\
40539169 & 74.6333 & 5.20249 & (20,12,0) & 0.44735 & 0.31 & 0.26 & 0.0 & ew & 14.88 $\pm$ 0.01 & 14.48 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
40410911 & 73.1042 & 4.56914 & (16,20,0) & 0.38303 & 0.24 & 0.36 & 0.0 & ew & 17.90 $\pm$ 0.04 & 17.50 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
40419252 & 73.2099 & 4.77186 & (12,19,0) & 0.31732 & 0.36 & 0.38 & 0.0 & ew & 16.00 $\pm$ 0.01 & 15.48 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
40517233 & 74.3755 & 4.65902 & (19,17,0) & 0.25372 & 0.52 & 0.38 & 0.0 & ew & 17.86 $\pm$ 0.03 & 17.49 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
40421225 & 73.2336 & 3.59787 & (19,20,22) & 2.06681 & 0.41 & 0.62 & 0.56 & ea & 14.98 $\pm$ 0.01 & 14.81 $\pm$ 0.01 & 14.69 $\pm$ 0.01 \\
40458997 & 73.6945 & 3.64800 & (21,20,21) & 0.28715 & 0.51 & 0.53 & 0.49 & ew & 15.13 $\pm$ 0.01 & 14.68 $\pm$ 0.01 & 14.27 $\pm$ 0.01 \\
40494440 & 74.1124 & 3.54062 & (18,9,14) & 0.35284 & 0.28 & 0.17 & 0.23 & ew & 14.3 $\pm$ 0.01 & 13.97 $\pm$ 0.01 & 13.50 $\pm$ 0.01 \\
40556678 & 74.8392 & 3.96906 & (51,37,32) & 0.41060 & 0.35 & 0.28 & 0.19 & ew & 15.83 $\pm$ 0.01 & 15.63 $\pm$ 0.01 & 15.44 $\pm$ 0.01 \\
40567663 & 74.9678 & 3.56225 & (26,15,0) & 0.33340 & 0.37 & 0.39 & 0.0 & ew & 18.13 $\pm$ 0.05 & 17.81 $\pm$ 0.04 & 0.0 $\pm$ 0.0 \\
50057618 & 75.6055 & 5.75843 & (15,19,24) & 0.39409 & 0.46 & 0.33 & 0.32 & ew & 15.19 $\pm$ 0.01 & 14.97 $\pm$ 0.01 & 14.52 $\pm$ 0.01 \\
50088742 & 75.9277 & 5.67430 & (19,18,19) & 0.51726 & 0.45 & 0.28 & 0.26 & ew & 15.29 $\pm$ 0.01 & 15.05 $\pm$ 0.01 & 14.62 $\pm$ 0.01 \\
50096181 & 76.0013 & 5.79369 & (16,17,20) & 0.29192 & 0.33 & 0.32 & 0.3 & ew & 16.84 $\pm$ 0.02 & 16.29 $\pm$ 0.01 & 15.76 $\pm$ 0.01 \\
50107075 & 76.1116 & 5.56829 & (18,16,21) & 0.73002 & 0.39 & 0.44 & 0.35 & ea & 15.09 $\pm$ 0.01 & 14.92 $\pm$ 0.01 & 14.62 $\pm$ 0.01 \\
50148458 & 76.5552 & 5.82154 & (13,16,20) & 1.37289 & 0.7 & 0.41 & 0.30 & ea & 18.46 $\pm$ 0.07 & 17.38 $\pm$ 0.03 & 16.23 $\pm$ 0.02 \\
50189044 & 76.9914 & 5.72902 & (19,17,20) & 0.25944 & 0.49 & 0.46 & 0.50 & ew & 15.76 $\pm$ 0.01 & 15.5 $\pm$ 0.01 & 15.00 $\pm$ 0.01 \\
50207297 & 77.1816 & 5.86626 & (20,18,14) & 0.20311 & 0.61 & 0.61 & 0.39 & ew & 17.02 $\pm$ 0.02 & 16.38 $\pm$ 0.01 & 15.96 $\pm$ 0.01 \\
50216332 & 77.2725 & 5.88113 & (19,19,22) & 0.46696 & 0.64 & 0.61 & 0.63 & ea & 16.11 $\pm$ 0.01 & 15.71 $\pm$ 0.01 & 15.12 $\pm$ 0.01 \\
50283773 & 77.8998 & 5.68789 & (17,16,20) & 0.28289 & 0.47 & 0.50 & 0.49 & ew & 17.28 $\pm$ 0.03 & 17.06 $\pm$ 0.02 & 16.63 $\pm$ 0.02 \\
50443226 & 79.3450 & 5.90648 & (16,18,23) & 0.54885 & 0.61 & 0.20 & 0.12 & ew & 15.83 $\pm$ 0.01 & 15.22 $\pm$ 0.01 & 14.24 $\pm$ 0.01 \\
50467272 & 79.5703 & 5.62278 & (16,20,16) & 0.38998 & 0.57 & 0.39 & 0.33 & ew & 15.47 $\pm$ 0.01 & 15.09 $\pm$ 0.01 & 14.70 $\pm$ 0.01 \\
50592282 & 80.7113 & 5.73228 & (16,19,20) & 0.32038 & 0.4 & 0.29 & 0.27 & ew & 17.93 $\pm$ 0.05 & 17.45 $\pm$ 0.03 & 16.93 $\pm$ 0.03 \\
50653408 & 81.2200 & 5.74281 & (14,19,22) & 0.38863 & 0.27 & 0.28 & 0.27 & ew & 16.49 $\pm$ 0.01 & 16.28 $\pm$ 0.01 & 15.8 $\pm$ 0.01 \\
50691067 & 81.5322 & 5.88029 & (18,20,20) & 1.12994 & 0.25 & 0.26 & 0.24 & ew & 14.63 $\pm$ 0.01 & 14.55 $\pm$ 0.01 & 14.14 $\pm$ 0.01 \\
50724279 & 81.8019 & 5.98868 & (16,16,21) & 0.25033 & 0.62 & 0.43 & 0.41 & ew & 18.34 $\pm$ 0.06 & 18.08 $\pm$ 0.04 & 17.37 $\pm$ 0.05 \\
50793492 & 82.3572 & 5.83179 & (17,17,17) & 0.26489 & 0.24 & 0.24 & 0.24 & ew & 16.51 $\pm$ 0.01 & 15.86 $\pm$ 0.01 & 15.10 $\pm$ 0.01 \\
50882615 & 83.1125 & 5.99973 & (19,18,20) & 0.32614 & 0.46 & 0.50 & 0.41 & ew & 15.52 $\pm$ 0.01 & 15.06 $\pm$ 0.01 & 14.26 $\pm$ 0.01 \\
50891351 & 83.1894 & 5.72582 & (22,18,21) & 0.27920 & 0.31 & 0.26 & 0.26 & ew & 16.35 $\pm$ 0.01 & 15.82 $\pm$ 0.01 & 15.17 $\pm$ 0.01 \\
50916933 & 83.4127 & 5.81559 & (17,16,21) & 1.24147 & 0.56 & 0.49 & 0.5 & ew & 15.85 $\pm$ 0.01 & 15.74 $\pm$ 0.01 & 15.32 $\pm$ 0.01 \\
50957494 & 83.7538 & 5.56540 & (20,13,19) & 0.48729 & 0.72 & 0.73 & 0.70 & ew & 17.44 $\pm$ 0.03 & 17.10 $\pm$ 0.02 & 16.50 $\pm$ 0.02 \\
51026720 & 84.3330 & 5.81475 & (18,16,17) & 0.45626 & 0.36 & 0.33 & 0.25 & ew & 14.50 $\pm$ 0.01 & 14.22 $\pm$ 0.01 & 13.61 $\pm$ 0.01 \\
51072869 & 84.7191 & 5.61887 & (15,17,19) & 0.40529 & 0.55 & 0.54 & 0.47 & ew & 17.60 $\pm$ 0.04 & 17.15 $\pm$ 0.02 & 16.52 $\pm$ 0.02 \\
50064487 & 75.6806 & 5.07014 & (21,12,20) & 0.55526 & 0.54 & 0.38 & 0.38 & ew & 15.78 $\pm$ 0.01 & 15.63 $\pm$ 0.01 & 15.42 $\pm$ 0.03 \\
50400992 & 78.9566 & 5.21046 & (22,13,20) & 0.27265 & 0.59 & 0.48 & 0.51 & ew & 15.56 $\pm$ 0.01 & 15.20 $\pm$ 0.01 & 14.60 $\pm$ 0.02 \\
50423084 & 79.1571 & 5.26208 & (20,15,21) & 0.29180 & 0.37 & 0.25 & 0.41 & ew & 17.34 $\pm$ 0.03 & 16.90 $\pm$ 0.02 & 16.15 $\pm$ 0.04 \\
50434679 & 79.2645 & 5.21278 & (21,15,21) & 0.95828 & 0.38 & 0.36 & 0.45 & ea & 16.13 $\pm$ 0.01 & 15.92 $\pm$ 0.01 & 15.49 $\pm$ 0.03 \\
50486089 & 79.7487 & 5.23114 & (16,16,19) & 0.26053 & 0.62 & 0.42 & 0.35 & ew & 16.76 $\pm$ 0.02 & 16.31 $\pm$ 0.01 & 15.84 $\pm$ 0.04 \\
50488408 & 79.7701 & 5.17122 & (18,15,22) & 0.69960 & 0.72 & 0.65 & 0.71 & ea & 17.56 $\pm$ 0.03 & 16.82 $\pm$ 0.02 & 15.82 $\pm$ 0.04 \\
50607820 & 80.8463 & 5.29003 & (20,14,17) & 0.57685 & 0.45 & 0.46 & 0.59 & ew & 17.52 $\pm$ 0.03 & 17.3 $\pm$ 0.02 & 17.20 $\pm$ 0.09 \\
50658547 & 81.2628 & 5.03111 & (20,15,0) & 1.28602 & 0.34 & 0.20 & 0.0 & ew & 15.04 $\pm$ 0.01 & 14.86 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50698135 & 81.5900 & 5.29900 & (20,0,18) & 0.28262 & 0.50 & 0.0 & 0.44 & ew & 17.12 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 15.96 $\pm$ 0.04 \\
50793950 & 82.3607 & 5.06924 & (23,14,19) & 0.29600 & 0.32 & 0.32 & 0.44 & ew & 15.85 $\pm$ 0.01 & 15.58 $\pm$ 0.01 & 15.20 $\pm$ 0.03 \\
50912009 & 83.3693 & 5.26496 & (20,14,19) & 0.35349 & 0.65 & 0.51 & 0.62 & ew & 16.84 $\pm$ 0.02 & 16.37 $\pm$ 0.01 & 15.73 $\pm$ 0.03 \\
50939657 & 83.6057 & 5.08963 & (20,14,21) & 0.25759 & 0.66 & 0.65 & 0.62 & ew & 16.87 $\pm$ 0.02 & 16.36 $\pm$ 0.01 & 15.79 $\pm$ 0.04 \\
50951000 & 83.7002 & 5.07227 & (20,14,21) & 2.90498 & 0.77 & 0.61 & 0.78 & ea & 18.20 $\pm$ 0.05 & 17.44 $\pm$ 0.03 & 16.49 $\pm$ 0.05 \\
50952250 & 83.7108 & 5.00152 & (21,9,17) & 0.24115 & 0.48 & 0.28 & 0.35 & ew & 16.95 $\pm$ 0.02 & 16.74 $\pm$ 0.01 & 15.95 $\pm$ 0.04 \\
50961355 & 83.7866 & 5.09232 & (23,15,22) & 0.29925 & 0.48 & 0.42 & 0.48 & ew & 17.41 $\pm$ 0.03 & 17.10 $\pm$ 0.02 & 16.61 $\pm$ 0.06 \\
51006204 & 84.1605 & 5.34003 & (0,12,19) & 0.06006 & 0.0 & 0.28 & 1.08 & ea & 0.0 $\pm$ 0.0 & 18.76 $\pm$ 0.07 & 17.04 $\pm$ 0.08 \\
51044826 & 84.4851 & 5.04101 & (19,15,20) & 2.02277 & 0.78 & 0.67 & 0.78 & ea & 17.29 $\pm$ 0.02 & 16.84 $\pm$ 0.02 & 16.19 $\pm$ 0.04 \\
51048972 & 84.5203 & 4.99535 & (17,10,19) & 0.31935 & 0.68 & 0.65 & 0.51 & ew & 17.18 $\pm$ 0.02 & 16.40 $\pm$ 0.01 & 15.53 $\pm$ 0.03 \\
51090913 & 84.8685 & 5.30810 & (23,14,0) & 0.28536 & 0.46 & 0.34 & 0.0 & ew & 17.27 $\pm$ 0.02 & 16.34 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51188444 & 85.7208 & 4.98640 & (0,8,19) & 0.33915 & 0.0 & 0.23 & 0.30 & ew & 0.0 $\pm$ 0.0 & 14.82 $\pm$ 0.01 & 14.43 $\pm$ 0.02 \\
51198026 & 85.8024 & 5.33633 & (20,13,18) & 0.31573 & 0.39 & 0.29 & 0.25 & eb & 16.64 $\pm$ 0.02 & 16.02 $\pm$ 0.01 & 15.52 $\pm$ 0.03 \\
51274299 & 86.4573 & 5.19172 & (20,11,20) & 0.36985 & 0.48 & 0.46 & 0.44 & eb & 16.08 $\pm$ 0.01 & 15.29 $\pm$ 0.01 & 14.48 $\pm$ 0.02 \\
51297128 & 86.6592 & 5.15545 & (19,13,17) & 0.45748 & 0.44 & 0.38 & 0.51 & ew & 15.99 $\pm$ 0.01 & 15.43 $\pm$ 0.01 & 14.82 $\pm$ 0.03 \\
51310859 & 86.7823 & 5.26988 & (20,8,20) & 0.35111 & 0.37 & 0.26 & 0.50 & ew & 17.98 $\pm$ 0.04 & 17.53 $\pm$ 0.03 & 16.85 $\pm$ 0.07 \\
51340891 & 87.0445 & 5.26646 & (18,13,16) & 0.44887 & 0.25 & 0.21 & 0.26 & ew & 16.01 $\pm$ 0.01 & 15.42 $\pm$ 0.01 & 14.77 $\pm$ 0.03 \\
51347369 & 87.0990 & 5.17294 & (18,11,17) & 0.52204 & 0.63 & 0.53 & 0.55 & ew & 15.60 $\pm$ 0.01 & 15.09 $\pm$ 0.01 & 14.54 $\pm$ 0.02 \\
51439824 & 87.8165 & 5.36860 & (15,11,18) & 0.51983 & 0.55 & 0.49 & 0.54 & ew & 16.90 $\pm$ 0.02 & 16.59 $\pm$ 0.01 & 16.06 $\pm$ 0.04 \\
51556152 & 88.7464 & 5.07209 & (18,13,18) & 0.21491 & 0.44 & 0.61 & 0.40 & ew & 16.74 $\pm$ 0.02 & 15.56 $\pm$ 0.01 & 15.06 $\pm$ 0.03 \\
51635765 & 89.3395 & 5.24397 & (19,12,17) & 0.42778 & 0.48 & 0.48 & 0.50 & ew & 16.72 $\pm$ 0.02 & 15.92 $\pm$ 0.01 & 15.14 $\pm$ 0.03 \\
51699218 & 89.7537 & 5.31616 & (20,12,15) & 0.29234 & 0.33 & 0.24 & 0.28 & ew & 17.62 $\pm$ 0.03 & 16.75 $\pm$ 0.01 & 15.32 $\pm$ 0.03 \\
50116858 & 76.2134 & 4.41846 & (16,15,13) & 0.25929 & 0.60 & 0.47 & 0.45 & ew & 17.76 $\pm$ 0.03 & 17.28 $\pm$ 0.03 & 16.70 $\pm$ 0.03 \\
50141196 & 76.4760 & 4.54716 & (21,16,19) & 0.45564 & 0.46 & 0.37 & 0.43 & ew & 16.5 $\pm$ 0.01 & 16.05 $\pm$ 0.01 & 15.62 $\pm$ 0.02 \\
50061013 & 75.6430 & 3.68682 & (33,26,26) & 0.29290 & 0.29 & 0.26 & 0.18 & ew & 16.87 $\pm$ 0.02 & 16.51 $\pm$ 0.02 & 16.24 $\pm$ 0.02 \\
50128282 & 76.3377 & 3.81214 & (51,10,0) & 0.45392 & 0.45 & 0.21 & 0.0 & ew & 13.68 $\pm$ 0.01 & 13.52 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50251372 & 77.6048 & 3.93631 & (50,38,36) & 0.34241 & 0.36 & 0.33 & 0.31 & ew & 16.52 $\pm$ 0.02 & 16.13 $\pm$ 0.02 & 15.78 $\pm$ 0.01 \\
50271843 & 77.7882 & 3.99025 & (45,36,36) & 0.36675 & 0.48 & 0.45 & 0.66 & eb & 17.93 $\pm$ 0.05 & 17.49 $\pm$ 0.04 & 17.13 $\pm$ 0.03 \\
50276127 & 77.8289 & 3.98075 & (34,35,33) & 0.27483 & 0.57 & 0.68 & 0.74 & ew & 18.73 $\pm$ 0.08 & 18.02 $\pm$ 0.05 & 17.43 $\pm$ 0.04 \\
50279491 & 77.8603 & 3.81617 & (45,30,33) & 0.40645 & 0.71 & 0.27 & 0.31 & ew & 17.73 $\pm$ 0.04 & 17.33 $\pm$ 0.03 & 17.19 $\pm$ 0.03 \\
50294558 & 77.9946 & 3.64116 & (32,19,20) & 1.85383 & 0.36 & 0.35 & 0.20 & ew & 18.12 $\pm$ 0.05 & 17.52 $\pm$ 0.04 & 16.92 $\pm$ 0.03 \\
50298388 & 78.0273 & 3.83457 & (44,33,28) & 1.99390 & 0.48 & 0.43 & 0.52 & ew & 18.34 $\pm$ 0.06 & 17.97 $\pm$ 0.05 & 17.46 $\pm$ 0.04 \\
50311100 & 78.1432 & 3.58402 & (32,17,18) & 0.25745 & 0.21 & 0.23 & 0.14 & ew & 14.90 $\pm$ 0.01 & 14.29 $\pm$ 0.01 & 13.81 $\pm$ 0.01 \\
50335109 & 78.3657 & 3.74252 & (43,35,35) & 0.32076 & 0.42 & 0.35 & 0.33 & ew & 15.56 $\pm$ 0.01 & 15.04 $\pm$ 0.01 & 14.59 $\pm$ 0.01 \\
50349482 & 78.4959 & 3.66260 & (32,23,24) & 0.54915 & 0.44 & 0.36 & 0.34 & eb & 14.98 $\pm$ 0.01 & 14.76 $\pm$ 0.01 & 14.57 $\pm$ 0.01 \\
50369474 & 78.6757 & 3.69106 & (35,27,26) & 1.91536 & 0.49 & 0.48 & 0.45 & ea & 15.06 $\pm$ 0.01 & 14.62 $\pm$ 0.01 & 14.24 $\pm$ 0.01 \\
50386575 & 78.8288 & 3.85137 & (43,39,29) & 0.23821 & 0.33 & 0.42 & 0.35 & ew & 16.22 $\pm$ 0.02 & 15.36 $\pm$ 0.01 & 14.84 $\pm$ 0.01 \\
50390110 & 78.8599 & 3.85233 & (48,36,27) & 0.53534 & 0.66 & 0.44 & 0.4 & ew & 14.09 $\pm$ 0.01 & 13.88 $\pm$ 0.01 & 13.77 $\pm$ 0.01 \\
50392433 & 78.8807 & 3.85264 & (47,29,0) & 0.43440 & 0.35 & 0.30 & 0.0 & eb & 13.77 $\pm$ 0.01 & 13.53 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50424009 & 79.1657 & 3.57321 & (28,13,19) & 0.56131 & 0.32 & 0.26 & 0.28 & ea & 17.19 $\pm$ 0.03 & 16.63 $\pm$ 0.02 & 16.32 $\pm$ 0.02 \\
50431752 & 79.2373 & 4.13486 & (19,22,13) & 0.31339 & 0.34 & 0.36 & 0.26 & ew & 16.03 $\pm$ 0.02 & 15.36 $\pm$ 0.01 & 15.00 $\pm$ 0.01 \\
50481359 & 79.7035 & 3.56530 & (29,11,22) & 0.38298 & 0.28 & 0.27 & 0.35 & ew & 16.36 $\pm$ 0.02 & 15.98 $\pm$ 0.02 & 15.71 $\pm$ 0.01 \\
50543256 & 80.2734 & 3.60018 & (31,19,22) & 0.43799 & 0.70 & 0.62 & 0.60 & ew & 16.81 $\pm$ 0.02 & 16.43 $\pm$ 0.02 & 16.15 $\pm$ 0.02 \\
50545221 & 80.2908 & 3.63751 & (29,0,18) & 0.38117 & 0.70 & 0.0 & 0.63 & ew & 16.75 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 16.05 $\pm$ 0.01 \\
50546307 & 80.3005 & 3.95289 & (51,33,4) & 0.40051 & 0.45 & 0.25 & 0.15 & ew & 13.98 $\pm$ 0.01 & 13.64 $\pm$ 0.01 & 13.53 $\pm$ 0.01 \\
50690051 & 81.5239 & 3.64015 & (30,17,19) & 0.31470 & 0.43 & 0.43 & 0.50 & ew & 16.91 $\pm$ 0.02 & 16.50 $\pm$ 0.02 & 16.10 $\pm$ 0.02 \\
50703622 & 81.6361 & 3.82652 & (41,30,33) & 0.28087 & 0.55 & 0.48 & 0.49 & ew & 16.41 $\pm$ 0.02 & 15.91 $\pm$ 0.02 & 15.44 $\pm$ 0.01 \\
50711451 & 81.6998 & 3.87504 & (49,32,21) & 0.51593 & 0.82 & 0.79 & 0.93 & ea & 16.96 $\pm$ 0.02 & 16.38 $\pm$ 0.02 & 15.82 $\pm$ 0.01 \\
50780824 & 82.2521 & 3.90153 & (50,40,34) & 0.39883 & 0.45 & 0.40 & 0.49 & ew & 15.89 $\pm$ 0.01 & 15.43 $\pm$ 0.01 & 15.00 $\pm$ 0.01 \\
50787252 & 82.3040 & 4.01608 & (43,36,36) & 4.37137 & 0.97 & 0.93 & 0.85 & ea & 14.94 $\pm$ 0.01 & 14.78 $\pm$ 0.01 & 14.61 $\pm$ 0.01 \\
50797908 & 82.3935 & 4.07657 & (27,39,27) & 0.34486 & 0.53 & 0.69 & 0.75 & ew & 17.5 $\pm$ 0.03 & 17.06 $\pm$ 0.03 & 16.64 $\pm$ 0.02 \\
50798370 & 82.3974 & 3.95830 & (47,30,17) & 0.89868 & 0.45 & 0.46 & 0.40 & ea & 15.76 $\pm$ 0.01 & 15.23 $\pm$ 0.01 & 14.75 $\pm$ 0.01 \\
50798398 & 82.3975 & 4.11426 & (20,26,0) & 0.27757 & 0.71 & 0.69 & 0.0 & ew & 16.16 $\pm$ 0.02 & 15.51 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50801428 & 82.4235 & 3.64568 & (28,20,19) & 1.01925 & 0.34 & 0.28 & 0.30 & ea & 15.91 $\pm$ 0.01 & 15.08 $\pm$ 0.01 & 14.37 $\pm$ 0.01 \\
50818997 & 82.5719 & 3.81201 & (46,32,33) & 0.26930 & 0.33 & 0.32 & 0.35 & ew & 17.89 $\pm$ 0.05 & 17.54 $\pm$ 0.04 & 17.07 $\pm$ 0.03 \\
50823983 & 82.6144 & 3.71283 & (36,22,21) & 0.48409 & 0.36 & 0.36 & 0.35 & ew & 16.30 $\pm$ 0.02 & 15.98 $\pm$ 0.02 & 15.68 $\pm$ 0.01 \\
50824981 & 82.6227 & 3.78130 & (38,29,39) & 0.2446 & 0.37 & 0.35 & 0.27 & ew & 14.91 $\pm$ 0.01 & 14.45 $\pm$ 0.01 & 14.01 $\pm$ 0.01 \\
50891971 & 83.1951 & 3.63965 & (29,18,16) & 0.35584 & 0.69 & 0.71 & 0.59 & eb & 17.25 $\pm$ 0.03 & 16.76 $\pm$ 0.02 & 16.23 $\pm$ 0.02 \\
50911750 & 83.3670 & 3.87074 & (46,36,30) & 0.29624 & 0.30 & 0.90 & 0.25 & ew & 17.72 $\pm$ 0.04 & 17.00 $\pm$ 0.03 & 16.50 $\pm$ 0.02 \\
50978560 & 83.9275 & 4.03095 & (46,33,0) & 0.35366 & 0.53 & 0.46 & 0.0 & ew & 14.40 $\pm$ 0.01 & 13.77 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50991946 & 84.0403 & 3.70132 & (32,23,25) & 0.22194 & 0.72 & 0.87 & 0.61 & ew & 17.70 $\pm$ 0.04 & 16.93 $\pm$ 0.03 & 16.23 $\pm$ 0.02 \\
51015973 & 84.2421 & 3.90570 & (55,42,30) & 0.37719 & 0.64 & 0.62 & 0.6 & ew & 17.18 $\pm$ 0.03 & 16.68 $\pm$ 0.02 & 16.22 $\pm$ 0.02 \\
51065437 & 84.6565 & 3.79275 & (41,28,33) & 0.36088 & 1.98 & 0.51 & 0.50 & ew & 17.06 $\pm$ 0.03 & 16.46 $\pm$ 0.02 & 15.95 $\pm$ 0.01 \\
51143378 & 85.3233 & 3.92311 & (46,35,18) & 0.29375 & 0.89 & 0.57 & 0.53 & ew & 18.28 $\pm$ 0.06 & 17.27 $\pm$ 0.03 & 16.29 $\pm$ 0.02 \\
51151082 & 85.3935 & 3.62773 & (30,15,16) & 0.28598 & 0.55 & 0.47 & 0.46 & eb & 16.02 $\pm$ 0.02 & 15.20 $\pm$ 0.01 & 14.48 $\pm$ 0.01 \\
51157669 & 85.4534 & 3.75229 & (38,31,28) & 1.41928 & 0.39 & 0.47 & 0.38 & ea & 18.63 $\pm$ 0.08 & 17.88 $\pm$ 0.05 & 17.33 $\pm$ 0.04 \\
51185766 & 85.6987 & 3.87449 & (51,40,26) & 21.6168 & 0.82 & 0.66 & 0.57 & ea & 17.24 $\pm$ 0.03 & 16.84 $\pm$ 0.02 & 16.33 $\pm$ 0.02 \\
51189789 & 85.7323 & 3.61600 & (27,18,21) & 0.26833 & 0.64 & 0.69 & 0.51 & ew & 18.68 $\pm$ 0.08 & 17.64 $\pm$ 0.04 & 17.04 $\pm$ 0.03 \\
51199913 & 85.8189 & 3.59116 & (29,16,16) & 0.57335 & 0.36 & 0.34 & 0.27 & ew & 18.28 $\pm$ 0.06 & 17.58 $\pm$ 0.04 & 17.02 $\pm$ 0.03 \\
51231455 & 86.0880 & 3.78963 & (42,27,0) & 0.32053 & 1.38 & 0.39 & 0.0 & ew & 18.01 $\pm$ 0.05 & 17.20 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
51235641 & 86.1235 & 3.93230 & (49,41,34) & 0.33392 & 0.59 & 0.38 & 0.70 & ew & 16.05 $\pm$ 0.02 & 15.24 $\pm$ 0.01 & 14.45 $\pm$ 0.01 \\
51239506 & 86.1559 & 3.80685 & (44,26,36) & 0.28362 & 1.24 & 0.24 & 0.21 & ew & 16.93 $\pm$ 0.02 & 15.95 $\pm$ 0.02 & 15.10 $\pm$ 0.01 \\
51242499 & 86.1811 & 4.03452 & (46,36,37) & 1.13497 & 0.52 & 0.54 & 0.48 & ea & 15.37 $\pm$ 0.01 & 14.73 $\pm$ 0.01 & 14.13 $\pm$ 0.01 \\
51249595 & 86.2416 & 3.72310 & (40,33,36) & 2.05702 & 0.65 & 0.41 & 0.43 & ea & 16.91 $\pm$ 0.02 & 16.05 $\pm$ 0.02 & 15.15 $\pm$ 0.01 \\
51287703 & 86.5757 & 3.64246 & (28,15,17) & 0.69964 & 0.67 & 0.63 & 0.57 & ew & 16.46 $\pm$ 0.02 & 15.98 $\pm$ 0.02 & 15.51 $\pm$ 0.01 \\
51292247 & 86.6157 & 3.97777 & (47,38,35) & 0.41798 & 0.58 & 0.38 & 0.37 & ew & 17.05 $\pm$ 0.03 & 16.09 $\pm$ 0.02 & 15.42 $\pm$ 0.01 \\
51329779 & 86.9493 & 3.99280 & (22,32,33) & 0.35914 & 0.90 & 0.80 & 0.81 & ew & 18.99 $\pm$ 0.09 & 18.25 $\pm$ 0.06 & 17.42 $\pm$ 0.04 \\
51353765 & 87.1503 & 4.05367 & (31,37,33) & 9.98573 & 0.49 & 0.44 & 0.29 & ew & 16.91 $\pm$ 0.02 & 15.68 $\pm$ 0.01 & 14.24 $\pm$ 0.01 \\
51358312 & 87.1872 & 3.69119 & (29,25,24) & 0.32936 & 0.48 & 0.47 & 0.40 & ew & 18.44 $\pm$ 0.07 & 17.87 $\pm$ 0.05 & 17.27 $\pm$ 0.04 \\
51413573 & 87.6144 & 4.14862 & (19,17,16) & 0.27570 & 0.74 & 0.53 & 0.41 & ew & 17.96 $\pm$ 0.05 & 17.13 $\pm$ 0.03 & 16.34 $\pm$ 0.02 \\
51551470 & 88.7104 & 4.02364 & (40,39,35) & 0.49229 & 0.86 & 0.36 & 0.37 & ew & 18.07 $\pm$ 0.05 & 17.03 $\pm$ 0.03 & 15.90 $\pm$ 0.01 \\
51554869 & 88.7366 & 3.60181 & (26,19,20) & 0.34478 & 0.37 & 0.37 & 0.35 & ew & 16.25 $\pm$ 0.02 & 15.12 $\pm$ 0.01 & 13.93 $\pm$ 0.01 \\
51633384 & 89.3235 & 3.71682 & (40,30,27) & 2.52841 & 0.54 & 0.53 & 0.28 & ea & 17.25 $\pm$ 0.03 & 16.46 $\pm$ 0.02 & 15.62 $\pm$ 0.01 \\
51637836 & 89.3545 & 3.96382 & (43,40,22) & 0.45878 & 0.55 & 0.51 & 0.50 & ew & 15.13 $\pm$ 0.01 & 14.49 $\pm$ 0.01 & 13.83 $\pm$ 0.01 \\
51647088 & 89.4172 & 4.00093 & (36,35,35) & 0.38146 & 0.70 & 0.60 & 0.62 & ew & 18.71 $\pm$ 0.08 & 17.94 $\pm$ 0.05 & 17.19 $\pm$ 0.03 \\
51662663 & 89.5185 & 3.57060 & (27,16,20) & 0.25713 & 0.66 & 0.57 & 0.50 & ew & 17.79 $\pm$ 0.04 & 16.83 $\pm$ 0.02 & 15.97 $\pm$ 0.01 \\
51705107 & 89.7921 & 3.59431 & (29,17,17) & 0.33017 & 0.34 & 0.31 & 0.27 & ew & 16.40 $\pm$ 0.02 & 15.71 $\pm$ 0.01 & 15.06 $\pm$ 0.01 \\
40083051 & 65.6370 & -1.9609 & (32,0,25) & 0.35222 & 0.32 & 0.0 & 0.31 & ew & 14.33 $\pm$ 0.01 & 0.0 $\pm$ 0.0 & 13.53 $\pm$ 0.01 \\
40141914 & 68.0677 & -1.9950 & (36,27,30) & 0.40957 & 0.52 & 0.52 & 0.58 & ew & 15.98 $\pm$ 0.02 & 15.61 $\pm$ 0.01 & 15.16 $\pm$ 0.02 \\
40152097 & 68.4100 & -1.9886 & (32,25,30) & 0.26794 & 0.66 & 0.41 & 0.45 & ew & 17.92 $\pm$ 0.05 & 17.19 $\pm$ 0.02 & 16.60 $\pm$ 0.03 \\
40167353 & 68.9317 & -2.2806 & (26,17,22) & 0.2619 & 0.35 & 0.27 & 0.30 & ew & 17.74 $\pm$ 0.05 & 17.31 $\pm$ 0.03 & 16.61 $\pm$ 0.03 \\
40214294 & 70.1318 & -2.3441 & (25,14,20) & 1.21665 & 0.48 & 0.44 & 0.51 & ew & 14.21 $\pm$ 0.01 & 13.93 $\pm$ 0.01 & 13.55 $\pm$ 0.01 \\
40216809 & 70.1798 & -2.3856 & (24,16,19) & 0.62237 & 0.23 & 0.22 & 0.33 & ew & 16.06 $\pm$ 0.02 & 15.75 $\pm$ 0.01 & 15.39 $\pm$ 0.02 \\
40330828 & 72.0685 & -1.9246 & (30,24,29) & 0.28170 & 0.33 & 0.33 & 0.50 & ew & 16.04 $\pm$ 0.02 & 15.52 $\pm$ 0.01 & 14.96 $\pm$ 0.02 \\
40413074 & 73.1750 & -2.0549 & (44,28,32) & 0.40274 & 0.32 & 0.26 & 0.27 & ew & 15.07 $\pm$ 0.01 & 14.59 $\pm$ 0.01 & 14.07 $\pm$ 0.02 \\
40478116 & 73.9644 & -2.1061 & (36,26,30) & 0.23099 & 0.41 & 0.37 & 0.29 & ew & 17.52 $\pm$ 0.04 & 17.33 $\pm$ 0.03 & 16.49 $\pm$ 0.03 \\
50499158 & 79.8553 & -0.6952 & (58,14,47) & 0.25607 & 0.78 & 0.64 & 0.61 & ew & 17.81 $\pm$ 0.04 & 17.44 $\pm$ 0.03 & 16.94 $\pm$ 0.03 \\
50527821 & 80.1170 & -0.5338 & (58,10,41) & 0.33165 & 0.76 & 0.39 & 0.48 & ew & 15.83 $\pm$ 0.01 & 15.46 $\pm$ 0.01 & 14.92 $\pm$ 0.01 \\
50579339 & 80.5820 & -0.6299 & (60,43,45) & 0.25144 & 0.84 & 0.84 & 0.79 & ew & 16.83 $\pm$ 0.02 & 16.35 $\pm$ 0.01 & 15.74 $\pm$ 0.02 \\
50653608 & 81.2043 & -1.0327 & (19,0,43) & 0.24747 & 0.56 & 0.0 & 0.58 & ew & 17.35 $\pm$ 0.03 & 0.0 $\pm$ 0.0 & 16.10 $\pm$ 0.02 \\
50727066 & 81.8047 & -0.6951 & (44,54,80) & 0.25275 & 0.72 & 0.76 & 0.66 & ew & 18.28 $\pm$ 0.06 & 17.79 $\pm$ 0.03 & 17.3 $\pm$ 0.04 \\
50765017 & 82.1039 & -0.5447 & (62,48,87) & 0.33982 & 0.68 & 0.62 & 0.63 & ew & 16.80 $\pm$ 0.02 & 16.37 $\pm$ 0.01 & 15.79 $\pm$ 0.02 \\
50771676 & 82.1577 & -0.7435 & (61,59,102) & 0.29686 & 0.29 & 0.23 & 0.22 & ew & 16.16 $\pm$ 0.01 & 15.66 $\pm$ 0.01 & 14.91 $\pm$ 0.01 \\
50815994 & 82.5232 & -0.9878 & (27,55,98) & 0.16060 & 0.21 & 0.30 & 0.17 & ew & 16.59 $\pm$ 0.02 & 16.21 $\pm$ 0.01 & 15.67 $\pm$ 0.02 \\
50837510 & 82.7030 & -0.6828 & (64,57,98) & 0.39974 & 0.20 & 0.12 & 0.26 & ew & 16.95 $\pm$ 0.02 & 16.67 $\pm$ 0.02 & 16.13 $\pm$ 0.02 \\
51033757 & 84.3590 & -0.8975 & (62,63,0) & 1.05470 & 0.63 & 0.92 & 0.0 & ew & 15.90 $\pm$ 0.01 & 14.93 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51047175 & 84.4719 & -0.8239 & (64,60,108) & 0.15105 & 0.26 & 0.24 & 0.29 & ew & 15.14 $\pm$ 0.01 & 15.23 $\pm$ 0.01 & 15.17 $\pm$ 0.01 \\
51204961 & 85.8199 & -0.8155 & (60,57,111) & 0.27229 & 0.46 & 0.35 & 0.45 & ew & 17.84 $\pm$ 0.05 & 17.03 $\pm$ 0.02 & 15.99 $\pm$ 0.02 \\
51394111 & 87.4190 & -0.6146 & (30,48,65) & 0.34070 & 0.26 & 0.29 & 0.34 & ew & 18.34 $\pm$ 0.06 & 17.49 $\pm$ 0.03 & 16.65 $\pm$ 0.03 \\
50535283 & 80.1857 & -1.1543 & (37,4,38) & 2.99903 & 1.02 & 1.06 & 0.13 & ea & 15.73 $\pm$ 0.01 & 15.39 $\pm$ 0.01 & 14.91 $\pm$ 0.01 \\
50761981 & 82.0797 & -1.5610 & (26,45,65) & 0.31435 & 0.46 & 0.48 & 0.5 & ew & 18.48 $\pm$ 0.06 & 18.13 $\pm$ 0.05 & 17.80 $\pm$ 0.06 \\
50788205 & 82.2904 & -1.4188 & (42,53,91) & 0.35670 & 0.33 & 0.32 & 0.32 & ew & 15.36 $\pm$ 0.01 & 14.81 $\pm$ 0.01 & 14.19 $\pm$ 0.01 \\
50789669 & 82.3023 & -1.4403 & (49,51,94) & 0.24300 & 0.30 & 0.26 & 0.26 & ew & 15.77 $\pm$ 0.01 & 15.22 $\pm$ 0.01 & 14.62 $\pm$ 0.01 \\
50918295 & 83.3960 & -1.2534 & (0,45,84) & 0.2378 & 0.0 & 0.43 & 0.55 & ew & 0.0 $\pm$ 0.0 & 18.00 $\pm$ 0.05 & 17.62 $\pm$ 0.05 \\
50933210 & 83.5234 & -1.2980 & (44,49,91) & 0.31765 & 0.43 & 0.42 & 0.53 & ew & 17.27 $\pm$ 0.03 & 16.80 $\pm$ 0.02 & 16.22 $\pm$ 0.02 \\
50936079 & 83.5473 & -1.5087 & (42,44,0) & 1.27930 & 0.22 & 0.21 & 0.0 & ew & 14.35 $\pm$ 0.01 & 13.66 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51114393 & 85.0331 & -1.3233 & (32,41,79) & 0.31156 & 0.58 & 0.45 & 0.44 & ew & 17.91 $\pm$ 0.04 & 17.23 $\pm$ 0.03 & 16.58 $\pm$ 0.02 \\
51397444 & 87.4443 & -1.2442 & (19,42,55) & 2.08433 & 0.24 & 0.42 & 0.46 & ea & 16.79 $\pm$ 0.02 & 15.99 $\pm$ 0.01 & 15.24 $\pm$ 0.01 \\
51409696 & 87.5367 & -1.4436 & (16,40,54) & 0.26897 & 0.46 & 0.43 & 0.39 & ew & 18.11 $\pm$ 0.05 & 17.09 $\pm$ 0.02 & 16.18 $\pm$ 0.02 \\
51451903 & 87.8600 & -1.5405 & (0,35,49) & 0.32271 & 0.0 & 0.59 & 0.58 & ew & 0.0 $\pm$ 0.0 & 17.51 $\pm$ 0.03 & 16.87 $\pm$ 0.03 \\
50130978 & 76.3623 & -1.9109 & (23,25,27) & 0.33727 & 0.38 & 0.40 & 0.34 & ew & 15.65 $\pm$ 0.01 & 15.36 $\pm$ 0.01 & 15.07 $\pm$ 0.01 \\
50313800 & 78.1610 & -2.2294 & (10,23,27) & 0.26706 & 0.47 & 0.55 & 0.51 & ew & 14.79 $\pm$ 0.01 & 14.27 $\pm$ 0.01 & 14.23 $\pm$ 0.01 \\
50379385 & 78.7546 & -2.3306 & (26,19,23) & 0.26113 & 0.49 & 0.43 & 0.40 & ew & 14.92 $\pm$ 0.01 & 14.34 $\pm$ 0.01 & 13.74 $\pm$ 0.01 \\
50508506 & 79.9426 & -2.2597 & (47,23,43) & 2.76694 & 0.47 & 0.46 & 0.20 & ew & 17.56 $\pm$ 0.04 & 16.42 $\pm$ 0.02 & 14.71 $\pm$ 0.01 \\
50571325 & 80.5105 & -2.0130 & (76,36,70) & 0.37984 & 0.53 & 0.53 & 0.46 & ew & 17.35 $\pm$ 0.03 & 17.0 $\pm$ 0.02 & 16.60 $\pm$ 0.02 \\
50615100 & 80.8917 & -1.9388 & (58,71,67) & 1.42084 & 0.66 & 0.65 & 0.56 & ea & 15.71 $\pm$ 0.01 & 15.26 $\pm$ 0.01 & 14.81 $\pm$ 0.01 \\
60139366 & 91.0725 & -1.9781 & (29,21,23) & 0.36904 & 0.30 & 0.24 & 0.34 & ew & 17.03 $\pm$ 0.02 & 16.47 $\pm$ 0.02 & 16.00 $\pm$ 0.02 \\
60145380 & 91.1153 & -1.9840 & (0,19,23) & 0.69210 & 0.0 & 0.29 & 0.4 & ew & 0.0 $\pm$ 0.0 & 15.39 $\pm$ 0.03 & 15.01 $\pm$ 0.02 \\
60152089 & 91.1647 & -1.9550 & (24,21,22) & 0.23102 & 0.32 & 0.38 & 0.31 & ew & 17.61 $\pm$ 0.03 & 16.73 $\pm$ 0.02 & 15.91 $\pm$ 0.02 \\
60159436 & 91.2187 & -2.0246 & (21,25,24) & 0.32011 & 0.74 & 0.86 & 0.76 & ew & 18.30 $\pm$ 0.05 & 17.53 $\pm$ 0.03 & 16.67 $\pm$ 0.03 \\
60163655 & 91.2497 & -2.1932 & (29,17,0) & 2.36617 & 0.43 & 0.35 & 0.0 & ea & 16.80 $\pm$ 0.02 & 16.50 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
60191888 & 91.4494 & -2.2075 & (27,21,22) & 0.48843 & 0.49 & 0.30 & 0.51 & ew & 16.62 $\pm$ 0.02 & 16.25 $\pm$ 0.02 & 15.43 $\pm$ 0.02 \\
60270734 & 92.0073 & -2.1783 & (28,19,21) & 5.68045 & 0.79 & 0.26 & 0.71 & ea & 15.26 $\pm$ 0.01 & 14.55 $\pm$ 0.04 & 13.88 $\pm$ 0.03 \\
60303130 & 92.2445 & -2.0602 & (33,18,23) & 1.51910 & 0.61 & 0.42 & 0.42 & ew & 16.75 $\pm$ 0.02 & 16.78 $\pm$ 0.02 & 16.33 $\pm$ 0.03 \\
60393204 & 92.8963 & -2.2102 & (27,15,22) & 0.57113 & 0.37 & 0.32 & 0.40 & ea & 17.54 $\pm$ 0.03 & 17.06 $\pm$ 0.03 & 16.57 $\pm$ 0.03 \\
60482084 & 93.5224 & -2.2289 & (23,14,20) & 0.43237 & 0.42 & 0.41 & 0.45 & ew & 17.08 $\pm$ 0.02 & 16.61 $\pm$ 0.02 & 16.48 $\pm$ 0.03 \\
60734192 & 95.4207 & -2.2509 & (24,18,18) & 0.39109 & 0.43 & 0.6 & 0.41 & ew & 17.43 $\pm$ 0.03 & 16.91 $\pm$ 0.02 & 16.62 $\pm$ 0.03 \\
60794577 & 95.8873 & -2.3002 & (25,0,20) & 0.38237 & 0.39 & 0.0 & 0.35 & ew & 15.81 $\pm$ 0.01 & 0.0 $\pm$ 0.0 & 15.15 $\pm$ 0.02 \\
60821662 & 96.0962 & -2.2236 & (27,15,20) & 0.34410 & 0.84 & 0.44 & 0.83 & eb & 16.47 $\pm$ 0.01 & 15.98 $\pm$ 0.02 & 15.52 $\pm$ 0.02 \\
60911824 & 96.7827 & -2.0779 & (19,14,15) & 0.27825 & 0.64 & 0.59 & 0.61 & ew & 17.75 $\pm$ 0.03 & 17.15 $\pm$ 0.03 & 16.56 $\pm$ 0.03 \\
60957046 & 97.1360 & -2.2467 & (24,16,20) & 0.32546 & 0.28 & 0.24 & 0.26 & ew & 16.71 $\pm$ 0.02 & 16.15 $\pm$ 0.02 & 15.62 $\pm$ 0.02 \\
60980494 & 97.3146 & -2.2629 & (23,16,20) & 0.69497 & 0.64 & 0.75 & 0.72 & ew & 16.20 $\pm$ 0.01 & 15.77 $\pm$ 0.03 & 15.28 $\pm$ 0.02 \\
61003139 & 97.4848 & -2.2621 & (26,19,20) & 2.26622 & 0.28 & 0.39 & 0.29 & ea & 16.30 $\pm$ 0.01 & 15.71 $\pm$ 0.03 & 15.12 $\pm$ 0.02 \\
61015451 & 97.5767 & -2.2839 & (26,17,15) & 0.37868 & 0.31 & 0.27 & 0.30 & ew & 17.57 $\pm$ 0.03 & 16.89 $\pm$ 0.02 & 16.23 $\pm$ 0.03 \\
61262394 & 99.4938 & -2.1165 & (25,17,18) & 0.59372 & 0.65 & 0.56 & 0.60 & ew & 15.12 $\pm$ 0.01 & 14.62 $\pm$ 0.04 & 13.93 $\pm$ 0.03 \\
61270551 & 99.5536 & -2.0477 & (23,17,20) & 0.44462 & 0.20 & 0.31 & 0.29 & ew & 14.58 $\pm$ 0.01 & 14.05 $\pm$ 0.04 & 13.68 $\pm$ 0.03 \\
61420027 & 100.671 & -2.3949 & (22,19,18) & 0.86339 & 0.26 & 0.22 & 0.18 & ew & 16.89 $\pm$ 0.02 & 16.07 $\pm$ 0.02 & 15.24 $\pm$ 0.02 \\
61523537 & 101.560 & -2.2763 & (25,18,16) & 0.48418 & 0.44 & 0.40 & 0.55 & ea & 17.17 $\pm$ 0.02 & 16.60 $\pm$ 0.02 & 15.99 $\pm$ 0.02 \\
61552736 & 101.852 & -2.2575 & (25,20,25) & 0.50640 & 0.49 & 0.42 & 0.47 & ea & 15.57 $\pm$ 0.01 & 15.07 $\pm$ 0.03 & 14.57 $\pm$ 0.02 \\
61555030 & 101.876 & -2.3355 & (26,17,17) & 0.29017 & 0.39 & 0.31 & 0.28 & ew & 16.64 $\pm$ 0.02 & 16.06 $\pm$ 0.02 & 15.49 $\pm$ 0.02 \\
61606027 & 102.442 & -2.0182 & (24,16,17) & 0.42088 & 0.44 & 0.46 & 0.37 & ew & 15.62 $\pm$ 0.01 & 15.16 $\pm$ 0.03 & 14.62 $\pm$ 0.02 \\
61659198 & 103.002 & -2.3817 & (20,18,18) & 0.37092 & 0.22 & 0.24 & 0.26 & ew & 17.19 $\pm$ 0.02 & 16.71 $\pm$ 0.02 & 15.89 $\pm$ 0.02 \\
70132189 & 106.257 & -2.3889 & (17,16,14) & 1.83196 & 0.33 & 0.50 & 0.43 & ea & 16.38 $\pm$ 0.01 & 16.07 $\pm$ 0.02 & 15.56 $\pm$ 0.02 \\
70262674 & 107.423 & -2.2028 & (17,13,15) & 0.39542 & 0.43 & 0.41 & 0.62 & ew & 17.27 $\pm$ 0.02 & 16.67 $\pm$ 0.02 & 16.11 $\pm$ 0.03 \\
70272265 & 107.509 & -2.0670 & (19,10,11) & 0.41992 & 0.63 & 0.54 & 0.56 & ew & 16.36 $\pm$ 0.01 & 15.99 $\pm$ 0.02 & 15.46 $\pm$ 0.02 \\
70303323 & 107.793 & -2.0415 & (24,12,14) & 0.29662 & 0.35 & 0.26 & 0.30 & ew & 16.08 $\pm$ 0.01 & 15.59 $\pm$ 0.02 & 14.99 $\pm$ 0.02 \\
70317213 & 107.919 & -2.1804 & (25,17,14) & 0.26695 & 0.55 & 0.47 & 0.46 & ew & 17.31 $\pm$ 0.02 & 16.87 $\pm$ 0.02 & 16.36 $\pm$ 0.03 \\
70490735 & 109.439 & -1.9861 & (21,15,15) & 0.45273 & 0.32 & 0.27 & 0.37 & ew & 16.30 $\pm$ 0.01 & 16.24 $\pm$ 0.02 & 15.57 $\pm$ 0.02 \\
70497958 & 109.501 & -2.4001 & (19,10,15) & 1.10743 & 0.32 & 0.25 & 0.22 & ew & 15.02 $\pm$ 0.01 & 14.82 $\pm$ 0.03 & 14.69 $\pm$ 0.02 \\
70505376 & 109.565 & -2.1408 & (26,14,0) & 0.38116 & 0.66 & 0.58 & 0.0 & ew & 15.97 $\pm$ 0.01 & 15.58 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
70562794 & 110.048 & -2.1618 & (25,17,0) & 0.45472 & 0.31 & 0.30 & 0.0 & ew & 14.77 $\pm$ 0.01 & 14.65 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
70579650 & 110.185 & -2.1817 & (23,22,11) & 1.46909 & 0.21 & 0.29 & 0.25 & ew & 16.04 $\pm$ 0.01 & 15.64 $\pm$ 0.02 & 15.30 $\pm$ 0.02 \\
70620174 & 110.496 & -2.2400 & (25,13,12) & 0.31206 & 0.36 & 0.27 & 0.30 & ew & 16.03 $\pm$ 0.01 & 15.70 $\pm$ 0.02 & 15.27 $\pm$ 0.02 \\
70654019 & 110.770 & -2.0787 & (28,19,17) & 0.29561 & 0.3 & 0.30 & 0.26 & ew & 16.07 $\pm$ 0.01 & 15.80 $\pm$ 0.02 & 15.35 $\pm$ 0.02 \\
70876485 & 112.627 & -2.0718 & (27,12,10) & 0.43420 & 0.45 & 0.38 & 0.43 & ew & 14.12 $\pm$ 0.01 & 14.10 $\pm$ 0.03 & 13.72 $\pm$ 0.02 \\
70905977 & 112.867 & -2.0972 & (24,22,12) & 0.23265 & 0.42 & 0.42 & 0.38 & ew & 17.63 $\pm$ 0.03 & 17.09 $\pm$ 0.02 & 16.50 $\pm$ 0.03 \\
70988368 & 113.525 & -2.0204 & (26,26,10) & 11.2152 & 0.42 & 0.34 & 0.27 & ea & 17.29 $\pm$ 0.02 & 16.92 $\pm$ 0.02 & 16.51 $\pm$ 0.03 \\
71014867 & 113.747 & -1.9728 & (26,26,4) & 0.38604 & 0.52 & 0.50 & 0.35 & ew & 17.60 $\pm$ 0.03 & 17.24 $\pm$ 0.02 & 16.97 $\pm$ 0.04 \\
71139917 & 114.839 & -2.1704 & (30,20,0) & 1.98594 & 0.37 & 0.34 & 0.0 & ea & 15.21 $\pm$ 0.01 & 14.85 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
71150616 & 114.933 & -1.9399 & (20,26,17) & 0.37425 & 0.33 & 0.33 & 0.33 & ew & 16.61 $\pm$ 0.02 & 16.13 $\pm$ 0.02 & 15.66 $\pm$ 0.02 \\
71152329 & 114.948 & -2.0336 & (19,24,19) & 0.29003 & 0.40 & 0.48 & 0.46 & ew & 18.37 $\pm$ 0.05 & 17.91 $\pm$ 0.04 & 17.43 $\pm$ 0.04 \\
71181780 & 115.196 & -1.9467 & (28,26,20) & 0.32188 & 0.47 & 0.45 & 0.45 & ew & 16.47 $\pm$ 0.02 & 15.96 $\pm$ 0.02 & 15.46 $\pm$ 0.02 \\
71208098 & 115.417 & -2.0987 & (38,26,17) & 0.37302 & 0.27 & 0.22 & 0.27 & ew & 17.07 $\pm$ 0.02 & 16.75 $\pm$ 0.02 & 16.14 $\pm$ 0.03 \\
71227790 & 115.577 & -2.1245 & (36,32,9) & 0.48080 & 0.34 & 0.33 & 0.56 & ew & 15.16 $\pm$ 0.01 & 14.81 $\pm$ 0.03 & 14.40 $\pm$ 0.02 \\
71228914 & 115.585 & -2.3022 & (28,20,14) & 0.37092 & 0.29 & 0.26 & 0.25 & ew & 14.09 $\pm$ 0.01 & 13.79 $\pm$ 0.04 & 13.59 $\pm$ 0.02 \\
71234225 & 115.627 & -1.9341 & (21,28,0) & 0.80036 & 0.36 & 0.35 & 0.0 & ew & 15.33 $\pm$ 0.01 & 15.07 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
71243211 & 115.698 & -2.1433 & (36,25,0) & 0.45126 & 0.53 & 0.48 & 0.0 & eb & 14.79 $\pm$ 0.01 & 14.53 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
71298766 & 116.187 & -2.2541 & (32,24,23) & 0.37168 & 0.50 & 0.42 & 0.36 & ew & 17.06 $\pm$ 0.02 & 16.51 $\pm$ 0.02 & 15.89 $\pm$ 0.02 \\
71314286 & 116.346 & -2.2052 & (28,31,21) & 3.56385 & 0.76 & 0.50 & 0.69 & ea & 15.44 $\pm$ 0.01 & 15.13 $\pm$ 0.03 & 14.81 $\pm$ 0.02 \\
71318120 & 116.386 & -2.0585 & (29,23,20) & 0.32235 & 0.64 & 0.77 & 0.68 & ew & 15.65 $\pm$ 0.01 & 15.21 $\pm$ 0.03 & 14.69 $\pm$ 0.02 \\
71357499 & 116.791 & -1.9784 & (30,26,21) & 1.20937 & 0.42 & 0.39 & 0.38 & ew & 15.53 $\pm$ 0.01 & 15.29 $\pm$ 0.02 & 15.00 $\pm$ 0.02 \\
71372920 & 116.956 & -2.1005 & (34,23,22) & 0.51758 & 0.36 & 0.28 & 0.24 & ew & 14.35 $\pm$ 0.01 & 14.36 $\pm$ 0.03 & 13.95 $\pm$ 0.02 \\
71384517 & 117.082 & -2.2529 & (28,19,22) & 0.31755 & 0.44 & 0.37 & 0.39 & ew & 16.46 $\pm$ 0.02 & 16.15 $\pm$ 0.02 & 15.79 $\pm$ 0.02 \\
71415977 & 117.423 & -2.3172 & (30,26,17) & 1.01433 & 0.15 & 0.28 & 0.37 & ea & 15.11 $\pm$ 0.01 & 14.78 $\pm$ 0.03 & 14.51 $\pm$ 0.02 \\
71423027 & 117.498 & -2.1382 & (29,30,17) & 0.25508 & 0.54 & 0.46 & 0.74 & ew & 16.66 $\pm$ 0.02 & 16.32 $\pm$ 0.02 & 15.93 $\pm$ 0.02 \\
71449300 & 117.789 & -2.3209 & (24,24,23) & 0.40611 & 0.33 & 0.30 & 0.64 & ew & 16.57 $\pm$ 0.02 & 16.43 $\pm$ 0.02 & 15.84 $\pm$ 0.02 \\
71457194 & 117.876 & -2.0333 & (35,35,22) & 0.30946 & 0.30 & 0.27 & 0.22 & ew & 14.76 $\pm$ 0.01 & 14.43 $\pm$ 0.03 & 14.29 $\pm$ 0.02 \\
71536438 & 118.768 & -2.3822 & (23,12,24) & 0.28432 & 0.28 & 0.27 & 0.24 & ew & 16.06 $\pm$ 0.01 & 15.69 $\pm$ 0.02 & 15.37 $\pm$ 0.02 \\
71545993 & 118.873 & -2.2003 & (27,31,18) & 0.32725 & 0.83 & 0.72 & 2.22 & eb & 16.91 $\pm$ 0.02 & 16.53 $\pm$ 0.02 & 16.16 $\pm$ 0.03 \\
71566129 & 119.102 & -1.9949 & (32,39,17) & 0.37487 & 0.20 & 0.21 & 0.21 & ew & 14.95 $\pm$ 0.01 & 14.60 $\pm$ 0.03 & 14.26 $\pm$ 0.02 \\
71599767 & 119.513 & -2.0996 & (35,25,12) & 0.54154 & 0.61 & 0.56 & 0.30 & ea & 17.12 $\pm$ 0.02 & 16.57 $\pm$ 0.02 & 15.95 $\pm$ 0.02 \\
71610884 & 119.651 & -2.2350 & (39,38,12) & 0.27173 & 0.68 & 0.68 & 0.54 & ew & 16.77 $\pm$ 0.02 & 16.21 $\pm$ 0.02 & 15.64 $\pm$ 0.02 \\
80312834 & 124.292 & -0.6457 & (23,31,0) & 0.69016 & 0.50 & 0.40 & 0.0 & ew & 16.65 $\pm$ 0.01 & 16.14 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80745967 & 132.840 & -0.9100 & (25,32,0) & 0.25718 & 0.52 & 0.48 & 0.0 & eb & 17.28 $\pm$ 0.02 & 16.31 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80815591 & 134.738 & -0.8390 & (24,28,0) & 0.28097 & 0.52 & 0.41 & 0.0 & ew & 17.28 $\pm$ 0.02 & 16.97 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
80129138 & 121.643 & -1.3196 & (21,32,0) & 0.37438 & 0.60 & 0.59 & 0.0 & ew & 16.52 $\pm$ 0.01 & 16.17 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80194618 & 122.538 & -1.3108 & (23,33,0) & 0.35212 & 0.82 & 0.75 & 0.0 & ew & 17.26 $\pm$ 0.02 & 16.81 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
80333393 & 124.615 & -1.3787 & (23,31,0) & 0.10048 & 0.26 & 0.22 & 0.0 & ew & 17.34 $\pm$ 0.02 & 17.20 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
80428018 & 126.219 & -1.5173 & (23,32,0) & 0.31221 & 0.59 & 0.48 & 0.0 & ew & 15.69 $\pm$ 0.01 & 15.34 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80492343 & 127.375 & -1.5634 & (24,28,0) & 2.02468 & 0.35 & 0.30 & 0.0 & ew & 15.16 $\pm$ 0.01 & 14.53 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80604817 & 129.610 & -1.4288 & (25,28,0) & 0.30815 & 0.27 & 0.30 & 0.0 & ew & 16.83 $\pm$ 0.02 & 16.47 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80727469 & 132.364 & -1.3935 & (23,34,0) & 0.24403 & 0.66 & 0.78 & 0.0 & ew & 17.82 $\pm$ 0.03 & 17.3 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
80010865 & 120.136 & -2.2126 & (47,39,21) & 0.41857 & 0.42 & 0.25 & 0.44 & ew & 16.00 $\pm$ 0.02 & 16.02 $\pm$ 0.02 & 15.62 $\pm$ 0.02 \\
80010915 & 120.137 & -2.3292 & (41,41,20) & 0.30155 & 0.79 & 0.73 & 0.50 & ew & 16.52 $\pm$ 0.02 & 16.11 $\pm$ 0.02 & 15.67 $\pm$ 0.02 \\
80055771 & 120.696 & -2.2677 & (49,35,23) & 0.42460 & 0.47 & 0.54 & 0.44 & ew & 15.77 $\pm$ 0.01 & 15.47 $\pm$ 0.02 & 15.16 $\pm$ 0.02 \\
80114061 & 121.444 & -1.9794 & (48,48,23) & 1.29415 & 0.60 & 0.64 & 0.45 & ew & 14.49 $\pm$ 0.01 & 14.32 $\pm$ 0.02 & 14.09 $\pm$ 0.01 \\
80213291 & 122.803 & -2.2612 & (45,47,20) & 0.37835 & 0.33 & 0.35 & 0.23 & ew & 17.39 $\pm$ 0.03 & 16.88 $\pm$ 0.02 & 16.45 $\pm$ 0.02 \\
80235224 & 123.119 & -2.0349 & (50,50,26) & 0.36126 & 0.87 & 0.78 & 0.76 & ew & 17.29 $\pm$ 0.03 & 16.81 $\pm$ 0.02 & 16.35 $\pm$ 0.02 \\
80281680 & 123.809 & -2.1105 & (54,56,17) & 0.38685 & 0.50 & 0.47 & 0.34 & ew & 14.57 $\pm$ 0.01 & 14.14 $\pm$ 0.02 & 13.78 $\pm$ 0.01 \\
80414589 & 125.986 & -2.4514 & (14,14,15) & 0.74089 & 0.31 & 0.31 & 0.34 & ew & 14.43 $\pm$ 0.01 & 14.22 $\pm$ 0.02 & 14.09 $\pm$ 0.01 \\
80494973 & 127.424 & -1.9940 & (54,58,22) & 0.48057 & 0.50 & 0.40 & 0.36 & ew & 15.70 $\pm$ 0.01 & 15.40 $\pm$ 0.02 & 15.44 $\pm$ 0.02 \\
80515127 & 127.811 & -1.8271 & (23,38,3) & 0.29940 & 0.32 & 0.30 & 0.22 & ew & 17.38 $\pm$ 0.03 & 17.15 $\pm$ 0.03 & 16.90 $\pm$ 0.03 \\
80565237 & 128.784 & -1.8638 & (24,38,2) & 1.06563 & 0.34 & 0.31 & 0.01 & ew & 17.49 $\pm$ 0.04 & 17.00 $\pm$ 0.02 & 16.61 $\pm$ 0.02 \\
80566476 & 128.808 & -2.1496 & (47,57,16) & 0.49667 & 0.68 & 0.63 & 0.16 & eb & 17.63 $\pm$ 0.04 & 17.06 $\pm$ 0.02 & 16.47 $\pm$ 0.02 \\
80592473 & 129.347 & -2.1502 & (51,54,14) & 0.31662 & 0.27 & 0.23 & 0.26 & ew & 14.43 $\pm$ 0.01 & 14.06 $\pm$ 0.02 & 13.71 $\pm$ 0.01 \\
80611793 & 129.762 & -2.1265 & (56,54,13) & 0.24309 & 0.27 & 0.30 & 0.36 & ew & 16.75 $\pm$ 0.02 & 16.29 $\pm$ 0.02 & 15.90 $\pm$ 0.02 \\
80632331 & 130.206 & -2.1143 & (54,50,15) & 0.25159 & 0.71 & 0.28 & 0.31 & ew & 15.46 $\pm$ 0.01 & 14.79 $\pm$ 0.02 & 14.25 $\pm$ 0.01 \\
80673891 & 131.077 & -2.1773 & (57,52,11) & 0.26225 & 0.25 & 0.43 & 0.20 & ew & 16.40 $\pm$ 0.02 & 16.00 $\pm$ 0.02 & 15.65 $\pm$ 0.02 \\
80679069 & 131.202 & -2.1272 & (50,56,10) & 0.23912 & 0.82 & 0.73 & 0.42 & ew & 16.63 $\pm$ 0.02 & 16.13 $\pm$ 0.02 & 15.71 $\pm$ 0.02 \\
80756751 & 133.130 & -2.1339 & (47,56,0) & 0.27496 & 0.62 & 0.54 & 0.0 & ew & 14.97 $\pm$ 0.01 & 14.48 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
80764204 & 133.328 & -1.8074 & (24,26,0) & 0.40583 & 0.28 & 0.25 & 0.0 & ew & 15.25 $\pm$ 0.01 & 15.12 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
80765662 & 133.367 & -1.7964 & (20,17,0) & 0.34299 & 0.43 & 0.39 & 0.0 & ew & 14.84 $\pm$ 0.01 & 14.48 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
40067341 & 64.5433 & -2.7742 & (34,42,54) & 0.31050 & 0.32 & 0.39 & 0.36 & ea & 15.54 $\pm$ 0.01 & 14.93 $\pm$ 0.01 & 14.36 $\pm$ 0.01 \\
40241503 & 70.5802 & -2.7546 & (38,46,0) & 1.11058 & 0.29 & 0.76 & 0.0 & ew & 15.87 $\pm$ 0.02 & 14.74 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
40389330 & 72.8285 & -2.8056 & (42,51,61) & 0.26819 & 0.25 & 0.20 & 0.18 & ew & 17.06 $\pm$ 0.03 & 16.52 $\pm$ 0.02 & 15.90 $\pm$ 0.02 \\
40454051 & 73.6359 & -2.9842 & (20,30,58) & 0.37267 & 0.43 & 0.42 & 0.43 & ew & 15.66 $\pm$ 0.01 & 15.36 $\pm$ 0.01 & 15.05 $\pm$ 0.02 \\
40047541 & 63.3737 & -3.2339 & (25,16,23) & 0.26327 & 0.30 & 0.27 & 0.23 & ew & 14.91 $\pm$ 0.01 & 14.45 $\pm$ 0.02 & 14.04 $\pm$ 0.01 \\
40235593 & 70.4690 & -3.3072 & (31,22,25) & 3.00691 & 0.36 & 0.31 & 0.19 & ew & 16.95 $\pm$ 0.02 & 16.17 $\pm$ 0.02 & 15.48 $\pm$ 0.01 \\
40341518 & 72.1737 & -3.1824 & (21,21,26) & 0.49317 & 0.31 & 0.29 & 0.31 & ew & 16.56 $\pm$ 0.02 & 16.47 $\pm$ 0.02 & 16.46 $\pm$ 0.02 \\
40500728 & 74.1848 & -3.1692 & (28,20,22) & 0.33335 & 0.46 & 0.39 & 0.43 & ew & 17.61 $\pm$ 0.03 & 17.17 $\pm$ 0.03 & 16.99 $\pm$ 0.04 \\
40264408 & 70.9889 & -4.1058 & (37,27,18) & 0.2378 & 0.36 & 0.50 & 0.29 & ew & 16.58 $\pm$ 0.02 & 15.91 $\pm$ 0.01 & 15.61 $\pm$ 0.01 \\
40369450 & 72.5637 & -3.8497 & (31,22,14) & 0.47258 & 0.44 & 0.40 & 0.41 & ew & 16.16 $\pm$ 0.02 & 15.81 $\pm$ 0.01 & 15.48 $\pm$ 0.01 \\
40497858 & 74.1517 & -3.7406 & (21,18,12) & 0.99497 & 0.50 & 0.55 & 0.28 & ew & 17.72 $\pm$ 0.04 & 17.49 $\pm$ 0.03 & 17.38 $\pm$ 0.04 \\
40521875 & 74.4315 & -3.8583 & (31,21,14) & 1.43695 & 0.38 & 0.39 & 0.37 & ea & 14.69 $\pm$ 0.01 & 14.43 $\pm$ 0.02 & 14.16 $\pm$ 0.01 \\
40547620 & 74.7322 & -3.8047 & (32,20,13) & 0.30555 & 0.65 & 0.45 & 0.43 & ew & 18.05 $\pm$ 0.06 & 17.54 $\pm$ 0.03 & 17.13 $\pm$ 0.03 \\
40563699 & 74.9217 & -3.7894 & (30,22,15) & 2.52282 & 0.42 & 0.26 & 0.11 & ea & 15.80 $\pm$ 0.02 & 15.49 $\pm$ 0.01 & 15.06 $\pm$ 0.01 \\
50319018 & 78.2170 & -2.6691 & (46,47,57) & 0.96376 & 0.37 & 0.36 & 0.34 & ea & 14.43 $\pm$ 0.01 & 14.30 $\pm$ 0.01 & 14.17 $\pm$ 0.01 \\
50444482 & 79.3568 & -2.9019 & (48,32,0) & 0.61633 & 0.50 & 0.37 & 0.0 & ew & 13.92 $\pm$ 0.01 & 13.47 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50493050 & 79.8131 & -2.9020 & (52,48,0) & 2.24806 & 0.27 & 0.22 & 0.0 & ew & 15.73 $\pm$ 0.01 & 14.62 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50552687 & 80.3576 & -2.7685 & (44,52,66) & 0.35663 & 0.39 & 0.37 & 0.38 & ew & 14.68 $\pm$ 0.01 & 14.17 $\pm$ 0.01 & 13.69 $\pm$ 0.02 \\
50574471 & 80.5550 & -2.7198 & (52,51,61) & 0.98489 & 0.48 & 0.41 & 0.55 & ew & 16.03 $\pm$ 0.02 & 15.63 $\pm$ 0.01 & 15.27 $\pm$ 0.02 \\
50742052 & 81.9414 & -2.7636 & (54,49,0) & 0.73283 & 0.44 & 0.32 & 0.0 & ew & 16.29 $\pm$ 0.02 & 15.25 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50758840 & 82.0747 & -2.5339 & (24,44,50) & 0.28699 & 0.39 & 0.48 & 0.41 & ew & 17.01 $\pm$ 0.03 & 16.38 $\pm$ 0.01 & 15.74 $\pm$ 0.02 \\
50759022 & 82.0761 & -2.8136 & (54,49,67) & 5.20771 & 0.30 & 0.32 & 0.30 & ea & 14.97 $\pm$ 0.01 & 14.56 $\pm$ 0.01 & 14.18 $\pm$ 0.01 \\
50822867 & 82.6046 & -2.5092 & (24,30,49) & 0.60706 & 0.23 & 0.28 & 0.21 & ew & 15.52 $\pm$ 0.01 & 15.02 $\pm$ 0.01 & 14.51 $\pm$ 0.02 \\
50846625 & 82.8032 & -2.6150 & (54,47,0) & 0.61631 & 0.56 & 0.43 & 0.0 & ew & 17.36 $\pm$ 0.04 & 17.03 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
50854807 & 82.8731 & -2.9403 & (48,34,0) & 4.37773 & 0.28 & 0.30 & 0.0 & ea & 14.99 $\pm$ 0.01 & 14.17 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50953170 & 83.7186 & -2.8897 & (58,44,0) & 1.19298 & 0.44 & 0.21 & 0.0 & ew & 16.39 $\pm$ 0.02 & 15.34 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
50988099 & 84.0078 & -2.8549 & (56,55,0) & 1.66351 & 0.39 & 0.35 & 0.0 & ew & 15.49 $\pm$ 0.01 & 14.47 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51023667 & 84.3080 & -2.7310 & (54,52,0) & 0.33845 & 0.76 & 0.68 & 0.0 & ew & 15.57 $\pm$ 0.01 & 14.86 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51239813 & 86.1585 & -2.8455 & (60,56,78) & 0.32324 & 0.29 & 0.25 & 0.46 & ew & 16.53 $\pm$ 0.02 & 15.64 $\pm$ 0.01 & 14.98 $\pm$ 0.02 \\
51390034 & 87.4357 & -2.9475 & (0,54,72) & 10.8635 & 0.0 & 0.24 & 0.52 & ea & 0.0 $\pm$ 0.0 & 18.40 $\pm$ 0.06 & 17.57 $\pm$ 0.06 \\
51433825 & 87.7708 & -2.7702 & (50,54,79) & 1.06220 & 0.23 & 0.33 & 0.23 & ew & 17.13 $\pm$ 0.03 & 16.36 $\pm$ 0.01 & 15.65 $\pm$ 0.02 \\
51483475 & 88.1627 & -2.8002 & (53,55,85) & 0.47803 & 0.64 & 0.58 & 0.65 & ew & 17.65 $\pm$ 0.05 & 17.04 $\pm$ 0.02 & 15.97 $\pm$ 0.02 \\
51499114 & 88.2886 & -2.7352 & (56,52,72) & 0.78834 & 0.43 & 0.49 & 0.66 & ew & 17.88 $\pm$ 0.06 & 17.37 $\pm$ 0.02 & 17.16 $\pm$ 0.04 \\
51506182 & 88.3452 & -2.9535 & (42,54,67) & 0.25662 & 0.49 & 0.60 & 0.54 & ew & 17.62 $\pm$ 0.05 & 16.62 $\pm$ 0.01 & 15.59 $\pm$ 0.02 \\
51510025 & 88.3752 & -2.6096 & (52,50,73) & 0.56751 & 0.58 & 0.49 & 0.50 & eb & 15.26 $\pm$ 0.01 & 14.62 $\pm$ 0.01 & 13.93 $\pm$ 0.01 \\
51671374 & 89.5749 & -2.7633 & (58,56,0) & 0.45031 & 0.87 & 0.87 & 0.0 & eb & 16.68 $\pm$ 0.02 & 15.96 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51677757 & 89.6162 & -2.7380 & (62,54,0) & 0.90373 & 0.60 & 0.46 & 0.0 & ew & 17.42 $\pm$ 0.04 & 16.79 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
50161894 & 76.7013 & -3.4605 & (22,19,12) & 5.31580 & 0.49 & 0.46 & 0.17 & ew & 15.82 $\pm$ 0.01 & 14.67 $\pm$ 0.01 & 13.41 $\pm$ 0.01 \\
50374754 & 78.7227 & -3.5480 & (23,17,29) & 0.26842 & 0.44 & 0.38 & 0.31 & ew & 17.48 $\pm$ 0.03 & 17.06 $\pm$ 0.02 & 16.71 $\pm$ 0.03 \\
50391066 & 78.8680 & -3.4166 & (31,22,29) & 0.29979 & 0.58 & 0.46 & 0.43 & ew & 15.24 $\pm$ 0.01 & 14.75 $\pm$ 0.01 & 14.32 $\pm$ 0.01 \\
50433609 & 79.2544 & -3.2573 & (29,21,26) & 0.31315 & 0.59 & 0.70 & 0.61 & ew & 17.71 $\pm$ 0.04 & 17.15 $\pm$ 0.03 & 16.63 $\pm$ 0.03 \\
50438838 & 79.3039 & -3.5867 & (31,21,28) & 0.35285 & 0.51 & 0.38 & 0.38 & ew & 16.51 $\pm$ 0.02 & 16.07 $\pm$ 0.01 & 15.60 $\pm$ 0.01 \\
50541136 & 80.2541 & -3.2934 & (32,22,27) & 7.08801 & 0.95 & 0.86 & 0.78 & ea & 14.46 $\pm$ 0.01 & 13.92 $\pm$ 0.01 & 13.40 $\pm$ 0.01 \\
50564011 & 80.4613 & -3.4466 & (26,23,30) & 0.53888 & 0.50 & 0.47 & 0.42 & ew & 16.22 $\pm$ 0.02 & 15.73 $\pm$ 0.01 & 15.26 $\pm$ 0.01 \\
50694000 & 81.5569 & -3.4794 & (32,24,28) & 0.30580 & 0.21 & 0.27 & 0.11 & ew & 14.78 $\pm$ 0.01 & 14.28 $\pm$ 0.01 & 13.93 $\pm$ 0.01 \\
50735395 & 81.8893 & -3.6233 & (32,25,24) & 0.34603 & 0.74 & 0.77 & 0.62 & ew & 16.87 $\pm$ 0.02 & 16.29 $\pm$ 0.02 & 15.83 $\pm$ 0.01 \\
50755709 & 82.0491 & -3.2297 & (33,20,28) & 2.24093 & 0.29 & 0.23 & 0.17 & eb & 16.85 $\pm$ 0.02 & 15.79 $\pm$ 0.01 & 14.37 $\pm$ 0.01 \\
50917935 & 83.4212 & -3.2244 & (33,24,34) & 0.47431 & 0.34 & 0.30 & 0.31 & ew & 16.74 $\pm$ 0.02 & 16.24 $\pm$ 0.01 & 15.65 $\pm$ 0.01 \\
51000045 & 84.1088 & -3.2318 & (30,21,0) & 1.66799 & 0.42 & 0.32 & 0.0 & ew & 14.69 $\pm$ 0.01 & 14.03 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51102994 & 84.9721 & -3.4780 & (34,24,37) & 0.50124 & 0.70 & 0.56 & 0.59 & ew & 17.86 $\pm$ 0.04 & 17.23 $\pm$ 0.03 & 16.70 $\pm$ 0.03 \\
51156545 & 85.4430 & -3.1251 & (20,17,27) & 0.23638 & 0.79 & 0.77 & 0.77 & eb & 18.03 $\pm$ 0.05 & 16.88 $\pm$ 0.02 & 15.66 $\pm$ 0.01 \\
51211698 & 85.9183 & -3.4108 & (35,24,33) & 11.1791 & 0.82 & 0.71 & 0.70 & ew & 16.06 $\pm$ 0.01 & 15.19 $\pm$ 0.01 & 14.35 $\pm$ 0.01 \\
51293974 & 86.6310 & -3.2914 & (35,20,21) & 7.45376 & 0.56 & 0.52 & 0.22 & ew & 15.73 $\pm$ 0.01 & 14.64 $\pm$ 0.01 & 13.27 $\pm$ 0.01 \\
51357785 & 87.1829 & -3.5546 & (25,18,33) & 0.47701 & 0.82 & 0.66 & 0.71 & ea & 17.52 $\pm$ 0.03 & 16.72 $\pm$ 0.02 & 16.03 $\pm$ 0.02 \\
51406238 & 87.5576 & -3.3068 & (35,24,35) & 0.29611 & 0.29 & 0.31 & 0.26 & ew & 16.99 $\pm$ 0.02 & 16.47 $\pm$ 0.02 & 15.77 $\pm$ 0.01 \\
51439080 & 87.8110 & -3.5862 & (34,21,31) & 0.44614 & 0.59 & 0.64 & 0.53 & eb & 16.95 $\pm$ 0.02 & 16.44 $\pm$ 0.02 & 15.98 $\pm$ 0.02 \\
51450376 & 87.8984 & -3.3741 & (32,23,33) & 0.33454 & 0.73 & 0.40 & 0.44 & ew & 18.12 $\pm$ 0.05 & 17.43 $\pm$ 0.03 & 16.72 $\pm$ 0.03 \\
51467049 & 88.0293 & -3.4898 & (31,25,37) & 1.06584 & 0.75 & 0.70 & 0.83 & ew & 16.20 $\pm$ 0.02 & 15.55 $\pm$ 0.01 & 14.91 $\pm$ 0.01 \\
51530564 & 88.5402 & -3.2893 & (37,20,23) & 0.32067 & 0.39 & 0.39 & 0.32 & ew & 18.11 $\pm$ 0.05 & 17.18 $\pm$ 0.03 & 16.67 $\pm$ 0.03 \\
51564755 & 88.8118 & -3.3802 & (0,21,35) & 0.41068 & 0.0 & 0.53 & 0.66 & ew & 0.0 $\pm$ 0.0 & 18.31 $\pm$ 0.06 & 17.44 $\pm$ 0.05 \\
51619018 & 89.2213 & -3.3763 & (33,23,36) & 0.48992 & 0.58 & 0.53 & 0.60 & ew & 18.46 $\pm$ 0.06 & 17.76 $\pm$ 0.04 & 17.03 $\pm$ 0.03 \\
51631101 & 89.3073 & -3.2232 & (33,24,36) & 0.3117 & 0.70 & 0.37 & 0.35 & ew & 17.56 $\pm$ 0.03 & 16.97 $\pm$ 0.02 & 15.87 $\pm$ 0.01 \\
51694867 & 89.7261 & -3.4115 & (36,23,34) & 1.55161 & 0.55 & 0.66 & 0.55 & ew & 18.26 $\pm$ 0.06 & 17.84 $\pm$ 0.04 & 17.45 $\pm$ 0.05 \\
51721519 & 89.8971 & -3.4195 & (32,22,32) & 0.27403 & 0.74 & 0.85 & 0.77 & ew & 18.27 $\pm$ 0.06 & 17.59 $\pm$ 0.03 & 16.89 $\pm$ 0.03 \\
51728781 & 89.9422 & -3.2426 & (36,24,37) & 0.36286 & 0.52 & 0.50 & 0.49 & ew & 16.15 $\pm$ 0.02 & 15.84 $\pm$ 0.01 & 14.73 $\pm$ 0.01 \\
50424100 & 79.1718 & -3.9427 & (46,26,24) & 0.62314 & 0.37 & 0.24 & 0.28 & ew & 16.02 $\pm$ 0.02 & 15.92 $\pm$ 0.01 & 15.32 $\pm$ 0.01 \\
50571898 & 80.5376 & -4.1641 & (36,25,26) & 10.7861 & 0.21 & 0.20 & 0.13 & ew & 16.14 $\pm$ 0.02 & 15.53 $\pm$ 0.01 & 14.96 $\pm$ 0.01 \\
50576660 & 80.5799 & -4.1615 & (37,29,25) & 1.81425 & 0.31 & 0.54 & 0.25 & ew & 16.07 $\pm$ 0.02 & 15.09 $\pm$ 0.01 & 13.91 $\pm$ 0.01 \\
50607615 & 80.8495 & -4.1461 & (41,27,24) & 0.34856 & 0.65 & 0.46 & 0.47 & ew & 18.32 $\pm$ 0.07 & 17.89 $\pm$ 0.04 & 17.44 $\pm$ 0.05 \\
50765586 & 82.1337 & -4.1187 & (51,30,28) & 4.64812 & 0.34 & 0.36 & 0.37 & ew & 15.66 $\pm$ 0.02 & 14.51 $\pm$ 0.01 & 13.54 $\pm$ 0.01 \\
50848444 & 82.8250 & -4.1121 & (54,31,29) & 4.21510 & 0.26 & 0.23 & 0.11 & ew & 16.79 $\pm$ 0.03 & 15.66 $\pm$ 0.01 & 14.29 $\pm$ 0.01 \\
50887780 & 83.1638 & -3.8950 & (42,20,0) & 12.2920 & 0.27 & 0.31 & 0.0 & ew & 14.93 $\pm$ 0.02 & 14.06 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
50969201 & 83.8572 & -4.0922 & (52,29,0) & 10.6965 & 0.31 & 0.33 & 0.0 & ew & 15.46 $\pm$ 0.02 & 14.34 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51022720 & 84.3070 & -4.0168 & (58,31,28) & 2.28257 & 0.46 & 0.41 & 0.23 & ew & 15.60 $\pm$ 0.02 & 14.68 $\pm$ 0.01 & 13.57 $\pm$ 0.01 \\
51083382 & 84.8139 & -3.8989 & (42,22,0) & 3.33639 & 0.43 & 0.48 & 0.0 & ew & 17.46 $\pm$ 0.04 & 16.33 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
51085303 & 84.8298 & -4.0153 & (57,28,29) & 0.30464 & 0.80 & 0.68 & 0.62 & ew & 15.84 $\pm$ 0.02 & 14.97 $\pm$ 0.01 & 14.17 $\pm$ 0.01 \\
51112128 & 85.0576 & -4.0034 & (59,25,28) & 0.59045 & 0.58 & 0.46 & 0.44 & ea & 16.05 $\pm$ 0.02 & 15.14 $\pm$ 0.01 & 14.17 $\pm$ 0.01 \\
51178734 & 85.6469 & -3.7810 & (34,22,16) & 0.39264 & 0.83 & 0.55 & 0.47 & ew & 18.05 $\pm$ 0.06 & 17.32 $\pm$ 0.03 & 16.54 $\pm$ 0.02 \\
51184530 & 85.6960 & -4.0167 & (60,29,25) & 0.72476 & 0.41 & 0.27 & 0.26 & ew & 17.97 $\pm$ 0.06 & 17.29 $\pm$ 0.03 & 16.71 $\pm$ 0.03 \\
51325825 & 86.9223 & -4.0266 & (57,20,17) & 0.47701 & 0.46 & 0.39 & 0.39 & ew & 17.62 $\pm$ 0.04 & 16.97 $\pm$ 0.02 & 16.31 $\pm$ 0.02 \\
51345608 & 87.0922 & -3.8568 & (34,22,18) & 0.28025 & 0.61 & 0.46 & 0.36 & ew & 17.5 $\pm$ 0.04 & 16.85 $\pm$ 0.02 & 16.23 $\pm$ 0.02 \\
51355304 & 87.1706 & -3.9907 & (59,30,30) & 9.19473 & 0.71 & 0.52 & 0.63 & ea & 16.81 $\pm$ 0.03 & 16.10 $\pm$ 0.01 & 15.44 $\pm$ 0.01 \\
51512684 & 88.4045 & -4.1728 & (37,25,24) & 0.26660 & 0.33 & 0.23 & 0.20 & ew & 17.23 $\pm$ 0.03 & 16.63 $\pm$ 0.02 & 15.93 $\pm$ 0.01 \\
51512884 & 88.4062 & -4.0148 & (59,29,24) & 2.05032 & 0.54 & 0.42 & 0.42 & ea & 17.53 $\pm$ 0.04 & 16.95 $\pm$ 0.02 & 16.39 $\pm$ 0.02 \\
51529378 & 88.5389 & -3.7556 & (27,18,13) & 0.35436 & 0.62 & 0.36 & 0.43 & ew & 17.52 $\pm$ 0.04 & 16.68 $\pm$ 0.02 & 15.88 $\pm$ 0.01 \\
51546167 & 88.6755 & -4.2268 & (40,24,24) & 0.31742 & 0.41 & 0.37 & 0.36 & ew & 16.49 $\pm$ 0.03 & 15.86 $\pm$ 0.01 & 15.30 $\pm$ 0.01 \\
51576398 & 88.9082 & -4.0818 & (59,29,28) & 0.64861 & 0.45 & 0.32 & 0.39 & eb & 16.65 $\pm$ 0.03 & 15.96 $\pm$ 0.01 & 15.26 $\pm$ 0.01 \\
51609449 & 89.1589 & -4.0582 & (61,28,32) & 0.38599 & 0.54 & 0.47 & 0.44 & ew & 15.89 $\pm$ 0.02 & 15.13 $\pm$ 0.01 & 14.40 $\pm$ 0.01 \\
51653590 & 89.4665 & -4.0828 & (59,28,29) & 0.29775 & 0.55 & 0.49 & 0.58 & ew & 16.21 $\pm$ 0.02 & 15.58 $\pm$ 0.01 & 14.99 $\pm$ 0.01 \\
51655119 & 89.4768 & -3.7889 & (33,21,16) & 0.26100 & 1.08 & 0.66 & 0.52 & ew & 18.03 $\pm$ 0.06 & 17.21 $\pm$ 0.02 & 16.35 $\pm$ 0.02 \\
60017637 & 90.1560 & -2.6325 & (57,40,0) & 0.90424 & 0.50 & 0.44 & 0.0 & ew & 15.41 $\pm$ 0.02 & 15.25 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
60072822 & 90.5822 & -2.7790 & (36,48,76) & 0.84299 & 0.39 & 0.39 & 0.36 & ew & 17.91 $\pm$ 0.05 & 17.07 $\pm$ 0.02 & 16.76 $\pm$ 0.03 \\
60119819 & 90.9326 & -2.7274 & (40,47,0) & 0.30271 & 0.27 & 0.26 & 0.0 & ew & 16.95 $\pm$ 0.03 & 16.24 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
60224749 & 91.6741 & -2.9281 & (55,41,68) & 0.27462 & 0.32 & 0.30 & 0.29 & ew & 16.12 $\pm$ 0.02 & 15.53 $\pm$ 0.01 & 14.91 $\pm$ 0.02 \\
60295349 & 92.1872 & -2.9643 & (48,40,0) & 0.74753 & 0.43 & 0.47 & 0.0 & eb & 16.31 $\pm$ 0.03 & 16.07 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
60297615 & 92.2042 & -2.8389 & (43,49,76) & 3.2003 & 0.46 & 0.54 & 0.55 & ea & 18.01 $\pm$ 0.06 & 17.54 $\pm$ 0.02 & 16.97 $\pm$ 0.03 \\
60329340 & 92.4390 & -2.7395 & (48,47,0) & 0.85495 & 0.40 & 0.35 & 0.0 & ew & 17.69 $\pm$ 0.05 & 17.29 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
60366679 & 92.7102 & -2.7901 & (60,48,76) & 5.55545 & 0.60 & 0.50 & 0.46 & ea & 15.19 $\pm$ 0.02 & 14.89 $\pm$ 0.01 & 14.48 $\pm$ 0.02 \\
60370784 & 92.7395 & -2.8426 & (59,48,0) & 0.41010 & 0.38 & 0.32 & 0.0 & ew & 15.00 $\pm$ 0.03 & 14.79 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
60380892 & 92.8107 & -2.7479 & (49,46,76) & 3.58558 & 0.37 & 0.31 & 0.33 & ea & 17.33 $\pm$ 0.04 & 16.94 $\pm$ 0.02 & 16.46 $\pm$ 0.02 \\
60435934 & 93.1973 & -2.8699 & (55,46,62) & 0.43039 & 0.25 & 0.21 & 0.19 & ew & 16.96 $\pm$ 0.03 & 16.56 $\pm$ 0.01 & 15.92 $\pm$ 0.02 \\
60459931 & 93.3660 & -2.6181 & (56,54,64) & 14.5866 & 0.37 & 0.37 & 0.42 & ew & 15.11 $\pm$ 0.03 & 14.88 $\pm$ 0.01 & 14.59 $\pm$ 0.02 \\
60480101 & 93.5067 & -2.7011 & (61,41,73) & 0.36719 & 0.35 & 0.28 & 0.28 & ew & 16.01 $\pm$ 0.02 & 15.43 $\pm$ 0.01 & 14.98 $\pm$ 0.02 \\
60491174 & 93.5943 & -2.9427 & (0,42,71) & 0.18440 & 0.0 & 0.36 & 0.49 & ew & 0.0 $\pm$ 0.0 & 18.27 $\pm$ 0.04 & 17.39 $\pm$ 0.04 \\
60513217 & 93.7641 & -2.9245 & (0,46,60) & 0.32716 & 0.0 & 0.77 & 0.55 & ew & 0.0 $\pm$ 0.0 & 18.17 $\pm$ 0.04 & 17.61 $\pm$ 0.04 \\
60513409 & 93.7656 & -2.9070 & (51,48,62) & 0.70887 & 0.54 & 0.44 & 0.46 & eb & 17.10 $\pm$ 0.04 & 16.75 $\pm$ 0.01 & 16.36 $\pm$ 0.02 \\
60554813 & 94.0838 & -2.7384 & (61,46,0) & 1.01708 & 0.34 & 0.34 & 0.0 & eb & 14.92 $\pm$ 0.03 & 14.68 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
60560682 & 94.1268 & -2.7267 & (51,43,72) & 0.31222 & 0.44 & 0.36 & 0.41 & ew & 17.87 $\pm$ 0.05 & 17.10 $\pm$ 0.02 & 16.50 $\pm$ 0.02 \\
60569420 & 94.1911 & -2.6968 & (63,36,0) & 0.26831 & 0.31 & 0.27 & 0.0 & ew & 15.50 $\pm$ 0.02 & 14.70 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
60591098 & 94.3479 & -2.6340 & (59,46,79) & 0.26852 & 0.69 & 0.56 & 0.54 & ew & 16.27 $\pm$ 0.03 & 15.82 $\pm$ 0.01 & 15.32 $\pm$ 0.02 \\
60664317 & 94.8754 & -2.6954 & (28,36,55) & 0.32228 & 0.43 & 0.34 & 0.32 & ew & 18.26 $\pm$ 0.06 & 17.80 $\pm$ 0.03 & 17.08 $\pm$ 0.03 \\
60719304 & 95.3045 & -2.9148 & (51,40,46) & 0.28325 & 0.68 & 0.53 & 0.59 & ew & 16.61 $\pm$ 0.03 & 16.12 $\pm$ 0.01 & 15.59 $\pm$ 0.02 \\
60775693 & 95.7417 & -2.9904 & (0,50,61) & 0.27568 & 0.0 & 0.38 & 0.29 & ew & 0.0 $\pm$ 0.0 & 17.20 $\pm$ 0.02 & 16.59 $\pm$ 0.02 \\
60802230 & 95.9469 & -3.0570 & (0,38,42) & 0.27664 & 0.0 & 0.87 & 0.87 & eb & 0.0 $\pm$ 0.0 & 18.03 $\pm$ 0.03 & 17.35 $\pm$ 0.04 \\
60804160 & 95.9624 & -2.8718 & (67,48,0) & 0.52223 & 0.42 & 0.33 & 0.0 & ew & 14.57 $\pm$ 0.03 & 14.15 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
60821816 & 96.0974 & -2.7857 & (46,46,0) & 0.37872 & 0.46 & 0.34 & 0.0 & ew & 17.78 $\pm$ 0.05 & 17.28 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
60837186 & 96.2118 & -2.7612 & (38,48,60) & 0.39127 & 0.56 & 0.60 & 0.57 & ew & 17.70 $\pm$ 0.05 & 17.35 $\pm$ 0.02 & 17.33 $\pm$ 0.04 \\
60841609 & 96.2452 & -2.7525 & (49,53,67) & 7.41442 & 0.66 & 0.57 & 0.4 & ea & 17.12 $\pm$ 0.04 & 16.51 $\pm$ 0.01 & 15.82 $\pm$ 0.02 \\
60903920 & 96.7208 & -2.8863 & (44,42,65) & 4.43029 & 0.44 & 0.65 & 0.66 & ea & 17.70 $\pm$ 0.05 & 16.94 $\pm$ 0.02 & 16.04 $\pm$ 0.02 \\
60933741 & 96.9548 & -2.6362 & (20,50,48) & 0.51079 & 0.38 & 0.51 & 0.51 & eb & 18.85 $\pm$ 0.08 & 18.30 $\pm$ 0.04 & 17.72 $\pm$ 0.05 \\
60966592 & 97.2082 & -2.7247 & (48,49,72) & 0.30283 & 0.35 & 0.40 & 0.45 & ew & 17.51 $\pm$ 0.04 & 17.27 $\pm$ 0.02 & 16.69 $\pm$ 0.02 \\
61048121 & 97.8150 & -2.6892 & (64,36,74) & 0.34082 & 0.37 & 0.34 & 0.32 & ew & 17.18 $\pm$ 0.04 & 16.59 $\pm$ 0.01 & 15.96 $\pm$ 0.02 \\
61053723 & 97.8555 & -2.9581 & (0,36,56) & 0.95515 & 0.0 & 0.38 & 0.43 & ea & 0.0 $\pm$ 0.0 & 17.88 $\pm$ 0.03 & 17.01 $\pm$ 0.03 \\
61083328 & 98.0706 & -2.8106 & (50,45,55) & 0.26002 & 0.33 & 0.26 & 0.26 & ew & 17.40 $\pm$ 0.04 & 16.69 $\pm$ 0.01 & 16.08 $\pm$ 0.02 \\
61092308 & 98.1372 & -2.7690 & (61,46,74) & 0.29686 & 0.28 & 0.24 & 0.26 & ew & 16.20 $\pm$ 0.03 & 15.58 $\pm$ 0.01 & 14.93 $\pm$ 0.02 \\
61108996 & 98.2700 & -2.5861 & (30,42,64) & 0.45146 & 0.39 & 0.29 & 0.33 & ew & 18.46 $\pm$ 0.07 & 17.59 $\pm$ 0.02 & 16.79 $\pm$ 0.03 \\
61112913 & 98.3008 & -2.6326 & (56,44,77) & 0.44714 & 0.34 & 0.29 & 0.23 & ew & 16.09 $\pm$ 0.02 & 15.49 $\pm$ 0.01 & 14.83 $\pm$ 0.02 \\
61167067 & 98.7398 & -2.5973 & (28,40,56) & 0.35885 & 0.35 & 0.35 & 0.45 & ew & 18.14 $\pm$ 0.06 & 17.59 $\pm$ 0.02 & 16.84 $\pm$ 0.03 \\
61189183 & 98.9172 & -2.7977 & (55,32,0) & 0.43391 & 0.32 & 0.28 & 0.0 & ew & 15.81 $\pm$ 0.02 & 15.17 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
61227177 & 99.2247 & -2.9424 & (48,51,60) & 5.21212 & 0.28 & 0.33 & 0.38 & ea & 17.6 $\pm$ 0.05 & 16.95 $\pm$ 0.02 & 16.15 $\pm$ 0.02 \\
61307463 & 99.8211 & -2.7279 & (64,45,0) & 0.26461 & 0.47 & 0.40 & 0.0 & ew & 16.00 $\pm$ 0.02 & 15.39 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
61335836 & 100.032 & -2.8168 & (55,48,0) & 1.95053 & 0.55 & 0.41 & 0.0 & ea & 17.05 $\pm$ 0.04 & 16.39 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
61335952 & 100.032 & -2.9132 & (58,41,68) & 0.25775 & 0.48 & 0.4 & 0.43 & ew & 16.54 $\pm$ 0.03 & 16.29 $\pm$ 0.01 & 15.35 $\pm$ 0.02 \\
61375658 & 100.335 & -2.6442 & (58,39,0) & 0.81518 & 0.34 & 0.32 & 0.0 & ea & 14.67 $\pm$ 0.03 & 14.24 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
61468783 & 101.033 & -2.9970 & (30,47,58) & 0.45937 & 0.46 & 0.44 & 0.44 & ew & 15.80 $\pm$ 0.02 & 15.34 $\pm$ 0.01 & 14.84 $\pm$ 0.02 \\
61475060 & 101.090 & -2.6798 & (60,42,0) & 0.35044 & 0.61 & 0.54 & 0.0 & ew & 15.06 $\pm$ 0.03 & 14.61 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
61478638 & 101.124 & -2.9028 & (61,52,66) & 0.85397 & 0.31 & 0.27 & 0.29 & ea & 16.33 $\pm$ 0.03 & 15.71 $\pm$ 0.01 & 14.94 $\pm$ 0.02 \\
61480393 & 101.141 & -2.6846 & (60,48,0) & 0.30478 & 1.08 & 0.88 & 0.0 & ea & 16.43 $\pm$ 0.03 & 15.78 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
61486876 & 101.203 & -2.9622 & (52,38,68) & 0.26245 & 0.78 & 0.54 & 0.53 & ew & 15.87 $\pm$ 0.02 & 15.05 $\pm$ 0.01 & 14.27 $\pm$ 0.02 \\
61511310 & 101.441 & -2.8094 & (56,51,70) & 0.32054 & 0.32 & 0.31 & 0.37 & ew & 16.08 $\pm$ 0.02 & 15.54 $\pm$ 0.01 & 14.96 $\pm$ 0.02 \\
61515576 & 101.483 & -2.8424 & (52,48,63) & 6.47969 & 0.3 & 0.24 & 0.23 & ew & 17.43 $\pm$ 0.04 & 16.70 $\pm$ 0.01 & 15.82 $\pm$ 0.02 \\
61530130 & 101.624 & -2.8503 & (49,51,0) & 0.81489 & 0.60 & 0.68 & 0.0 & eb & 17.50 $\pm$ 0.04 & 16.77 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
61539748 & 101.718 & -2.7935 & (58,0,66) & 4.65358 & 0.85 & 0.0 & 0.72 & ea & 16.66 $\pm$ 0.03 & 0.0 $\pm$ 0.0 & 15.57 $\pm$ 0.02 \\
61540609 & 101.727 & -2.8410 & (50,43,64) & 1.01619 & 0.38 & 0.31 & 0.28 & ea & 17.38 $\pm$ 0.04 & 16.71 $\pm$ 0.01 & 15.85 $\pm$ 0.02 \\
61550342 & 101.827 & -2.7556 & (50,48,68) & 0.32822 & 0.43 & 0.60 & 0.53 & ew & 17.63 $\pm$ 0.05 & 17.02 $\pm$ 0.02 & 16.30 $\pm$ 0.02 \\
61553439 & 101.860 & -2.9009 & (68,45,55) & 0.32255 & 0.40 & 0.33 & 0.36 & ew & 15.91 $\pm$ 0.02 & 15.43 $\pm$ 0.01 & 14.90 $\pm$ 0.02 \\
61560000 & 101.930 & -2.8325 & (63,0,66) & 0.26772 & 0.38 & 0.0 & 0.38 & ew & 16.84 $\pm$ 0.03 & 0.0 $\pm$ 0.0 & 15.31 $\pm$ 0.02 \\
61566644 & 102.006 & -2.8533 & (56,38,60) & 2.48713 & 0.77 & 0.39 & 0.43 & ea & 17.51 $\pm$ 0.04 & 16.95 $\pm$ 0.02 & 16.11 $\pm$ 0.02 \\
61641601 & 102.816 & -2.7468 & (51,38,52) & 0.14121 & 0.80 & 0.48 & 0.45 & ew & 17.62 $\pm$ 0.05 & 16.78 $\pm$ 0.01 & 16.50 $\pm$ 0.02 \\
61651384 & 102.920 & -2.8920 & (45,36,0) & 0.28955 & 0.77 & 0.81 & 0.0 & ew & 17.61 $\pm$ 0.05 & 16.87 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
61660487 & 103.015 & -2.7529 & (52,43,66) & 0.61497 & 0.25 & 0.28 & 0.33 & ew & 17.86 $\pm$ 0.05 & 17.46 $\pm$ 0.02 & 16.89 $\pm$ 0.03 \\
61671372 & 103.127 & -2.7187 & (34,32,48) & 0.72839 & 0.57 & 0.36 & 0.44 & ew & 18.02 $\pm$ 0.06 & 17.59 $\pm$ 0.02 & 16.98 $\pm$ 0.03 \\
61683143 & 103.250 & -2.8700 & (56,38,0) & 1.17437 & 0.56 & 0.52 & 0.0 & ea & 16.50 $\pm$ 0.03 & 15.93 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
61692729 & 103.347 & -2.6144 & (54,38,64) & 1.02451 & 0.46 & 0.43 & 0.49 & ew & 16.75 $\pm$ 0.03 & 16.17 $\pm$ 0.01 & 15.50 $\pm$ 0.02 \\
61712578 & 103.552 & -2.9446 & (58,46,62) & 3.64994 & 0.43 & 0.35 & 0.41 & ea & 15.24 $\pm$ 0.02 & 14.93 $\pm$ 0.01 & 14.56 $\pm$ 0.02 \\
61712985 & 103.556 & -2.7776 & (52,40,61) & 0.06724 & 0.23 & 0.19 & 0.20 & ew & 15.29 $\pm$ 0.02 & 14.92 $\pm$ 0.01 & 14.56 $\pm$ 0.02 \\
61715472 & 103.581 & -2.9888 & (32,42,37) & 0.30049 & 0.64 & 0.73 & 0.64 & eb & 15.43 $\pm$ 0.02 & 14.91 $\pm$ 0.01 & 14.38 $\pm$ 0.02 \\
61716523 & 103.593 & -2.7140 & (40,42,42) & 1.03272 & 0.41 & 0.41 & 0.40 & ew & 18.06 $\pm$ 0.06 & 17.47 $\pm$ 0.02 & 16.73 $\pm$ 0.02 \\
61776745 & 104.226 & -2.8044 & (57,41,64) & 0.38178 & 0.25 & 0.20 & 0.18 & ew & 17.52 $\pm$ 0.04 & 16.73 $\pm$ 0.01 & 15.61 $\pm$ 0.02 \\
61826939 & 104.761 & -2.8287 & (65,50,64) & 3.00418 & 0.50 & 0.38 & 0.40 & ea & 16.31 $\pm$ 0.03 & 15.85 $\pm$ 0.01 & 15.20 $\pm$ 0.02 \\
60011880 & 90.1075 & -3.6062 & (34,26,27) & 0.54048 & 0.30 & 0.27 & 0.25 & ew & 16.68 $\pm$ 0.02 & 16.24 $\pm$ 0.02 & 15.62 $\pm$ 0.02 \\
60014726 & 90.1313 & -3.6283 & (33,0,31) & 0.43349 & 0.55 & 0.0 & 0.36 & ew & 17.07 $\pm$ 0.03 & 0.0 $\pm$ 0.0 & 16.14 $\pm$ 0.02 \\
60046150 & 90.3781 & -3.2324 & (37,25,37) & 0.43239 & 0.69 & 0.87 & 0.58 & ew & 16.98 $\pm$ 0.02 & 16.48 $\pm$ 0.02 & 15.79 $\pm$ 0.02 \\
60088657 & 90.7016 & -3.5406 & (19,18,33) & 9.10690 & 0.47 & 0.30 & 0.29 & ew & 18.6 $\pm$ 0.06 & 17.62 $\pm$ 0.03 & 16.61 $\pm$ 0.03 \\
60114297 & 90.8923 & -3.4151 & (23,23,34) & 0.45841 & 0.35 & 0.26 & 0.26 & ew & 17.20 $\pm$ 0.03 & 16.82 $\pm$ 0.02 & 16.21 $\pm$ 0.02 \\
60158615 & 91.2125 & -3.1427 & (20,15,24) & 0.38518 & 0.54 & 0.42 & 0.59 & ew & 16.85 $\pm$ 0.02 & 16.33 $\pm$ 0.02 & 15.74 $\pm$ 0.02 \\
60173598 & 91.3220 & -3.3360 & (28,20,32) & 0.97852 & 0.77 & 0.59 & 0.73 & ea & 17.47 $\pm$ 0.03 & 17.06 $\pm$ 0.02 & 16.49 $\pm$ 0.03 \\
60202242 & 91.5200 & -3.4039 & (30,23,30) & 0.33341 & 0.75 & 0.67 & 0.61 & ew & 16.34 $\pm$ 0.02 & 15.93 $\pm$ 0.02 & 15.38 $\pm$ 0.02 \\
60247571 & 91.8375 & -3.6493 & (24,18,29) & 0.38824 & 0.67 & 0.5 & 0.58 & ew & 17.83 $\pm$ 0.04 & 17.30 $\pm$ 0.02 & 17.02 $\pm$ 0.04 \\
60397311 & 92.9257 & -3.3301 & (21,19,26) & 0.98839 & 0.36 & 0.30 & 0.35 & ew & 17.30 $\pm$ 0.03 & 16.96 $\pm$ 0.02 & 16.47 $\pm$ 0.03 \\
60401014 & 92.9517 & -3.4630 & (23,22,0) & 0.31741 & 0.39 & 0.40 & 0.0 & ew & 17.19 $\pm$ 0.03 & 16.63 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
60402034 & 92.9593 & -3.6013 & (23,20,35) & 2.30995 & 0.52 & 0.82 & 0.64 & ea & 17.95 $\pm$ 0.04 & 17.62 $\pm$ 0.03 & 17.08 $\pm$ 0.04 \\
60466996 & 93.4142 & -3.3559 & (32,20,33) & 0.12007 & 0.37 & 0.18 & 0.25 & ew & 18.10 $\pm$ 0.04 & 17.70 $\pm$ 0.03 & 17.16 $\pm$ 0.04 \\
60484905 & 93.5450 & -3.5778 & (0,18,30) & 0.28133 & 0.0 & 0.58 & 0.62 & ew & 0.0 $\pm$ 0.0 & 18.07 $\pm$ 0.04 & 17.27 $\pm$ 0.04 \\
60540857 & 93.9780 & -3.3030 & (31,21,29) & 0.34302 & 0.37 & 0.34 & 0.32 & ew & 16.93 $\pm$ 0.02 & 16.6 $\pm$ 0.02 & 16.12 $\pm$ 0.02 \\
60550505 & 94.0515 & -3.2927 & (22,22,31) & 0.34271 & 0.66 & 0.60 & 0.61 & ew & 18.53 $\pm$ 0.06 & 18.10 $\pm$ 0.04 & 17.89 $\pm$ 0.06 \\
60552882 & 94.0696 & -3.5262 & (21,19,32) & 0.56076 & 0.22 & 0.26 & 0.22 & ew & 16.26 $\pm$ 0.02 & 15.87 $\pm$ 0.02 & 15.39 $\pm$ 0.02 \\
60592656 & 94.3589 & -3.3455 & (28,22,28) & 0.50749 & 0.57 & 0.50 & 0.56 & ew & 17.90 $\pm$ 0.04 & 17.89 $\pm$ 0.04 & 16.96 $\pm$ 0.03 \\
60642104 & 94.7022 & -3.4049 & (27,22,0) & 0.62203 & 0.30 & 0.30 & 0.0 & ew & 15.71 $\pm$ 0.02 & 15.46 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
60681685 & 95.0088 & -3.1727 & (22,16,25) & 0.43209 & 0.34 & 0.32 & 0.28 & ew & 16.53 $\pm$ 0.02 & 16.18 $\pm$ 0.02 & 15.83 $\pm$ 0.02 \\
60735103 & 95.4277 & -3.4093 & (30,23,31) & 0.34462 & 0.25 & 0.24 & 0.23 & ew & 16.03 $\pm$ 0.02 & 15.70 $\pm$ 0.02 & 15.25 $\pm$ 0.02 \\
60741714 & 95.4779 & -3.5861 & (20,18,30) & 0.24193 & 0.82 & 0.75 & 0.67 & ew & 18.08 $\pm$ 0.04 & 17.31 $\pm$ 0.02 & 16.46 $\pm$ 0.03 \\
60761893 & 95.6354 & -3.4040 & (22,15,28) & 0.43039 & 0.62 & 0.64 & 0.58 & ew & 14.83 $\pm$ 0.02 & 14.50 $\pm$ 0.02 & 14.07 $\pm$ 0.03 \\
60776011 & 95.7441 & -3.4482 & (23,22,24) & 0.28073 & 0.52 & 0.37 & 0.41 & ew & 18.06 $\pm$ 0.04 & 17.66 $\pm$ 0.03 & 17.11 $\pm$ 0.04 \\
60781071 & 95.7822 & -3.3513 & (21,0,26) & 0.26841 & 0.62 & 0.0 & 0.58 & ew & 18.64 $\pm$ 0.06 & 0.0 $\pm$ 0.0 & 17.16 $\pm$ 0.04 \\
60097703 & 90.7695 & -3.9064 & (30,17,18) & 0.378 & 0.34 & 0.35 & 0.43 & ew & 15.74 $\pm$ 0.02 & 15.15 $\pm$ 0.03 & 14.41 $\pm$ 0.02 \\
60212701 & 91.5910 & -3.9883 & (47,0,16) & 9.45237 & 0.21 & 0.0 & 0.20 & ew & 15.19 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 13.5 $\pm$ 0.02 \\
60248515 & 91.8444 & -4.1746 & (23,0,23) & 0.44814 & 0.47 & 0.0 & 0.53 & ew & 18.28 $\pm$ 0.05 & 0.0 $\pm$ 0.0 & 16.96 $\pm$ 0.03 \\
60262701 & 91.9505 & -3.9961 & (37,16,21) & 0.43743 & 0.59 & 0.50 & 0.49 & ew & 17.10 $\pm$ 0.02 & 16.50 $\pm$ 0.02 & 15.88 $\pm$ 0.02 \\
60278487 & 92.0644 & -4.1327 & (35,19,23) & 0.22120 & 0.57 & 0.42 & 0.61 & ew & 18.71 $\pm$ 0.07 & 17.69 $\pm$ 0.03 & 16.97 $\pm$ 0.03 \\
60420907 & 93.0910 & -3.9417 & (44,19,21) & 0.37643 & 0.35 & 0.27 & 0.31 & ew & 17.07 $\pm$ 0.02 & 16.55 $\pm$ 0.02 & 15.93 $\pm$ 0.02 \\
60611514 & 94.4900 & -4.0175 & (44,21,17) & 0.35738 & 0.44 & 0.33 & 0.32 & ew & 17.22 $\pm$ 0.03 & 16.58 $\pm$ 0.02 & 16.03 $\pm$ 0.02 \\
60631894 & 94.6279 & -3.8779 & (27,16,17) & 0.70750 & 0.27 & 0.23 & 0.24 & ew & 16.04 $\pm$ 0.02 & 15.65 $\pm$ 0.03 & 15.18 $\pm$ 0.02 \\
60651901 & 94.7787 & -4.0052 & (38,20,19) & 0.40578 & 0.5 & 0.42 & 0.34 & ew & 17.80 $\pm$ 0.04 & 17.28 $\pm$ 0.03 & 16.74 $\pm$ 0.03 \\
60654122 & 94.7967 & -4.0566 & (37,23,19) & 0.2546 & 0.27 & 0.20 & 0.28 & ew & 17.66 $\pm$ 0.03 & 16.91 $\pm$ 0.02 & 16.26 $\pm$ 0.02 \\
60665770 & 94.8866 & -3.8812 & (29,16,15) & 0.44881 & 0.40 & 0.41 & 0.36 & ew & 15.73 $\pm$ 0.02 & 15.32 $\pm$ 0.03 & 14.81 $\pm$ 0.02 \\
60672124 & 94.9360 & -4.0216 & (39,18,18) & 0.35721 & 0.34 & 0.35 & 0.21 & ew & 15.44 $\pm$ 0.02 & 15.08 $\pm$ 0.03 & 14.64 $\pm$ 0.02 \\
60700766 & 95.1588 & -4.0841 & (40,23,23) & 0.32920 & 0.37 & 0.31 & 0.35 & ew & 17.95 $\pm$ 0.04 & 17.48 $\pm$ 0.03 & 16.98 $\pm$ 0.03 \\
60717970 & 95.2940 & -3.7889 & (28,17,13) & 0.10529 & 0.49 & 0.55 & 0.47 & ea & 16.73 $\pm$ 0.02 & 16.38 $\pm$ 0.02 & 16.14 $\pm$ 0.02 \\
60965944 & 97.2033 & -4.0784 & (44,0,13) & 0.46621 & 0.42 & 0.0 & 0.30 & ew & 17.17 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 16.53 $\pm$ 0.03 \\
61013543 & 97.5626 & -4.1413 & (45,21,19) & 0.36779 & 0.48 & 0.37 & 0.38 & eb & 17.29 $\pm$ 0.03 & 16.79 $\pm$ 0.02 & 16.25 $\pm$ 0.02 \\
61025492 & 97.6502 & -4.1911 & (28,16,0) & 0.37533 & 0.24 & 0.23 & 0.0 & ew & 16.33 $\pm$ 0.02 & 15.97 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
61042899 & 97.7770 & -4.2621 & (31,20,10) & 0.25458 & 0.47 & 0.52 & 0.55 & ew & 17.81 $\pm$ 0.04 & 17.26 $\pm$ 0.03 & 16.65 $\pm$ 0.03 \\
61055651 & 97.8695 & -3.9014 & (35,19,8) & 5.93673 & 0.45 & 0.27 & 0.10 & ew & 17.45 $\pm$ 0.03 & 16.14 $\pm$ 0.02 & 14.62 $\pm$ 0.02 \\
61109630 & 98.2750 & -3.7815 & (15,0,14) & 0.32270 & 0.83 & 0.0 & 0.61 & ew & 18.47 $\pm$ 0.06 & 0.0 $\pm$ 0.0 & 17.11 $\pm$ 0.03 \\
61141620 & 98.5345 & -4.1777 & (27,21,21) & 0.51382 & 0.60 & 0.61 & 0.55 & ea & 16.62 $\pm$ 0.02 & 16.14 $\pm$ 0.02 & 15.58 $\pm$ 0.02 \\
61164869 & 98.7219 & -3.8845 & (32,14,16) & 1.76492 & 1.04 & 0.94 & 0.47 & ea & 17.46 $\pm$ 0.03 & 16.86 $\pm$ 0.02 & 16.19 $\pm$ 0.02 \\
61220882 & 99.1737 & -4.0833 & (40,19,20) & 0.29637 & 0.50 & 0.21 & 0.21 & ew & 16.32 $\pm$ 0.02 & 15.66 $\pm$ 0.03 & 15.06 $\pm$ 0.02 \\
61236426 & 99.2977 & -4.2014 & (27,18,14) & 0.32269 & 0.42 & 0.32 & 0.32 & ew & 18.14 $\pm$ 0.05 & 17.21 $\pm$ 0.03 & 16.42 $\pm$ 0.03 \\
61306352 & 99.8132 & -4.2148 & (24,0,22) & 0.05465 & 0.23 & 0.0 & 0.51 & ea & 15.90 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 14.10 $\pm$ 0.02 \\
61345014 & 100.100 & -4.2157 & (22,18,23) & 0.04998 & 0.36 & 0.10 & 0.68 & ea & 15.68 $\pm$ 0.02 & 15.14 $\pm$ 0.03 & 14.57 $\pm$ 0.02 \\
61380005 & 100.368 & -3.8672 & (32,15,16) & 0.33823 & 0.85 & 0.78 & 0.77 & ew & 17.01 $\pm$ 0.02 & 16.45 $\pm$ 0.02 & 15.8 $\pm$ 0.02 \\
61460683 & 100.971 & -4.0175 & (42,23,17) & 0.31261 & 0.58 & 0.53 & 0.42 & ew & 17.0 $\pm$ 0.02 & 16.43 $\pm$ 0.02 & 15.74 $\pm$ 0.02 \\
61509099 & 101.420 & -4.2054 & (27,19,0) & 3.54293 & 0.75 & 0.61 & 0.0 & ea & 16.81 $\pm$ 0.02 & 16.33 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
61513519 & 101.463 & -3.9161 & (40,24,24) & 0.41299 & 0.31 & 0.30 & 0.23 & ew & 15.60 $\pm$ 0.02 & 14.99 $\pm$ 0.03 & 14.52 $\pm$ 0.02 \\
61539618 & 101.717 & -4.2107 & (26,0,17) & 0.04368 & 0.36 & 0.0 & 0.44 & ea & 15.08 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 14.11 $\pm$ 0.02 \\
61638109 & 102.779 & -3.9859 & (43,22,16) & 0.24005 & 0.42 & 0.38 & 0.43 & ew & 16.43 $\pm$ 0.02 & 15.99 $\pm$ 0.02 & 15.36 $\pm$ 0.02 \\
61643917 & 102.842 & -3.9011 & (39,0,13) & 0.39341 & 0.73 & 0.0 & 0.52 & ew & 14.02 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 13.35 $\pm$ 0.02 \\
61668053 & 103.092 & -4.0197 & (48,19,17) & 0.64134 & 0.35 & 0.36 & 0.26 & ew & 15.38 $\pm$ 0.02 & 15.05 $\pm$ 0.03 & 14.42 $\pm$ 0.02 \\
61711244 & 103.539 & -4.0011 & (43,0,14) & 1.95932 & 0.33 & 0.0 & 0.26 & ew & 15.43 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 13.47 $\pm$ 0.02 \\
61714460 & 103.571 & -3.7708 & (27,10,0) & 0.36096 & 0.27 & 0.20 & 0.0 & ew & 17.18 $\pm$ 0.03 & 16.60 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
61736597 & 103.802 & -3.9867 & (29,21,16) & 0.40813 & 0.40 & 0.55 & 0.34 & ew & 16.21 $\pm$ 0.02 & 15.71 $\pm$ 0.03 & 15.00 $\pm$ 0.02 \\
61791046 & 104.382 & -4.1027 & (39,21,0) & 0.31420 & 0.27 & 0.22 & 0.0 & ew & 17.66 $\pm$ 0.03 & 17.09 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
61816191 & 104.646 & -3.9616 & (45,20,15) & 0.59197 & 0.45 & 0.47 & 0.49 & eb & 16.90 $\pm$ 0.02 & 16.23 $\pm$ 0.02 & 15.46 $\pm$ 0.02 \\
61824736 & 104.737 & -4.0830 & (42,14,16) & 2.31641 & 0.64 & 0.09 & 0.33 & eb & 17.52 $\pm$ 0.03 & 16.90 $\pm$ 0.02 & 16.10 $\pm$ 0.02 \\
70002761 & 105.028 & -2.6365 & (46,53,58) & 2.83188 & 0.44 & 0.35 & 0.29 & ea & 16.51 $\pm$ 0.03 & 16.03 $\pm$ 0.01 & 15.39 $\pm$ 0.02 \\
70048565 & 105.482 & -2.6064 & (46,36,52) & 1.45348 & 0.47 & 0.43 & 0.42 & ea & 15.66 $\pm$ 0.02 & 15.21 $\pm$ 0.01 & 14.62 $\pm$ 0.02 \\
70051967 & 105.516 & -2.9833 & (0,45,57) & 0.52319 & 0.0 & 0.43 & 0.47 & ew & 0.0 $\pm$ 0.0 & 14.75 $\pm$ 0.01 & 14.41 $\pm$ 0.02 \\
70101485 & 105.977 & -2.6644 & (56,41,0) & 0.80217 & 0.53 & 0.43 & 0.0 & eb & 16.94 $\pm$ 0.03 & 16.50 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
70130383 & 106.241 & -2.9575 & (39,23,20) & 0.42856 & 0.46 & 0.38 & 0.45 & ew & 16.81 $\pm$ 0.03 & 16.40 $\pm$ 0.01 & 15.93 $\pm$ 0.02 \\
70178179 & 106.672 & -2.9444 & (53,47,55) & 0.37064 & 0.57 & 0.43 & 0.48 & ew & 16.02 $\pm$ 0.02 & 15.55 $\pm$ 0.01 & 15.03 $\pm$ 0.02 \\
70231591 & 107.145 & -2.8422 & (40,49,64) & 0.24549 & 0.44 & 0.43 & 0.41 & ew & 17.99 $\pm$ 0.05 & 17.48 $\pm$ 0.02 & 16.86 $\pm$ 0.03 \\
70290149 & 107.674 & -2.7959 & (40,40,45) & 0.24540 & 0.66 & 0.45 & 0.37 & ew & 17.25 $\pm$ 0.04 & 16.32 $\pm$ 0.01 & 15.65 $\pm$ 0.02 \\
70297750 & 107.743 & -2.8388 & (50,41,49) & 0.34433 & 0.61 & 0.34 & 0.41 & ew & 16.93 $\pm$ 0.03 & 16.50 $\pm$ 0.01 & 16.02 $\pm$ 0.02 \\
70333532 & 108.068 & -2.8602 & (42,41,51) & 0.37300 & 0.63 & 0.50 & 0.59 & ew & 17.31 $\pm$ 0.04 & 17.01 $\pm$ 0.02 & 16.62 $\pm$ 0.02 \\
70333768 & 108.070 & -2.5935 & (22,36,41) & 0.28084 & 0.47 & 0.37 & 0.38 & ew & 18.22 $\pm$ 0.06 & 17.77 $\pm$ 0.03 & 17.49 $\pm$ 0.04 \\
70334393 & 108.076 & -2.8048 & (64,53,66) & 0.42906 & 0.37 & 0.24 & 0.29 & ew & 15.41 $\pm$ 0.02 & 15.18 $\pm$ 0.01 & 14.92 $\pm$ 0.02 \\
70371343 & 108.406 & -2.7290 & (56,41,57) & 0.42004 & 0.49 & 0.59 & 0.65 & ew & 16.66 $\pm$ 0.03 & 16.04 $\pm$ 0.01 & 15.42 $\pm$ 0.02 \\
70377017 & 108.454 & -2.8773 & (56,40,65) & 0.45483 & 0.25 & 0.22 & 0.24 & ew & 16.04 $\pm$ 0.02 & 15.91 $\pm$ 0.01 & 15.36 $\pm$ 0.02 \\
70425900 & 108.865 & -2.7557 & (36,47,0) & 0.99158 & 0.51 & 0.40 & 0.0 & ea & 17.47 $\pm$ 0.04 & 17.04 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
70428264 & 108.886 & -3.0153 & (0,34,55) & 0.35258 & 0.0 & 0.25 & 0.29 & ew & 0.0 $\pm$ 0.0 & 17.08 $\pm$ 0.02 & 16.70 $\pm$ 0.02 \\
70448091 & 109.062 & -2.8282 & (40,43,64) & 0.27382 & 0.58 & 0.42 & 0.49 & ew & 17.81 $\pm$ 0.05 & 17.46 $\pm$ 0.02 & 17.07 $\pm$ 0.03 \\
70461527 & 109.181 & -2.7534 & (46,45,64) & 0.25950 & 0.50 & 0.54 & 0.40 & ew & 17.36 $\pm$ 0.04 & 16.93 $\pm$ 0.02 & 16.42 $\pm$ 0.02 \\
70563368 & 110.053 & -2.7080 & (58,45,61) & 0.34927 & 0.43 & 0.43 & 0.45 & ew & 15.71 $\pm$ 0.02 & 15.32 $\pm$ 0.01 & 14.89 $\pm$ 0.02 \\
70572340 & 110.126 & -2.7489 & (56,32,0) & 0.38358 & 0.43 & 0.35 & 0.0 & ew & 14.77 $\pm$ 0.03 & 14.32 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
70603168 & 110.368 & -2.6437 & (36,37,52) & 0.38124 & 0.29 & 0.26 & 0.26 & ew & 16.89 $\pm$ 0.03 & 16.36 $\pm$ 0.01 & 16.20 $\pm$ 0.02 \\
70620484 & 110.499 & -2.6259 & (51,38,0) & 0.45412 & 0.55 & 0.56 & 0.0 & eb & 15.95 $\pm$ 0.02 & 15.64 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
70633021 & 110.599 & -2.6663 & (48,33,49) & 0.52763 & 0.51 & 0.48 & 0.43 & eb & 14.72 $\pm$ 0.03 & 14.53 $\pm$ 0.01 & 14.33 $\pm$ 0.02 \\
70713373 & 111.234 & -2.5817 & (0,30,52) & 0.27587 & 0.0 & 0.23 & 0.46 & ea & 0.0 $\pm$ 0.0 & 13.99 $\pm$ 0.01 & 13.73 $\pm$ 0.02 \\
70718602 & 111.274 & -2.5749 & (37,36,0) & 1.51943 & 0.23 & 0.45 & 0.0 & ea & 15.12 $\pm$ 0.02 & 14.69 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
70730862 & 111.370 & -2.8498 & (50,46,71) & 0.29525 & 0.65 & 0.49 & 0.48 & ew & 17.19 $\pm$ 0.04 & 16.77 $\pm$ 0.01 & 16.15 $\pm$ 0.02 \\
70740960 & 111.456 & -2.9561 & (49,37,59) & 0.26030 & 0.56 & 0.57 & 0.58 & ew & 16.42 $\pm$ 0.03 & 16.08 $\pm$ 0.01 & 15.74 $\pm$ 0.02 \\
70754332 & 111.570 & -2.6975 & (0,47,59) & 0.95276 & 0.0 & 0.48 & 0.48 & ew & 0.0 $\pm$ 0.0 & 17.21 $\pm$ 0.02 & 16.82 $\pm$ 0.03 \\
70785245 & 111.839 & -2.9356 & (0,49,67) & 0.97811 & 0.0 & 0.43 & 0.44 & ew & 0.0 $\pm$ 0.0 & 16.09 $\pm$ 0.01 & 15.76 $\pm$ 0.02 \\
70868871 & 112.565 & -2.8042 & (65,48,0) & 4.57738 & 0.46 & 0.37 & 0.0 & ea & 15.9 $\pm$ 0.02 & 15.79 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
70875026 & 112.615 & -2.5904 & (46,41,50) & 1.93089 & 0.54 & 0.49 & 0.49 & ea & 16.96 $\pm$ 0.03 & 16.37 $\pm$ 0.01 & 15.71 $\pm$ 0.02 \\
70927748 & 113.045 & -2.8347 & (65,41,72) & 0.49212 & 0.49 & 0.42 & 0.69 & ew & 15.05 $\pm$ 0.03 & 14.87 $\pm$ 0.01 & 14.65 $\pm$ 0.02 \\
70946906 & 113.196 & -2.8201 & (0,37,53) & 0.30866 & 0.0 & 0.42 & 0.44 & eb & 0.0 $\pm$ 0.0 & 18.59 $\pm$ 0.05 & 17.68 $\pm$ 0.05 \\
70973944 & 113.410 & -2.7986 & (52,45,77) & 12.9058 & 0.48 & 0.3 & 0.4 & ea & 15.18 $\pm$ 0.02 & 15.06 $\pm$ 0.01 & 14.85 $\pm$ 0.02 \\
70980474 & 113.461 & -2.8739 & (58,56,0) & 0.43257 & 0.21 & 0.20 & 0.0 & ew & 15.37 $\pm$ 0.02 & 15.06 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
71011490 & 113.719 & -2.5598 & (28,32,40) & 1.04406 & 0.49 & 0.57 & 0.59 & ea & 16.78 $\pm$ 0.03 & 16.37 $\pm$ 0.01 & 15.90 $\pm$ 0.02 \\
71013797 & 113.738 & -2.7118 & (60,39,69) & 0.39311 & 0.77 & 0.70 & 0.69 & ew & 15.73 $\pm$ 0.02 & 15.33 $\pm$ 0.01 & 14.93 $\pm$ 0.02 \\
71023753 & 113.820 & -2.9233 & (0,37,57) & 0.24893 & 0.0 & 0.34 & 0.34 & ew & 0.0 $\pm$ 0.0 & 18.01 $\pm$ 0.03 & 17.41 $\pm$ 0.04 \\
71033006 & 113.899 & -2.6703 & (66,39,0) & 0.35707 & 0.34 & 0.27 & 0.0 & ew & 16.01 $\pm$ 0.02 & 15.72 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
71078875 & 114.296 & -3.0086 & (0,43,55) & 0.25685 & 0.0 & 0.71 & 0.63 & ew & 0.0 $\pm$ 0.0 & 15.72 $\pm$ 0.01 & 15.23 $\pm$ 0.02 \\
71081142 & 114.317 & -2.9119 & (51,52,74) & 0.78154 & 0.54 & 0.51 & 0.48 & ea & 17.26 $\pm$ 0.04 & 16.91 $\pm$ 0.02 & 16.50 $\pm$ 0.02 \\
71093951 & 114.428 & -2.8997 & (60,47,57) & 0.34959 & 0.76 & 0.55 & 0.57 & ew & 17.18 $\pm$ 0.04 & 16.84 $\pm$ 0.02 & 16.39 $\pm$ 0.02 \\
71100448 & 114.487 & -2.8316 & (68,50,73) & 0.26288 & 0.37 & 0.30 & 0.24 & ew & 16.81 $\pm$ 0.03 & 16.43 $\pm$ 0.01 & 16.10 $\pm$ 0.02 \\
71128041 & 114.732 & -3.0319 & (0,34,37) & 0.45856 & 0.0 & 0.49 & 0.52 & ew & 0.0 $\pm$ 0.0 & 16.67 $\pm$ 0.01 & 16.22 $\pm$ 0.02 \\
71138851 & 114.829 & -2.7498 & (39,40,51) & 0.22710 & 0.27 & 0.29 & 0.32 & ew & 17.87 $\pm$ 0.05 & 17.26 $\pm$ 0.02 & 16.86 $\pm$ 0.03 \\
71158141 & 114.996 & -3.0586 & (30,45,51) & 2.65710 & 0.48 & 0.27 & 0.33 & ea & 17.00 $\pm$ 0.03 & 16.58 $\pm$ 0.01 & 16.01 $\pm$ 0.02 \\
71185719 & 115.230 & -2.5983 & (49,41,0) & 0.95440 & 0.40 & 0.39 & 0.0 & eb & 15.96 $\pm$ 0.02 & 15.69 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
71204513 & 115.387 & -2.7101 & (48,38,64) & 3.51610 & 0.97 & 0.61 & 0.59 & ea & 18.05 $\pm$ 0.06 & 17.83 $\pm$ 0.03 & 17.52 $\pm$ 0.04 \\
71262309 & 115.852 & -2.9139 & (0,40,67) & 0.35268 & 0.0 & 0.80 & 0.78 & eb & 0.0 $\pm$ 0.0 & 17.90 $\pm$ 0.03 & 17.28 $\pm$ 0.03 \\
71309187 & 116.292 & -2.6233 & (48,39,60) & 0.38893 & 0.75 & 0.67 & 0.71 & ew & 17.40 $\pm$ 0.04 & 16.99 $\pm$ 0.02 & 16.61 $\pm$ 0.02 \\
71313850 & 116.341 & -2.7441 & (0,31,46) & 0.32767 & 0.0 & 0.47 & 0.54 & ew & 0.0 $\pm$ 0.0 & 18.34 $\pm$ 0.04 & 17.66 $\pm$ 0.04 \\
71339978 & 116.615 & -2.8459 & (46,43,75) & 0.23760 & 0.36 & 0.27 & 0.30 & ew & 17.69 $\pm$ 0.05 & 17.27 $\pm$ 0.02 & 17.06 $\pm$ 0.03 \\
71389787 & 117.139 & -2.9570 & (49,40,74) & 0.33072 & 0.74 & 0.54 & 0.56 & ew & 16.15 $\pm$ 0.03 & 15.79 $\pm$ 0.01 & 15.35 $\pm$ 0.02 \\
71397317 & 117.219 & -2.8534 & (59,41,73) & 0.46811 & 0.22 & 0.25 & 0.22 & ew & 16.48 $\pm$ 0.03 & 16.06 $\pm$ 0.01 & 15.84 $\pm$ 0.02 \\
71399363 & 117.241 & -2.7714 & (50,52,70) & 0.73842 & 0.63 & 0.26 & 0.22 & ew & 17.46 $\pm$ 0.04 & 16.94 $\pm$ 0.02 & 16.54 $\pm$ 0.02 \\
71407469 & 117.330 & -2.5499 & (30,32,0) & 0.35983 & 0.21 & 0.25 & 0.0 & ew & 15.65 $\pm$ 0.02 & 15.45 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
71411770 & 117.377 & -2.7065 & (23,47,50) & 0.24814 & 0.35 & 0.51 & 0.40 & ew & 18.62 $\pm$ 0.08 & 18.13 $\pm$ 0.04 & 17.25 $\pm$ 0.03 \\
71450326 & 117.800 & -2.6749 & (59,41,71) & 0.44436 & 0.43 & 0.22 & 0.26 & ew & 16.90 $\pm$ 0.03 & 16.36 $\pm$ 0.01 & 15.95 $\pm$ 0.02 \\
71478339 & 118.111 & -2.7102 & (49,45,65) & 0.32844 & 0.64 & 0.52 & 0.57 & ew & 17.57 $\pm$ 0.04 & 17.22 $\pm$ 0.02 & 16.78 $\pm$ 0.03 \\
71486159 & 118.201 & -2.7323 & (45,45,66) & 9.61467 & 0.45 & 0.29 & 0.33 & ea & 17.53 $\pm$ 0.04 & 17.33 $\pm$ 0.02 & 17.00 $\pm$ 0.03 \\
71510626 & 118.484 & -2.8487 & (57,49,79) & 4.45074 & 0.69 & 0.66 & 0.64 & ea & 15.35 $\pm$ 0.02 & 15.36 $\pm$ 0.01 & 15.36 $\pm$ 0.02 \\
71527033 & 118.662 & -2.7875 & (53,39,66) & 0.31897 & 0.56 & 0.49 & 0.54 & ew & 15.81 $\pm$ 0.02 & 15.57 $\pm$ 0.01 & 15.24 $\pm$ 0.02 \\
71611980 & 119.664 & -2.8746 & (61,45,79) & 0.18685 & 0.49 & 0.41 & 0.46 & ew & 15.25 $\pm$ 0.02 & 14.61 $\pm$ 0.01 & 13.93 $\pm$ 0.02 \\
71616585 & 119.724 & -2.8542 & (60,43,67) & 0.35318 & 0.31 & 0.24 & 0.31 & ew & 15.87 $\pm$ 0.02 & 15.61 $\pm$ 0.01 & 15.31 $\pm$ 0.02 \\
70002139 & 105.022 & -3.1647 & (16,13,21) & 0.42902 & 0.67 & 0.65 & 0.68 & ew & 16.16 $\pm$ 0.02 & 15.76 $\pm$ 0.02 & 15.23 $\pm$ 0.02 \\
70043628 & 105.435 & -3.5284 & (25,20,30) & 0.67161 & 0.36 & 0.34 & 0.35 & ew & 16.64 $\pm$ 0.02 & 16.11 $\pm$ 0.02 & 15.72 $\pm$ 0.02 \\
70149246 & 106.409 & -3.4202 & (20,16,24) & 1.61785 & 0.27 & 0.29 & 0.25 & ew & 14.10 $\pm$ 0.02 & 13.82 $\pm$ 0.02 & 13.53 $\pm$ 0.03 \\
70159263 & 106.501 & -3.2578 & (20,18,24) & 0.41751 & 0.55 & 0.57 & 0.67 & ew & 15.53 $\pm$ 0.02 & 15.13 $\pm$ 0.02 & 14.34 $\pm$ 0.02 \\
70241207 & 107.232 & -3.3940 & (18,16,30) & 0.39061 & 0.44 & 0.46 & 0.42 & ew & 16.25 $\pm$ 0.02 & 15.84 $\pm$ 0.02 & 15.37 $\pm$ 0.02 \\
70241389 & 107.234 & -3.4815 & (19,19,26) & 0.21919 & 0.33 & 0.40 & 0.40 & ew & 14.87 $\pm$ 0.02 & 14.66 $\pm$ 0.02 & 14.31 $\pm$ 0.02 \\
70248059 & 107.293 & -3.3170 & (21,12,20) & 0.32821 & 0.43 & 0.37 & 0.37 & ew & 16.08 $\pm$ 0.02 & 15.29 $\pm$ 0.02 & 15.07 $\pm$ 0.02 \\
70274462 & 107.529 & -3.2348 & (24,13,28) & 0.25531 & 0.66 & 0.56 & 0.69 & ew & 15.05 $\pm$ 0.02 & 14.68 $\pm$ 0.02 & 14.26 $\pm$ 0.02 \\
70323941 & 107.980 & -3.2067 & (22,14,22) & 0.26446 & 0.62 & 0.51 & 0.60 & ew & 17.88 $\pm$ 0.04 & 17.52 $\pm$ 0.03 & 17.00 $\pm$ 0.03 \\
70335879 & 108.089 & -3.3419 & (31,13,20) & 0.77673 & 0.39 & 0.45 & 0.37 & ew & 14.90 $\pm$ 0.02 & 14.65 $\pm$ 0.02 & 14.30 $\pm$ 0.02 \\
70342037 & 108.147 & -3.2212 & (25,19,24) & 0.41922 & 0.69 & 0.59 & 0.55 & ew & 17.37 $\pm$ 0.03 & 16.83 $\pm$ 0.02 & 16.21 $\pm$ 0.02 \\
70367323 & 108.373 & -3.4857 & (26,17,32) & 0.44996 & 0.28 & 0.32 & 0.28 & ew & 15.81 $\pm$ 0.02 & 15.44 $\pm$ 0.02 & 14.98 $\pm$ 0.02 \\
70389594 & 108.562 & -3.3775 & (0,18,28) & 0.59429 & 0.0 & 0.37 & 0.39 & eb & 0.0 $\pm$ 0.0 & 16.01 $\pm$ 0.02 & 15.61 $\pm$ 0.02 \\
70390170 & 108.566 & -3.3928 & (28,19,29) & 0.43909 & 0.3 & 0.25 & 0.24 & ew & 15.70 $\pm$ 0.02 & 15.33 $\pm$ 0.02 & 14.88 $\pm$ 0.02 \\
70395839 & 108.615 & -3.1886 & (16,18,30) & 0.41558 & 0.47 & 0.39 & 0.36 & ew & 15.46 $\pm$ 0.02 & 15.30 $\pm$ 0.02 & 15.04 $\pm$ 0.02 \\
70409564 & 108.729 & -3.6319 & (19,17,21) & 0.73188 & 0.57 & 0.52 & 0.55 & ew & 14.38 $\pm$ 0.02 & 14.08 $\pm$ 0.02 & 14.18 $\pm$ 0.02 \\
70416159 & 108.783 & -3.5124 & (21,20,28) & 0.36148 & 0.21 & 0.25 & 0.24 & ew & 16.50 $\pm$ 0.02 & 16.13 $\pm$ 0.02 & 15.73 $\pm$ 0.02 \\
70429081 & 108.893 & -3.3991 & (27,11,28) & 0.45812 & 0.36 & 0.39 & 0.32 & ew & 17.09 $\pm$ 0.02 & 16.69 $\pm$ 0.02 & 16.25 $\pm$ 0.02 \\
70447962 & 109.061 & -3.4205 & (26,18,28) & 0.38487 & 0.33 & 0.30 & 0.31 & ew & 17.70 $\pm$ 0.03 & 17.32 $\pm$ 0.03 & 16.97 $\pm$ 0.03 \\
70449282 & 109.072 & -3.3014 & (17,14,26) & 0.38098 & 0.78 & 0.72 & 0.90 & ew & 16.85 $\pm$ 0.02 & 16.53 $\pm$ 0.02 & 16.05 $\pm$ 0.02 \\
70459019 & 109.160 & -3.2272 & (23,20,0) & 0.31647 & 0.53 & 0.37 & 0.0 & ew & 18.20 $\pm$ 0.05 & 17.45 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
70465916 & 109.219 & -3.5439 & (0,18,24) & 0.30740 & 0.0 & 0.33 & 0.35 & ew & 0.0 $\pm$ 0.0 & 18.13 $\pm$ 0.04 & 17.44 $\pm$ 0.04 \\
70481877 & 109.360 & -3.5536 & (17,21,32) & 3.92192 & 0.43 & 0.37 & 0.35 & ea & 15.04 $\pm$ 0.02 & 14.79 $\pm$ 0.02 & 14.42 $\pm$ 0.02 \\
70483947 & 109.378 & -3.1869 & (20,18,29) & 0.40170 & 0.47 & 0.47 & 0.52 & ea & 16.46 $\pm$ 0.02 & 16.14 $\pm$ 0.02 & 15.71 $\pm$ 0.02 \\
70487946 & 109.414 & -3.6471 & (23,17,25) & 0.49293 & 0.42 & 0.45 & 0.44 & ew & 14.82 $\pm$ 0.02 & 14.24 $\pm$ 0.02 & 14.20 $\pm$ 0.02 \\
70500702 & 109.525 & -3.51 & (25,22,32) & 0.44706 & 0.55 & 0.58 & 0.54 & ew & 17.53 $\pm$ 0.03 & 17.14 $\pm$ 0.02 & 16.66 $\pm$ 0.03 \\
70518196 & 109.673 & -3.4157 & (24,17,31) & 0.45082 & 0.40 & 0.33 & 0.40 & ew & 16.00 $\pm$ 0.02 & 15.64 $\pm$ 0.02 & 15.47 $\pm$ 0.02 \\
70552006 & 109.960 & -3.2445 & (21,18,23) & 0.41770 & 0.48 & 0.41 & 0.54 & ew & 18.01 $\pm$ 0.04 & 17.64 $\pm$ 0.03 & 17.16 $\pm$ 0.04 \\
70649841 & 110.735 & -3.4113 & (27,21,33) & 0.32488 & 0.74 & 0.51 & 0.68 & ew & 15.87 $\pm$ 0.02 & 15.42 $\pm$ 0.02 & 14.88 $\pm$ 0.02 \\
70659637 & 110.816 & -3.5825 & (23,18,23) & 0.28789 & 0.31 & 0.29 & 0.32 & ew & 17.20 $\pm$ 0.03 & 16.86 $\pm$ 0.02 & 16.66 $\pm$ 0.03 \\
70666682 & 110.869 & -3.5454 & (20,15,26) & 0.39276 & 0.37 & 0.37 & 0.40 & ew & 17.30 $\pm$ 0.03 & 17.01 $\pm$ 0.02 & 16.61 $\pm$ 0.03 \\
70681909 & 110.985 & -3.2767 & (28,18,27) & 0.47229 & 0.21 & 0.20 & 0.20 & ew & 15.83 $\pm$ 0.02 & 15.59 $\pm$ 0.02 & 15.19 $\pm$ 0.02 \\
70705855 & 111.175 & -3.3354 & (26,16,0) & 0.32809 & 0.25 & 0.24 & 0.0 & ew & 15.47 $\pm$ 0.02 & 14.93 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
70725905 & 111.331 & -3.3977 & (26,19,29) & 0.23768 & 0.64 & 0.62 & 0.64 & ew & 17.56 $\pm$ 0.03 & 16.88 $\pm$ 0.02 & 16.22 $\pm$ 0.02 \\
70726538 & 111.336 & -3.5459 & (22,18,0) & 1.19344 & 0.39 & 0.30 & 0.0 & ea & 14.18 $\pm$ 0.02 & 13.84 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
70753886 & 111.567 & -3.5984 & (27,16,29) & 2.42675 & 0.45 & 0.41 & 0.41 & ea & 14.90 $\pm$ 0.02 & 14.59 $\pm$ 0.02 & 14.25 $\pm$ 0.02 \\
70762783 & 111.643 & -3.2481 & (19,23,0) & 12.2049 & 0.44 & 0.49 & 0.0 & ea & 15.25 $\pm$ 0.02 & 14.85 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
70775044 & 111.748 & -3.2059 & (27,21,30) & 0.38961 & 0.32 & 0.41 & 0.36 & ew & 15.19 $\pm$ 0.02 & 14.61 $\pm$ 0.02 & 14.24 $\pm$ 0.02 \\
70799176 & 111.960 & -3.5790 & (24,21,29) & 1.24421 & 0.41 & 0.27 & 0.32 & ea & 17.45 $\pm$ 0.03 & 17.12 $\pm$ 0.02 & 16.64 $\pm$ 0.03 \\
70811382 & 112.067 & -3.2075 & (24,18,25) & 0.33482 & 0.85 & 0.74 & 0.87 & ew & 17.45 $\pm$ 0.03 & 16.96 $\pm$ 0.02 & 16.30 $\pm$ 0.03 \\
70859626 & 112.487 & -3.5609 & (12,23,36) & 0.28362 & 0.31 & 0.36 & 0.33 & ew & 15.30 $\pm$ 0.02 & 15.24 $\pm$ 0.02 & 14.58 $\pm$ 0.02 \\
70938590 & 113.130 & -3.3603 & (30,20,21) & 0.35082 & 0.54 & 0.49 & 0.45 & ew & 17.88 $\pm$ 0.04 & 17.51 $\pm$ 0.03 & 17.37 $\pm$ 0.04 \\
70976484 & 113.430 & -3.5727 & (19,23,28) & 1.68954 & 0.44 & 0.49 & 0.44 & ew & 14.69 $\pm$ 0.02 & 14.49 $\pm$ 0.02 & 14.25 $\pm$ 0.02 \\
71066626 & 114.190 & -3.4022 & (27,17,34) & 0.26819 & 0.34 & 0.27 & 0.31 & eb & 17.31 $\pm$ 0.03 & 16.92 $\pm$ 0.02 & 16.40 $\pm$ 0.03 \\
71069308 & 114.214 & -3.4485 & (16,20,33) & 9.16107 & 0.41 & 0.47 & 0.38 & ew & 15.43 $\pm$ 0.02 & 14.77 $\pm$ 0.02 & 14.05 $\pm$ 0.02 \\
71112694 & 114.596 & -3.1368 & (19,14,24) & 0.41439 & 0.56 & 0.62 & 0.58 & ew & 16.78 $\pm$ 0.02 & 16.42 $\pm$ 0.02 & 15.99 $\pm$ 0.02 \\
71131920 & 114.768 & -3.4509 & (19,20,30) & 0.89111 & 0.28 & 0.46 & 0.45 & ea & 16.72 $\pm$ 0.02 & 16.19 $\pm$ 0.02 & 15.71 $\pm$ 0.02 \\
71157259 & 114.989 & -3.4580 & (25,21,35) & 0.34932 & 0.49 & 0.42 & 0.41 & ew & 16.82 $\pm$ 0.02 & 16.47 $\pm$ 0.02 & 16.04 $\pm$ 0.02 \\
71178866 & 115.172 & -3.3587 & (25,19,28) & 0.33541 & 0.41 & 0.39 & 0.40 & ew & 16.67 $\pm$ 0.02 & 16.27 $\pm$ 0.02 & 15.89 $\pm$ 0.02 \\
71233272 & 115.620 & -3.3160 & (24,20,28) & 0.33500 & 0.70 & 0.50 & 0.68 & ew & 15.47 $\pm$ 0.02 & 15.11 $\pm$ 0.02 & 14.65 $\pm$ 0.02 \\
71258051 & 115.817 & -3.2693 & (23,13,0) & 0.29448 & 0.67 & 0.48 & 0.0 & eb & 17.93 $\pm$ 0.04 & 17.42 $\pm$ 0.03 & 0.0 $\pm$ 0.0 \\
71277170 & 115.981 & -3.1841 & (20,15,30) & 0.26390 & 0.42 & 0.26 & 0.24 & ew & 16.60 $\pm$ 0.02 & 16.02 $\pm$ 0.02 & 15.33 $\pm$ 0.02 \\
71292680 & 116.123 & -3.4756 & (0,19,34) & 6.66464 & 0.0 & 0.28 & 0.30 & ea & 0.0 $\pm$ 0.0 & 16.33 $\pm$ 0.02 & 15.72 $\pm$ 0.02 \\
71299445 & 116.193 & -3.5272 & (0,18,33) & 0.40572 & 0.0 & 0.38 & 0.41 & ew & 0.0 $\pm$ 0.0 & 14.12 $\pm$ 0.02 & 13.82 $\pm$ 0.03 \\
71310469 & 116.306 & -3.2616 & (26,22,29) & 0.24883 & 0.54 & 0.47 & 0.52 & ew & 17.39 $\pm$ 0.03 & 16.85 $\pm$ 0.02 & 16.31 $\pm$ 0.03 \\
71314174 & 116.345 & -3.5202 & (24,24,28) & 0.36624 & 0.89 & 0.84 & 0.74 & ew & 15.73 $\pm$ 0.02 & 15.34 $\pm$ 0.02 & 14.93 $\pm$ 0.02 \\
71322417 & 116.431 & -3.5000 & (28,20,34) & 0.64514 & 0.25 & 0.29 & 0.27 & ew & 15.56 $\pm$ 0.02 & 15.40 $\pm$ 0.02 & 15.19 $\pm$ 0.02 \\
71354262 & 116.758 & -3.2564 & (27,25,34) & 0.47227 & 0.49 & 0.49 & 0.46 & ew & 16.94 $\pm$ 0.02 & 16.59 $\pm$ 0.02 & 16.15 $\pm$ 0.02 \\
71358728 & 116.804 & -3.1279 & (20,12,24) & 4.56840 & 0.53 & 0.47 & 0.65 & eb & 15.03 $\pm$ 0.02 & 14.82 $\pm$ 0.02 & 14.57 $\pm$ 0.02 \\
71385400 & 117.092 & -3.6417 & (24,21,28) & 0.34876 & 0.41 & 0.40 & 0.45 & ew & 17.62 $\pm$ 0.03 & 17.23 $\pm$ 0.02 & 16.77 $\pm$ 0.03 \\
71399124 & 117.239 & -3.6666 & (19,0,22) & 0.39243 & 0.44 & 0.0 & 0.42 & ew & 15.25 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 14.78 $\pm$ 0.02 \\
71432617 & 117.603 & -3.6318 & (0,19,34) & 0.28566 & 0.0 & 0.58 & 0.59 & ew & 0.0 $\pm$ 0.0 & 15.94 $\pm$ 0.02 & 15.49 $\pm$ 0.02 \\
71483795 & 118.173 & -3.5911 & (26,19,34) & 0.25303 & 0.56 & 0.50 & 0.55 & ew & 17.55 $\pm$ 0.03 & 17.29 $\pm$ 0.03 & 17.29 $\pm$ 0.04 \\
71499948 & 118.361 & -3.2241 & (27,17,34) & 0.30723 & 0.24 & 0.23 & 0.34 & ew & 18.12 $\pm$ 0.04 & 17.74 $\pm$ 0.03 & 17.23 $\pm$ 0.04 \\
71513613 & 118.517 & -3.5027 & (27,0,30) & 0.38113 & 0.43 & 0.0 & 0.42 & ew & 15.57 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 14.86 $\pm$ 0.02 \\
71541694 & 118.825 & -3.1824 & (25,19,33) & 0.32228 & 0.28 & 0.24 & 0.32 & ew & 15.84 $\pm$ 0.02 & 15.66 $\pm$ 0.02 & 15.31 $\pm$ 0.02 \\
71585054 & 119.329 & -3.2231 & (22,20,39) & 2.27091 & 0.30 & 0.66 & 0.66 & ea & 16.26 $\pm$ 0.02 & 15.95 $\pm$ 0.02 & 15.55 $\pm$ 0.02 \\
71595445 & 119.458 & -3.3767 & (0,21,33) & 1.52701 & 0.0 & 0.45 & 0.48 & ea & 0.0 $\pm$ 0.0 & 14.30 $\pm$ 0.02 & 14.07 $\pm$ 0.02 \\
71596153 & 119.467 & -3.2009 & (25,19,30) & 0.55696 & 1.04 & 0.66 & 0.62 & eb & 15.99 $\pm$ 0.02 & 15.76 $\pm$ 0.02 & 15.44 $\pm$ 0.02 \\
71623003 & 119.806 & -3.3340 & (25,19,38) & 0.25972 & 0.29 & 0.27 & 0.33 & ew & 17.21 $\pm$ 0.03 & 16.79 $\pm$ 0.02 & 16.31 $\pm$ 0.03 \\
70015486 & 105.160 & -3.8228 & (28,17,14) & 1.26087 & 0.57 & 0.38 & 0.43 & ew & 16.78 $\pm$ 0.02 & 16.04 $\pm$ 0.02 & 15.13 $\pm$ 0.02 \\
70041319 & 105.413 & -4.0834 & (45,20,18) & 1.99928 & 0.28 & 0.17 & 0.22 & ew & 17.22 $\pm$ 0.03 & 16.63 $\pm$ 0.02 & 16.07 $\pm$ 0.03 \\
70084514 & 105.819 & -4.0894 & (41,18,22) & 0.26340 & 0.76 & 0.72 & 0.60 & ew & 16.19 $\pm$ 0.02 & 15.51 $\pm$ 0.03 & 14.89 $\pm$ 0.02 \\
70147130 & 106.391 & -4.0417 & (36,21,19) & 0.60415 & 0.51 & 0.54 & 0.43 & eb & 16.40 $\pm$ 0.02 & 16.03 $\pm$ 0.02 & 15.49 $\pm$ 0.02 \\
70236405 & 107.189 & -3.8558 & (31,19,17) & 0.26581 & 0.36 & 0.34 & 0.35 & ew & 15.88 $\pm$ 0.02 & 15.49 $\pm$ 0.03 & 15.05 $\pm$ 0.02 \\
70236412 & 107.189 & -4.0746 & (39,16,13) & 0.48907 & 0.37 & 0.23 & 0.26 & ew & 16.40 $\pm$ 0.02 & 16.05 $\pm$ 0.02 & 15.55 $\pm$ 0.02 \\
70269205 & 107.482 & -4.0794 & (42,22,23) & 6.51866 & 1.05 & 0.97 & 0.92 & ea & 16.64 $\pm$ 0.02 & 16.07 $\pm$ 0.02 & 15.45 $\pm$ 0.02 \\
70284138 & 107.618 & -3.8049 & (24,17,12) & 0.56747 & 0.29 & 0.22 & 0.22 & ew & 15.31 $\pm$ 0.02 & 15.03 $\pm$ 0.03 & 14.84 $\pm$ 0.02 \\
70352471 & 108.244 & -3.8959 & (28,17,13) & 0.46205 & 0.33 & 0.37 & 0.29 & ew & 17.64 $\pm$ 0.03 & 17.12 $\pm$ 0.03 & 16.51 $\pm$ 0.03 \\
70384652 & 108.519 & -4.0124 & (43,21,22) & 0.58059 & 0.35 & 0.33 & 0.36 & ew & 15.58 $\pm$ 0.02 & 15.51 $\pm$ 0.03 & 15.11 $\pm$ 0.02 \\
70419346 & 108.810 & -3.9225 & (38,15,16) & 1.62033 & 0.68 & 0.31 & 0.33 & ea & 16.12 $\pm$ 0.02 & 15.78 $\pm$ 0.03 & 15.49 $\pm$ 0.02 \\
70435635 & 108.952 & -3.9172 & (29,24,22) & 16.5314 & 0.35 & 0.29 & 0.24 & ew & 16.22 $\pm$ 0.02 & 15.35 $\pm$ 0.03 & 14.88 $\pm$ 0.02 \\
70436331 & 108.958 & -4.0784 & (41,21,26) & 0.37526 & 0.31 & 0.34 & 0.27 & ew & 17.29 $\pm$ 0.03 & 16.68 $\pm$ 0.02 & 16.37 $\pm$ 0.03 \\
70442555 & 109.013 & -3.8560 & (28,18,13) & 0.43635 & 0.47 & 0.29 & 0.27 & ew & 16.86 $\pm$ 0.02 & 16.45 $\pm$ 0.02 & 16.06 $\pm$ 0.03 \\
70456702 & 109.139 & -4.0082 & (39,18,11) & 0.30606 & 0.43 & 0.45 & 0.43 & ew & 16.94 $\pm$ 0.02 & 16.55 $\pm$ 0.02 & 16.16 $\pm$ 0.03 \\
70469200 & 109.248 & -3.9006 & (37,19,20) & 7.08463 & 0.62 & 0.77 & 0.67 & ea & 14.84 $\pm$ 0.02 & 14.73 $\pm$ 0.03 & 14.57 $\pm$ 0.02 \\
70575450 & 110.151 & -4.0661 & (47,20,23) & 0.46712 & 0.48 & 0.39 & 0.42 & ew & 16.78 $\pm$ 0.02 & 16.36 $\pm$ 0.02 & 15.91 $\pm$ 0.03 \\
70576396 & 110.158 & -3.8431 & (34,16,13) & 0.36846 & 0.65 & 0.62 & 0.53 & ew & 17.11 $\pm$ 0.02 & 16.61 $\pm$ 0.02 & 16.12 $\pm$ 0.03 \\
70599060 & 110.337 & -4.0548 & (40,22,25) & 0.98489 & 0.53 & 0.46 & 0.37 & ew & 17.12 $\pm$ 0.02 & 16.83 $\pm$ 0.02 & 16.49 $\pm$ 0.03 \\
70618385 & 110.483 & -4.0553 & (35,0,21) & 0.27586 & 0.44 & 0.0 & 0.43 & ew & 15.35 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 14.59 $\pm$ 0.02 \\
70630614 & 110.579 & -3.9096 & (35,21,21) & 0.41060 & 0.45 & 0.32 & 0.39 & ew & 14.51 $\pm$ 0.02 & 14.12 $\pm$ 0.04 & 13.68 $\pm$ 0.03 \\
70633677 & 110.604 & -4.1330 & (36,19,20) & 0.60851 & 0.70 & 0.67 & 0.66 & ew & 15.23 $\pm$ 0.02 & 15.02 $\pm$ 0.03 & 14.75 $\pm$ 0.02 \\
70639101 & 110.648 & -4.0306 & (33,14,14) & 0.38901 & 0.44 & 0.38 & 0.42 & ew & 17.63 $\pm$ 0.03 & 17.18 $\pm$ 0.03 & 16.35 $\pm$ 0.03 \\
70651515 & 110.749 & -3.9558 & (33,14,20) & 0.30554 & 0.58 & 0.47 & 0.54 & ew & 16.40 $\pm$ 0.02 & 16.33 $\pm$ 0.02 & 15.51 $\pm$ 0.02 \\
70659534 & 110.815 & -4.2188 & (27,0,25) & 0.50760 & 2.39 & 0.0 & 0.72 & ea & 15.95 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 14.77 $\pm$ 0.02 \\
70673153 & 110.918 & -4.2182 & (24,0,24) & 0.99678 & 2.21 & 0.0 & 0.43 & ea & 15.47 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 14.82 $\pm$ 0.02 \\
70678357 & 110.958 & -4.0948 & (49,23,23) & 0.33981 & 0.22 & 0.17 & 0.25 & ew & 16.74 $\pm$ 0.02 & 16.13 $\pm$ 0.02 & 15.75 $\pm$ 0.02 \\
70731893 & 111.379 & -3.8045 & (28,14,11) & 0.31368 & 0.52 & 0.57 & 0.36 & ew & 16.44 $\pm$ 0.02 & 15.95 $\pm$ 0.02 & 15.40 $\pm$ 0.02 \\
70733462 & 111.392 & -4.0497 & (44,0,23) & 0.32868 & 0.47 & 0.0 & 0.43 & ew & 16.68 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 15.45 $\pm$ 0.02 \\
70764200 & 111.654 & -3.9917 & (39,0,22) & 0.40736 & 0.48 & 0.0 & 0.48 & ew & 17.22 $\pm$ 0.03 & 0.0 $\pm$ 0.0 & 16.40 $\pm$ 0.03 \\
70776462 & 111.761 & -3.9403 & (38,15,10) & 0.53621 & 0.30 & 0.31 & 0.25 & ew & 14.33 $\pm$ 0.02 & 14.32 $\pm$ 0.04 & 13.84 $\pm$ 0.03 \\
70846801 & 112.384 & -3.8743 & (31,13,20) & 3.15249 & 0.86 & 0.37 & 0.66 & ea & 15.20 $\pm$ 0.02 & 14.64 $\pm$ 0.03 & 14.20 $\pm$ 0.03 \\
70933035 & 113.087 & -3.8246 & (28,14,16) & 0.33581 & 0.60 & 0.22 & 0.20 & ew & 16.71 $\pm$ 0.02 & 16.21 $\pm$ 0.02 & 15.76 $\pm$ 0.02 \\
70964363 & 113.334 & -4.1620 & (27,17,15) & 0.28579 & 0.71 & 0.53 & 0.51 & ea & 17.53 $\pm$ 0.03 & 17.04 $\pm$ 0.03 & 16.52 $\pm$ 0.03 \\
71003955 & 113.655 & -4.1120 & (38,16,21) & 0.35526 & 0.80 & 0.75 & 0.69 & eb & 16.78 $\pm$ 0.02 & 16.41 $\pm$ 0.02 & 15.97 $\pm$ 0.03 \\
71009852 & 113.704 & -4.1361 & (41,20,17) & 0.30478 & 0.58 & 0.54 & 0.48 & eb & 16.32 $\pm$ 0.02 & 15.79 $\pm$ 0.03 & 15.25 $\pm$ 0.02 \\
71036349 & 113.928 & -3.8588 & (37,0,17) & 0.34605 & 0.57 & 0.0 & 0.38 & ew & 16.00 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 15.05 $\pm$ 0.02 \\
71050234 & 114.046 & -3.9266 & (44,23,17) & 0.29686 & 0.54 & 0.42 & 0.52 & ew & 15.71 $\pm$ 0.02 & 15.22 $\pm$ 0.03 & 14.66 $\pm$ 0.02 \\
71063356 & 114.161 & -4.0505 & (45,18,17) & 0.50303 & 0.59 & 0.28 & 0.30 & ea & 17.51 $\pm$ 0.03 & 16.90 $\pm$ 0.02 & 16.32 $\pm$ 0.03 \\
71103614 & 114.514 & -4.1601 & (30,18,0) & 0.35567 & 0.62 & 0.48 & 0.0 & ew & 18.43 $\pm$ 0.05 & 17.70 $\pm$ 0.04 & 0.0 $\pm$ 0.0 \\
71202458 & 115.371 & -4.1135 & (43,0,26) & 0.35344 & 0.45 & 0.0 & 0.38 & ew & 16.95 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 16.11 $\pm$ 0.03 \\
71328295 & 116.493 & -4.1092 & (42,22,21) & 0.31353 & 0.44 & 0.42 & 0.28 & ew & 17.71 $\pm$ 0.03 & 17.30 $\pm$ 0.03 & 16.85 $\pm$ 0.03 \\
71346080 & 116.676 & -4.1753 & (29,22,27) & 0.32889 & 0.46 & 0.46 & 0.42 & ew & 16.70 $\pm$ 0.02 & 16.39 $\pm$ 0.02 & 15.99 $\pm$ 0.03 \\
71408694 & 117.343 & -4.0335 & (41,25,24) & 0.04155 & 0.37 & 0.24 & 0.40 & ea & 17.56 $\pm$ 0.03 & 17.15 $\pm$ 0.03 & 16.75 $\pm$ 0.03 \\
71413779 & 117.399 & -4.0030 & (45,25,22) & 0.41893 & 0.27 & 0.27 & 0.27 & ew & 16.98 $\pm$ 0.02 & 16.75 $\pm$ 0.02 & 16.59 $\pm$ 0.03 \\
71419075 & 117.456 & -3.9918 & (45,21,23) & 3.89363 & 0.64 & 0.63 & 0.54 & eb & 15.87 $\pm$ 0.02 & 15.25 $\pm$ 0.03 & 14.46 $\pm$ 0.02 \\
71437037 & 117.652 & -3.9915 & (50,24,26) & 1.14111 & 0.32 & 0.38 & 0.38 & ea & 16.09 $\pm$ 0.02 & 15.97 $\pm$ 0.02 & 15.68 $\pm$ 0.02 \\
71458160 & 117.887 & -4.1093 & (40,0,27) & 0.54668 & 0.39 & 0.0 & 0.38 & ew & 14.11 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 13.32 $\pm$ 0.03 \\
71483854 & 118.173 & -4.0909 & (42,23,20) & 0.29388 & 0.20 & 0.20 & 0.13 & ew & 14.92 $\pm$ 0.02 & 14.67 $\pm$ 0.03 & 14.35 $\pm$ 0.02 \\
71488402 & 118.226 & -3.8321 & (31,15,19) & 0.45856 & 0.40 & 0.27 & 0.36 & ew & 16.41 $\pm$ 0.02 & 16.31 $\pm$ 0.02 & 15.62 $\pm$ 0.02 \\
71499801 & 118.360 & -4.1368 & (39,20,19) & 0.31221 & 0.7 & 0.62 & 0.77 & ew & 17.97 $\pm$ 0.04 & 17.57 $\pm$ 0.03 & 17.11 $\pm$ 0.04 \\
71508785 & 118.463 & -4.1291 & (43,18,20) & 0.49491 & 0.31 & 0.24 & 0.34 & ew & 15.43 $\pm$ 0.02 & 15.21 $\pm$ 0.03 & 14.99 $\pm$ 0.02 \\
71515587 & 118.538 & -4.2149 & (29,15,20) & 0.90977 & 0.28 & 0.29 & 0.67 & ew & 14.42 $\pm$ 0.02 & 14.09 $\pm$ 0.04 & 13.93 $\pm$ 0.03 \\
71543125 & 118.842 & -4.1213 & (37,18,23) & 0.22859 & 0.72 & 0.44 & 0.64 & ew & 17.75 $\pm$ 0.04 & 17.22 $\pm$ 0.03 & 16.64 $\pm$ 0.03 \\
71548827 & 118.905 & -4.2301 & (35,9,21) & 1.89363 & 0.45 & 0.25 & 0.71 & ea & 14.45 $\pm$ 0.02 & 14.25 $\pm$ 0.04 & 14.01 $\pm$ 0.03 \\
71556510 & 118.992 & -3.9640 & (36,17,24) & 5.82530 & 0.47 & 0.43 & 0.47 & ew & 15.24 $\pm$ 0.02 & 14.91 $\pm$ 0.03 & 14.48 $\pm$ 0.02 \\
71568922 & 119.136 & -4.2413 & (19,19,19) & 0.29387 & 0.7 & 0.65 & 0.70 & ea & 15.11 $\pm$ 0.02 & 14.61 $\pm$ 0.03 & 14.14 $\pm$ 0.03 \\
71576051 & 119.219 & -3.9349 & (42,23,21) & 2.80217 & 0.33 & 0.37 & 0.33 & ew & 15.19 $\pm$ 0.02 & 14.92 $\pm$ 0.03 & 14.61 $\pm$ 0.02 \\
71612248 & 119.668 & -4.0284 & (39,22,13) & 0.37280 & 0.36 & 0.36 & 0.34 & ew & 16.10 $\pm$ 0.02 & 15.83 $\pm$ 0.02 & 15.44 $\pm$ 0.02 \\
71625223 & 119.835 & -4.1519 & (31,18,19) & 0.36436 & 0.32 & 0.30 & 0.78 & ew & 16.90 $\pm$ 0.02 & 16.46 $\pm$ 0.02 & 16.0 $\pm$ 0.03 \\
80035729 & 120.442 & -2.8029 & (61,51,0) & 0.48679 & 0.50 & 0.52 & 0.0 & ea & 14.23 $\pm$ 0.03 & 13.83 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80037563 & 120.466 & -3.0372 & (39,34,64) & 4.23025 & 0.57 & 0.42 & 0.44 & ea & 14.25 $\pm$ 0.03 & 13.96 $\pm$ 0.01 & 13.71 $\pm$ 0.02 \\
80043922 & 120.548 & -2.8253 & (64,50,0) & 0.89874 & 0.34 & 0.35 & 0.0 & ew & 15.13 $\pm$ 0.02 & 14.90 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80073990 & 120.926 & -2.6789 & (71,44,0) & 0.37937 & 0.50 & 0.43 & 0.0 & ew & 16.51 $\pm$ 0.03 & 16.21 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80092610 & 121.167 & -2.8353 & (65,58,0) & 0.40705 & 0.29 & 0.23 & 0.0 & ew & 15.06 $\pm$ 0.02 & 14.81 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80136658 & 121.746 & -2.7817 & (38,60,87) & 0.25085 & 0.85 & 0.69 & 0.49 & ew & 18.05 $\pm$ 0.07 & 17.61 $\pm$ 0.03 & 17.52 $\pm$ 0.05 \\
80190546 & 122.482 & -2.5931 & (28,48,64) & 0.24214 & 0.71 & 0.64 & 0.60 & ew & 18.26 $\pm$ 0.08 & 17.85 $\pm$ 0.04 & 17.44 $\pm$ 0.05 \\
80228202 & 123.020 & -2.6968 & (0,50,76) & 0.33451 & 0.0 & 0.63 & 0.41 & ea & 0.0 $\pm$ 0.0 & 18.58 $\pm$ 0.07 & 18.12 $\pm$ 0.08 \\
80248581 & 123.317 & -2.6394 & (46,46,90) & 0.29132 & 0.63 & 0.63 & 0.48 & ew & 18.08 $\pm$ 0.07 & 17.44 $\pm$ 0.03 & 16.90 $\pm$ 0.03 \\
80250382 & 123.343 & -2.9036 & (62,46,82) & 0.34196 & 0.36 & 0.38 & 0.34 & ew & 14.86 $\pm$ 0.02 & 14.40 $\pm$ 0.01 & 14.08 $\pm$ 0.02 \\
80309940 & 124.248 & -3.0056 & (0,38,71) & 0.33738 & 0.0 & 0.47 & 0.43 & ew & 0.0 $\pm$ 0.0 & 17.17 $\pm$ 0.02 & 16.84 $\pm$ 0.03 \\
80342868 & 124.770 & -2.5126 & (18,32,54) & 10.2698 & 0.51 & 0.65 & 0.58 & ea & 18.10 $\pm$ 0.08 & 17.43 $\pm$ 0.03 & 16.84 $\pm$ 0.03 \\
80365215 & 125.134 & -2.9086 & (56,46,0) & 0.20217 & 0.59 & 0.41 & 0.0 & ew & 17.88 $\pm$ 0.07 & 17.23 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
80383570 & 125.445 & -2.8189 & (68,50,0) & 0.34105 & 0.25 & 0.21 & 0.0 & ew & 15.12 $\pm$ 0.02 & 14.69 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80416105 & 126.014 & -2.9232 & (61,41,80) & 0.77201 & 0.65 & 0.40 & 0.45 & ew & 17.48 $\pm$ 0.06 & 17.61 $\pm$ 0.03 & 17.39 $\pm$ 0.05 \\
80432262 & 126.295 & -2.6318 & (59,48,78) & 0.33473 & 0.58 & 0.36 & 0.41 & ew & 16.62 $\pm$ 0.03 & 16.36 $\pm$ 0.01 & 16.2 $\pm$ 0.03 \\
80453363 & 126.664 & -2.8067 & (65,48,86) & 0.21677 & 0.31 & 0.31 & 0.40 & ew & 16.54 $\pm$ 0.03 & 16.05 $\pm$ 0.01 & 15.64 $\pm$ 0.02 \\
80482415 & 127.189 & -2.8908 & (65,50,0) & 0.40177 & 0.66 & 0.70 & 0.0 & ew & 16.34 $\pm$ 0.03 & 15.98 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80482473 & 127.190 & -2.6299 & (51,50,0) & 0.31498 & 0.40 & 0.39 & 0.0 & ea & 17.38 $\pm$ 0.05 & 16.78 $\pm$ 0.02 & 0.0 $\pm$ 0.0 \\
80529680 & 128.092 & -2.8595 & (61,50,0) & 0.21427 & 0.41 & 0.36 & 0.0 & ew & 16.13 $\pm$ 0.02 & 15.79 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80538135 & 128.258 & -2.8486 & (62,52,88) & 0.27290 & 0.54 & 0.37 & 0.76 & ew & 17.15 $\pm$ 0.04 & 16.41 $\pm$ 0.01 & 16.01 $\pm$ 0.02 \\
80550396 & 128.499 & -2.5814 & (51,42,80) & 0.49180 & 0.56 & 0.42 & 0.50 & ew & 14.90 $\pm$ 0.02 & 14.96 $\pm$ 0.01 & 14.39 $\pm$ 0.02 \\
80579393 & 129.072 & -2.8578 & (55,48,86) & 0.45996 & 0.29 & 0.20 & 0.23 & ew & 16.09 $\pm$ 0.02 & 15.71 $\pm$ 0.01 & 15.46 $\pm$ 0.02 \\
80671001 & 131.010 & -2.8824 & (60,37,90) & 1.16237 & 0.26 & 0.27 & 0.27 & ew & 15.87 $\pm$ 0.02 & 15.76 $\pm$ 0.01 & 15.71 $\pm$ 0.02 \\
80760463 & 133.229 & -2.8599 & (51,46,78) & 0.38263 & 0.39 & 0.32 & 0.32 & ew & 17.02 $\pm$ 0.04 & 16.78 $\pm$ 0.02 & 16.66 $\pm$ 0.03 \\
80007177 & 120.091 & -3.4813 & (37,23,43) & 0.27379 & 0.31 & 0.27 & 0.31 & ew & 16.96 $\pm$ 0.02 & 16.57 $\pm$ 0.01 & 16.18 $\pm$ 0.02 \\
80026440 & 120.327 & -3.3119 & (32,21,41) & 0.26717 & 0.82 & 0.73 & 0.69 & ew & 16.89 $\pm$ 0.02 & 16.44 $\pm$ 0.01 & 16.05 $\pm$ 0.02 \\
80057215 & 120.715 & -3.3998 & (37,24,45) & 0.33863 & 0.90 & 0.50 & 0.80 & ew & 15.71 $\pm$ 0.01 & 15.40 $\pm$ 0.01 & 15.13 $\pm$ 0.01 \\
80075453 & 120.946 & -3.1728 & (0,18,34) & 0.32836 & 0.0 & 0.50 & 0.35 & ew & 0.0 $\pm$ 0.0 & 14.68 $\pm$ 0.01 & 14.42 $\pm$ 0.01 \\
80120014 & 121.521 & -3.3025 & (30,23,45) & 0.51822 & 0.30 & 0.25 & 0.27 & ew & 14.36 $\pm$ 0.01 & 14.19 $\pm$ 0.01 & 14.06 $\pm$ 0.01 \\
80131348 & 121.673 & -3.2002 & (36,18,29) & 0.31944 & 0.49 & 0.27 & 0.23 & ew & 16.92 $\pm$ 0.02 & 16.36 $\pm$ 0.01 & 15.93 $\pm$ 0.02 \\
80131616 & 121.677 & -3.5019 & (29,22,32) & 0.38340 & 0.85 & 0.86 & 0.89 & ew & 17.17 $\pm$ 0.03 & 16.85 $\pm$ 0.02 & 16.53 $\pm$ 0.02 \\
80151252 & 121.941 & -3.5100 & (32,26,42) & 0.54675 & 1.09 & 0.98 & 0.91 & ew & 17.22 $\pm$ 0.03 & 16.77 $\pm$ 0.02 & 16.37 $\pm$ 0.02 \\
80168830 & 122.181 & -3.6146 & (26,21,39) & 0.20900 & 0.34 & 0.24 & 0.29 & ew & 17.81 $\pm$ 0.04 & 17.03 $\pm$ 0.02 & 16.5 $\pm$ 0.02 \\
80211083 & 122.771 & -3.1945 & (29,24,34) & 0.76687 & 0.41 & 0.47 & 0.35 & ew & 17.05 $\pm$ 0.02 & 16.91 $\pm$ 0.02 & 16.74 $\pm$ 0.03 \\
80306755 & 124.197 & -3.6785 & (0,16,25) & 0.29762 & 0.0 & 0.41 & 0.42 & ew & 0.0 $\pm$ 0.0 & 16.45 $\pm$ 0.01 & 15.94 $\pm$ 0.02 \\
80324778 & 124.477 & -3.4832 & (33,25,40) & 0.48667 & 0.58 & 0.32 & 0.84 & ew & 16.30 $\pm$ 0.02 & 15.95 $\pm$ 0.01 & 15.65 $\pm$ 0.01 \\
80332259 & 124.595 & -3.3584 & (36,21,45) & 0.23554 & 0.56 & 0.34 & 0.34 & ew & 17.60 $\pm$ 0.03 & 17.04 $\pm$ 0.02 & 16.55 $\pm$ 0.02 \\
80337842 & 124.688 & -3.5874 & (34,24,41) & 0.27743 & 0.67 & 0.58 & 0.52 & ew & 18.15 $\pm$ 0.05 & 17.59 $\pm$ 0.03 & 17.03 $\pm$ 0.04 \\
80380421 & 125.392 & -3.1605 & (26,17,32) & 0.21178 & 0.29 & 0.21 & 0.29 & ew & 17.04 $\pm$ 0.02 & 16.52 $\pm$ 0.01 & 16.21 $\pm$ 0.02 \\
80398835 & 125.708 & -3.6187 & (29,18,40) & 0.33469 & 0.22 & 0.25 & 0.25 & ew & 16.47 $\pm$ 0.02 & 15.87 $\pm$ 0.01 & 15.34 $\pm$ 0.01 \\
80411627 & 125.935 & -3.6181 & (27,20,34) & 0.23811 & 0.41 & 0.29 & 0.38 & ew & 16.66 $\pm$ 0.02 & 16.19 $\pm$ 0.01 & 15.72 $\pm$ 0.02 \\
80444806 & 126.516 & -3.3488 & (29,23,38) & 0.34503 & 0.53 & 0.49 & 0.50 & ew & 14.99 $\pm$ 0.01 & 14.62 $\pm$ 0.01 & 14.24 $\pm$ 0.01 \\
80475567 & 127.063 & -3.3855 & (35,0,39) & 0.38175 & 0.36 & 0.0 & 0.33 & ew & 16.71 $\pm$ 0.02 & 0.0 $\pm$ 0.0 & 16.12 $\pm$ 0.02 \\
80496178 & 127.447 & -3.2784 & (32,23,34) & 0.24796 & 0.88 & 0.56 & 0.51 & ew & 18.50 $\pm$ 0.06 & 18.00 $\pm$ 0.05 & 17.45 $\pm$ 0.05 \\
80510152 & 127.714 & -3.5173 & (26,21,39) & 0.45164 & 0.61 & 0.52 & 0.57 & ew & 16.28 $\pm$ 0.02 & 16.00 $\pm$ 0.01 & 15.68 $\pm$ 0.02 \\
80560757 & 128.695 & -3.5022 & (24,19,41) & 0.41766 & 1.10 & 0.9 & 0.90 & ew & 18.75 $\pm$ 0.08 & 18.03 $\pm$ 0.05 & 17.41 $\pm$ 0.05 \\
80563334 & 128.745 & -3.1859 & (33,20,39) & 0.26367 & 0.45 & 0.26 & 0.23 & ew & 16.90 $\pm$ 0.02 & 16.48 $\pm$ 0.01 & 15.71 $\pm$ 0.02 \\
80640655 & 130.374 & -3.2221 & (35,19,40) & 0.33652 & 0.37 & 0.32 & 0.35 & ew & 15.08 $\pm$ 0.01 & 14.66 $\pm$ 0.01 & 14.31 $\pm$ 0.01 \\
80660959 & 130.786 & -3.6434 & (27,19,21) & 0.36548 & 0.55 & 0.52 & 0.50 & ew & 16.48 $\pm$ 0.02 & 16.08 $\pm$ 0.01 & 15.74 $\pm$ 0.02 \\
80705613 & 131.834 & -3.1423 & (23,14,27) & 0.55394 & 0.45 & 0.32 & 0.64 & ew & 16.24 $\pm$ 0.02 & 16.09 $\pm$ 0.01 & 15.95 $\pm$ 0.02 \\
80714634 & 132.051 & -3.5892 & (37,22,36) & 0.80126 & 0.56 & 0.41 & 0.39 & ew & 16.99 $\pm$ 0.02 & 16.80 $\pm$ 0.02 & 16.64 $\pm$ 0.03 \\
80802886 & 134.386 & -3.1606 & (23,15,32) & 0.48601 & 0.83 & 0.38 & 0.43 & ew & 14.96 $\pm$ 0.01 & 14.64 $\pm$ 0.01 & 14.41 $\pm$ 0.01 \\
80003367 & 120.043 & -4.0948 & (59,27,23) & 1.97606 & 0.69 & 0.64 & 0.67 & ea & 14.31 $\pm$ 0.02 & 14.09 $\pm$ 0.01 & 13.89 $\pm$ 0.01 \\
80014251 & 120.177 & -3.9017 & (54,29,28) & 0.34958 & 0.94 & 0.84 & 0.78 & eb & 16.77 $\pm$ 0.03 & 16.3 $\pm$ 0.02 & 15.85 $\pm$ 0.02 \\
80029283 & 120.362 & -3.7880 & (35,17,19) & 0.38960 & 0.43 & 0.40 & 0.61 & ew & 17.26 $\pm$ 0.03 & 16.94 $\pm$ 0.02 & 16.55 $\pm$ 0.03 \\
80067623 & 120.847 & -3.7887 & (33,18,24) & 0.87538 & 0.60 & 0.54 & 0.49 & ew & 15.43 $\pm$ 0.02 & 15.09 $\pm$ 0.01 & 14.81 $\pm$ 0.01 \\
80097504 & 121.230 & -4.1212 & (57,28,33) & 0.456 & 0.76 & 0.43 & 0.45 & ew & 15.00 $\pm$ 0.02 & 14.80 $\pm$ 0.01 & 14.52 $\pm$ 0.01 \\
80123250 & 121.563 & -4.1522 & (46,29,35) & 0.33095 & 0.56 & 0.61 & 0.97 & ew & 16.28 $\pm$ 0.03 & 16.0 $\pm$ 0.01 & 15.66 $\pm$ 0.02 \\
80148444 & 121.905 & -4.0497 & (54,34,35) & 0.49343 & 0.72 & 0.62 & 0.59 & ew & 15.02 $\pm$ 0.02 & 14.69 $\pm$ 0.01 & 14.43 $\pm$ 0.01 \\
80201516 & 122.634 & -3.9012 & (53,33,34) & 0.27266 & 0.85 & 0.61 & 0.57 & ew & 15.25 $\pm$ 0.02 & 14.85 $\pm$ 0.01 & 14.46 $\pm$ 0.01 \\
80204989 & 122.684 & -4.2371 & (50,27,31) & 0.32767 & 0.39 & 0.61 & 0.29 & ew & 15.91 $\pm$ 0.02 & 15.23 $\pm$ 0.01 & 14.79 $\pm$ 0.01 \\
80205630 & 122.693 & -4.1365 & (49,32,33) & 0.26199 & 0.24 & 0.40 & 0.65 & ew & 16.63 $\pm$ 0.03 & 16.20 $\pm$ 0.02 & 15.83 $\pm$ 0.02 \\
80262699 & 123.526 & -4.0365 & (56,33,32) & 0.36007 & 0.41 & 0.59 & 0.38 & ew & 17.00 $\pm$ 0.03 & 16.61 $\pm$ 0.02 & 16.23 $\pm$ 0.02 \\
80269434 & 123.624 & -3.9551 & (41,33,17) & 0.62653 & 0.61 & 0.73 & 0.62 & ew & 18.63 $\pm$ 0.09 & 18.41 $\pm$ 0.06 & 18.59 $\pm$ 0.10 \\
80271843 & 123.659 & -3.9990 & (38,33,33) & 0.22592 & 0.67 & 1.04 & 0.54 & ew & 19.11 $\pm$ 0.11 & 18.33 $\pm$ 0.06 & 17.84 $\pm$ 0.07 \\
80292101 & 123.969 & -4.2308 & (48,29,27) & 0.33736 & 0.62 & 0.36 & 0.61 & ea & 17.40 $\pm$ 0.04 & 16.73 $\pm$ 0.02 & 15.99 $\pm$ 0.02 \\
80292570 & 123.976 & -4.0189 & (59,32,32) & 0.40138 & 0.43 & 0.59 & 0.33 & ew & 16.36 $\pm$ 0.03 & 16.00 $\pm$ 0.01 & 15.60 $\pm$ 0.02 \\
80365166 & 125.134 & -4.2703 & (32,21,18) & 0.26874 & 0.46 & 0.39 & 0.42 & ew & 15.49 $\pm$ 0.02 & 14.99 $\pm$ 0.01 & 14.47 $\pm$ 0.01 \\
80400041 & 125.729 & -3.8001 & (34,23,0) & 2.41183 & 0.55 & 0.69 & 0.0 & ea & 16.14 $\pm$ 0.03 & 15.53 $\pm$ 0.01 & 0.0 $\pm$ 0.0 \\
80404115 & 125.802 & -4.0566 & (58,30,33) & 0.32079 & 0.29 & 0.24 & 0.32 & ew & 15.13 $\pm$ 0.02 & 15.00 $\pm$ 0.01 & 14.53 $\pm$ 0.01 \\
80470454 & 126.969 & -3.9881 & (57,28,33) & 1.99542 & 0.37 & 0.21 & 0.12 & ew & 14.98 $\pm$ 0.02 & 14.60 $\pm$ 0.01 & 13.99 $\pm$ 0.01 \\
80499392 & 127.508 & -4.0288 & (64,28,34) & 0.34919 & 0.23 & 0.26 & 0.28 & ew & 14.48 $\pm$ 0.02 & 14.07 $\pm$ 0.01 & 13.66 $\pm$ 0.01 \\
80526300 & 128.024 & -4.2917 & (30,18,16) & 0.43715 & 0.67 & 0.65 & 0.53 & ew & 14.41 $\pm$ 0.02 & 13.94 $\pm$ 0.02 & 13.49 $\pm$ 0.02 \\
80549180 & 128.476 & -4.2479 & (41,23,24) & 0.48137 & 0.45 & 0.27 & 0.47 & ew & 13.92 $\pm$ 0.02 & 13.72 $\pm$ 0.02 & 13.53 $\pm$ 0.02 \\
80598558 & 129.475 & -4.1050 & (57,26,28) & 0.51821 & 0.44 & 0.41 & 0.28 & ew & 16.00 $\pm$ 0.02 & 15.56 $\pm$ 0.01 & 15.05 $\pm$ 0.01 \\
80612587 & 129.779 & -4.1313 & (54,27,30) & 1.77939 & 0.49 & 2.61 & 0.53 & ea & 16.74 $\pm$ 0.03 & 16.43 $\pm$ 0.02 & 15.94 $\pm$ 0.02 \\
80612668 & 129.781 & -4.0933 & (60,29,33) & 1.00894 & 0.26 & 0.25 & 0.23 & ea & 14.99 $\pm$ 0.02 & 14.70 $\pm$ 0.01 & 14.36 $\pm$ 0.01 \\
80654234 & 130.646 & -4.0339 & (56,27,19) & 0.39912 & 0.42 & 0.87 & 0.41 & ew & 17.33 $\pm$ 0.04 & 17.05 $\pm$ 0.02 & 16.75 $\pm$ 0.03 \\
80655851 & 130.682 & -3.8390 & (39,0,11) & 0.41921 & 0.51 & 0.0 & 0.26 & ew & 16.96 $\pm$ 0.03 & 0.0 $\pm$ 0.0 & 16.58 $\pm$ 0.03 \\
80672147 & 131.036 & -4.1111 & (56,27,20) & 0.24442 & 0.88 & 0.78 & 0.63 & ew & 15.06 $\pm$ 0.02 & 14.30 $\pm$ 0.01 & 13.55 $\pm$ 0.02 \\
80704763 & 131.813 & -4.2719 & (30,21,20) & 1.99518 & 0.46 & 0.37 & 0.35 & ew & 17.84 $\pm$ 0.05 & 17.95 $\pm$ 0.04 & 17.49 $\pm$ 0.05 \\
51121900 & 85.1332 & -4.7224 & (20,11,21) & 0.30674 & 0.58 & 0.59 & 0.55 & ew & 16.62 $\pm$ 0.02 & 15.68 $\pm$ 0.01 & 14.72 $\pm$ 0.02 \\
80375784 & 125.312 & -6.0289 & (17,9,13) & 0.35602 & 0.50 & 0.59 & 0.45 & eb & 14.91 $\pm$ 0.02 & 14.4 $\pm$ 0.01 & 13.86 $\pm$ 0.02 \\
\hline
\end{tabular}


==> match_ctrs.tex <==
\begin{table*}
\caption{QUEST matches with ctrs catalogue}
\label{tab:table_cross1}
\begin{tabular}{ccccccccc}
\hline
$ID_{QUEST}$ & $P_{QUEST}$ & $V_{amp}$ & $Type_{QUEST}$ & $ID_{CTRS}$ & $P_{CTRS}$ & $V_{amp}$ & $Type_{CTRS}$ & Comments (periods)\\
\hline
40047541 & 0.263274 & 0.307 & EW & J041329.6-031402 & 0.26327 & 0.21 & EW & matches\\
40067341 & 0.310505 & 0.329 & EA & J041810.3-024627 & " & 0.07 & EA$_{UP}$ & "\\
40083051 & 0.352228 & 0.328 & EW & J042232.8-015739 & 0.352226 & 0.2 & EW & matches\\
40141914 & 0.409572 & 0.523 & EW & J043216.2-015942 & 0.29033 & 0.55 & EW & 1-day alias\\
40152097 & 0.267945 & 0.666 & EW & J043338.3-015918 & 0.23621 & 0.38 & EW & "\\
40167353 & 0.2619 & 0.358 & EW & J043543.5-021650 & 0.261898 & 0.23 & EW & matches\\
40214294 & 1.21665 & 0.489 & EW & J044031.5-022038 & 0.7556671 & 0.49 & EB & "\\
40216809 & 0.622373 & 0.237 & EW & J044043.1-022307 & 0.383198 & 0.2 & EW & 1-day alias\\
40235593 & 3.006914 & 0.369 & EW & J044152.6-031827 & 2.97192 & 0.36 & RS Cvn & matches\\
40241503 & 1.110584 & 0.292 & EW & J044219.2-024516 & 1.11057 & 0.18 & EW & matches\\
40264408 & 0.2378 & 0.362 & EW & J044357.3-040621 & 0.269994 & 0.24 & EW & "\\
40279847 & 0.333028 & 0.428 & EW & J044459.3+020007 & 0.333026 & 0.38 & EW & matches\\
40295540 & 0.351989 & 0.492 & EW & J044558.1+015643 & 0.351991 & 0.35 & EW & matches\\
40321878 & 0.554846 & 0.386 & EW & J044732.9+002319 & 0.55486 & 0.32 & EB & matches\\
40330828 & 0.281702 & 0.336 & EW & J044816.4-015528 & 0.281701 & 0.21 & EW & matches\\
40341518 & 0.493172 & 0.312 & EW & J044841.6-031056 & 0.395408 & 0.28 & EW & "\\
40344206 & 0.375206 & 0.301 & EW & J044850.6+024055 & 0.375202 & 0.21 & EW & matches\\
40367482 & 0.282216 & 0.55 & EW & J045020.0-000613 & 0.328732 & 0.46 & EW & "\\
40369450 & 0.472584 & 0.449 & EW & J045015.2-035058 & 0.31506 & 0.39 & EW & 1-day alias\\
40370918 & 0.473701 & 0.267 & EW & J045020.1+024205 & 0.473703 & 0.14 & EW & matches\\
40391814 & 0.327076 & 0.441 & EW & J045126.6+023302 & 0.327081 & 0.25 & EW & matches\\
40392956 & 0.269416 & 0.678 & EW & J045129.8+004132 & 0.26938 & 0.64 & EW & matches\\
40399642 & 0.619086 & 0.339 & EW & J045150.2+022749 & 0.618561 & 0.34 & EW & matches\\
40400407 & 2.285851 & 0.578 & EA & J045152.6+015641 & 1.06613 & 0.11 & EA & "\\
40402872 & 0.362674 & 0.318 & EW & J045200.5+032258 & 0.362674 & 0.26 & EW & matches\\
40410911 & 0.383036 & 0.242 & EW & J045224.9+043409 & 0.474088 & 0.26 & EW & "\\
40413074 & 0.402744 & 0.329 & EW & J045242.0-020317 & 0.286878 & 0.21 & EW & 1-day alias\\
40419252 & 0.317324 & 0.363 & EW & J045250.4+044618 & 0.317326 & 0.35 & EW & matches\\
40421225 & 2.066818 & 0.419 & EA & J045256.2+033551 & 0.8135789 & 0.65 & EA & "\\
40428207 & 0.346198 & 0.351 & EW & J045316.6+014845 & 0.34622 & 0.34 & EW & matches\\
40430447 & 0.30083 & 0.52 & EW & J045333.7-000605 & 0.300956 & 0.29 & EW & matches\\
40430964 & 0.362752 & 0.486 & EW & J045335.2+011241 & 0.359919 & 0.41 & EW & matches\\
40440270 & 0.620192 & 0.415 & EB & J045403.3+010602 & 0.620186 & 0.46 & EW & matches\\
40441101 & 0.242292 & 0.656 & EW & J045355.9+015432 & 0.242292 & 0.19 & EW & matches\\
40451647 & 0.262418 & 0.628 & EW & J045435.6+011128 & 0.302132 & 0.46 & EW & "\\
40452311 & 1.025858 & 0.43 & EA & J045437.5-000921 & 1.02586 & 0.31 & EA & matches\\
40454051 & 0.372674 & 0.438 & EW & J045432.6-025904 & 0.372672 & 0.41 & EW & matches\\
40458997 & 0.287152 & 0.51 & EW & J045446.6+033853 & 0.287153 & 0.5 & EW & matches\\
40473866 & 0.326712 & 0.661 & EW & J045529.5+015803 & 0.326712 & 0.55 & EW & matches\\
40487622 & 0.393556 & 0.622 & EW & J045608.5+013815 & 0.393485 & 0.54 & EW & matches\\
40492182 & 0.267967 & 0.453 & EW & J045620.7+015109 & 0.30956 & 0.15 & EW & "\\
40494440 & 0.352848 & 0.288 & EW & J045626.9+033226 & 0.352848 & 0.24 & EW & matches\\
40494852 & 0.364382 & 0.447 & EW & J045637.5+001223 & 0.364386 & 0.42 & EW & matches\\
40497160 & 0.358476 & 0.468 & EW & J045634.5+013402 & 0.35778 & 0.35 & EW & matches\\
40507509 & 0.430038 & 0.212 & EW & J045712.3+011411 & 0.426231 & 0.24 & EW & matches\\
40509333 & 0.277006 & 0.795 & EW & J045707.8+023127 & 0.243166 & 0.7 & EW & "\\
40516110 & 0.274568 & 0.469 & EW & J045726.9+024553 & 0.483082 & 0.39 & EW & "\\
40516319 & 0.326007 & 0.481 & EW & J045727.5+015840 & 0.326003 & 0.33 & EW & matches\\
40517233 & 0.25372 & 0.52 & EW & J045730.1+043932 & 0.340296 & 0.43 & EW & "\\
40521875 & 1.436956 & 0.389 & EA & J045743.5-035130 & 0.495864 & 0.38 & EW & 1/3-day alias\\
40538170 & 1.793697 & 0.245 & EW & J045829.2+020215 & 0.896755 & 0.17 & RRab & k=2 harmonic\\
40539169 & 0.447356 & 0.318 & EW & J045832.0+051208 & 0.447127 & 0.32 & EW & matches\\
40543399 & 0.423866 & 1.088 & EB & J045843.9+020047 & 0.423868 & 0.39 & EB & matches\\
40544320 & 0.321777 & 0.35 & EW & J045856.0-000808 & 0.321778 & 0.23 & EW & matches\\
40546984 & 0.283726 & 0.601 & EW & J045903.5+001600 & 0.284272 & 0.54 & EW & matches\\
40556678 & 0.410605 & 0.35 & EW & J045921.4+035808 & 0.516686 & 0.15 & EW & "\\
40560950 & 0.346804 & 0.281 & EW & J045933.5+025058 & 0.295434 & 0.24 & EW & "\\
40562332 & 1.956163 & 0.368 & EA & J045937.4+014853 & 0.651652 & 0.29 & EW & 1-day alias\\
40566273 & 0.385832 & 0.528 & EW & J045948.5+021349 & 0.323292 & 0.46 & EW & "\\
40567663 & 0.333408 & 0.379 & EW & J045952.2+033344 & 0.333372 & 0.2 & EW & matches\\
50001918 & 0.395974 & 0.23 & EW & J050005.1+024402 & 0.395974 & 0.17 & EW & matches\\
50002096 & 0.257872 & 0.85 & EW & J050005.5+024537 & 0.25787 & 0.68 & EW & matches\\
50009152 & 0.412072 & 0.462 & EW & J050024.1+010318 & 0.412232 & 0.3 & EW & matches\\
50019583 & 0.546926 & 0.412 & EW & J050050.9+030108 & 0.546924 & 0.36 & EW & matches\\
50023449 & 0.257276 & 0.297 & EW & J050100.8+023025 & 0.257278 & 0.22 & EW & matches\\
50030975 & 0.245154 & 0.0 & EW & J050119.6+032036 & 0.279326 & 0.45 & EW & "\\
50034168 & 0.353474 & 0.452 & EW & J050126.9+011806 & 0.353476 & 0.34 & EW & matches\\
50051435 & 0.33245 & 0.375 & EW & J050209.7+013409 & 0.39896 & 0.34 & EW & "\\
50057618 & 0.394096 & 0.463 & EW & J050225.3+054531 & 0.490815 & 0.31 & EW & "\\
50061013 & 0.292902 & 0.291 & EW & J050234.2+034112 & 0.343162 & 0.12 & EW & "\\
50061732 & 1.263232 & 1.023 & EA & J050236.0-000110 & 1.26322 & 0.78 & EA & matches\\
50064487 & 0.555266 & 0.541 & EW & J050243.3+050412 & 0.555268 & 0.47 & EW & matches\\
50074895 & 0.23399 & 0.563 & EW & J050308.8+030206 & 0.23386 & 0.27 & EW & matches\\
50079404 & 0.544602 & 0.427 & EW & J050320.0+002106 & 0.2754827 & 0.35 & RRc & 1/2-day alias\\
50085280 & 0.347349 & 0.65 & EW & J050334.2+024133 & 0.347348 & 0.68 & EW & matches\\
50088742 & 0.517262 & 0.455 & EW & J050342.6+054028 & 0.340631 & 0.25 & EW & 1-day alias\\
50091440 & 0.317056 & 0.615 & EW & J050348.9+002849 & 0.317056 & 0.31 & EW & matches\\
50096181 & 0.291922 & 0.339 & EW & J050400.2+054738 & 0.291924 & 0.31 & EW & matches\\
50097045 & 0.265602 & 0.609 & EW & J050402.3+003952 & 0.264552 & 0.43 & EW & matches\\
50104299 & 0.920906 & 0.688 & EA & J050419.0+011844 & 1.84642 & 0.56 & EA & k=1/2 harmonic\\
50107075 & 0.730026 & 0.398 & EA & J050426.9+053403 & 0.693538 & 0.42 & EW & matches\\
50108832 & 0.296694 & 0.615 & EW & J050431.0+030600 & 0.296695 & 0.33 & EW & matches\\
50116858 & 0.259296 & 0.604 & EW & J050451.2+042506 & 0.259374 & 0.38 & EW & matches\\
50122594 & 0.229272 & 0.413 & EW & J050505.1+012042 & 0.45855 & 0.21 & EW & k=1/2 harmonic\\
50128282 & 0.453925 & 0.457 & EW & J050521.1+034844 & 0.36977 & 0.4 & EW & "\\
50130978 & 0.337271 & 0.384 & EW & J050526.9-015439 & 0.40591 & 0.37 & EW & "\\
50141196 & 0.45564 & 0.468 & EW & J050554.2+043249 & 0.370906 & 0.43 & EW & "\\
50167431 & 0.248298 & 0.0 & EW & J050703.1+025151 & 0.283422 & 0.23 & EW & "\\
50182919 & 0.74998 & 0.268 & EA & J050740.2+011247 & 0.738448 & 0.17 & EB & matches\\
50189044 & 0.259445 & 0.497 & EW & J050757.9+054344 & 0.298117 & 0.39 & EW & "\\
50207034 & 0.337941 & 0.356 & EW & J050840.9+011309 & 0.288978 & 0.21 & EW & "\\
50207297 & 0.203113 & 0.616 & EW & J050843.5+055158 & 0.254972 & 0.48 & EW & "\\
50208473 & 0.367198 & 0.64 & EW & J050846.2+022047 & 0.367196 & 0.46 & EW & matches\\
50216332 & 0.46696 & 0.642 & EA & J050905.4+055252 & 0.466962 & 0.6 & EA & matches\\
50217451 & 0.268538 & 0.759 & EW & J050908.0+014009 & 0.26854 & 0.47 & EW & matches\\
50251372 & 0.342414 & 0.36 & EW & J051025.1+035610 & 0.292242 & 0.28 & EW & "\\
50266894 & 0.571482 & 0.784 & EB & J051058.2+013447 & 0.571487 & 0.56 & EW & matches\\
50271843 & 0.366753 & 0.483 & EB & J051109.1+035924 & 0.366749 & 0.47 & EW & matches\\
50276127 & 0.274833 & 0.573 & EW & J051118.9+035850 & 0.274836 & 0.46 & EW & matches\\
50283698 & 0.290904 & 0.427 & EW & J051136.8-000710 & 0.340581 & 0.38 & EW & "\\
50283773 & 0.282898 & 0.476 & EW & J051135.9+054116 & 0.32966 & 0.37 & EW & "\\
50286491 & 0.57669 & 0.381 & EB & J051140.4+011553 & 0.576683 & 0.31 & EW & matches\\
50294747 & 0.401558 & 0.488 & EW & J051159.1+032052 & 0.401507 & 0.46 & EW & matches\\
50295394 & 0.274138 & 1.197 & EW & J051200.3+015736 & 0.24101 & 0.6 & EW & "\\
50310388 & 0.786698 & 0.286 & EW & J051233.8-001446 & 0.564157 & 0.29 & EW & 1/3-day alias\\
50311100 & 0.257459 & 0.218 & EW & J051234.3+033502 & 0.346892 & 0.16 & EW & "\\
50313800 & 0.267061 & 0.475 & EW & J051238.6-021345 & 0.308349 & 0.38 & EW & "\\
50319018 & 0.963765 & 0.379 & EA & J051252.0-024008 & 0.9637699 & 0.31 & EA & matches\\
50322296 & 0.303586 & 0.78 & EW & J051300.5-001540 & 0.303584 & 0.26 & EW & matches\\
50324694 & 2.318376 & 0.673 & EW & J051305.8-001127 & 0.5360932 & 0.24 & EW & 1/2-day alias\\
50334073 & 0.326127 & 0.57 & EW & J051326.6+000257 & 0.326128 & 0.31 & EW & matches\\
50335109 & 0.320764 & 0.427 & EW & J051327.7+034432 & 0.320766 & 0.29 & EW & matches\\
50336458 & 0.33454 & 0.424 & EW & J051330.8+004727 & 0.286488 & 0.26 & EW & "\\
50339740 & 0.383845 & 0.889 & EA & J051337.7+014933 & 0.383851 & 0.57 & EA & matches\\
50344583 & 0.331664 & 0.713 & EW & J051347.9+024311 & 0.331666 & 0.64 & EW & matches\\
50349482 & 0.549157 & 0.445 & EB & J051359.0+033945 & 0.548743 & 0.35 & EW & matches\\
50356379 & 0.438454 & 0.398 & EW & J051411.5+011910 & 0.35944 & 0.35 & EW & "\\
50369474 & 1.915366 & 0.497 & EA & J051442.1+034127 & 1.77044 & 0.66 & EA & "\\
50379385 & 0.261134 & 0.499 & EW & J051501.1-021950 & 0.230904 & 0.51 & EW & "\\
50386575 & 0.238217 & 0.334 & EW & J051518.9+035104 & 0.238218 & 0.22 & EW & matches\\
50390110 & 0.535344 & 0.662 & EW & J051526.4+035108 & 0.535342 & 0.38 & EW & matches\\
50392149 & 0.371255 & 0.244 & EW & J051528.3+011520 & 0.371254 & 0.15 & EW & matches\\
50392433 & 0.434406 & 0.35 & EB & J051531.4+035109 & 0.434402 & 0.29 & EW & matches\\
50421522 & 0.602654 & 0.428 & EW & J051634.1+025633 & 0.463244 & 0.28 & EA & "\\
50423084 & 0.291804 & 0.372 & EW & J051637.7+051542 & 0.291802 & 0.26 & EW & matches\\
50424009 & 0.561312 & 0.329 & EA & J051639.7+033423 & 0.561947 & 0.22 & EW & matches\\
50424100 & 0.623148 & 0.378 & EW & J051641.2-035634 & 0.9062765 & 0.24 & EW & "\\
50429839 & 0.2737 & 0.541 & EA & J051652.8+022250 & 0.754456 & 0.28 & EA & "\\
50430702 & 0.240358 & 0.907 & EW & J051654.6+002332 & 0.273292 & 0.85 & EW & "\\
50431451 & 0.23865 & 0.471 & EW & J051656.3+025141 & 0.313488 & 0.31 & EW & "\\
50431752 & 0.313392 & 0.345 & EW & J051656.9+040805 & 0.313388 & 0.24 & EW & matches\\
50433609 & 0.313152 & 0.598 & EW & J051701.0-031527 & 0.313152 & 0.6 & EW & matches\\
50434679 & 0.95828 & 0.388 & EA & J051703.5+051245 & 0.479142 & 0.36 & EA & 1-day alias\\
50435681 & 0.385722 & 0.497 & EW & J051705.7+021458 & 0.323069 & 0.38 & EW & "\\
50443729 & 0.453769 & 0.317 & EW & J051725.2+001339 & 0.36967 & 0.12 & EW & "\\
50444482 & 0.616332 & 0.502 & EW & J051725.7-025408 & 0.616329 & 0.44 & EW & matches\\
50449876 & 0.250438 & 0.747 & EW & J051734.9+011517 & 0.250434 & 0.54 & EW & matches\\
50457846 & 0.586132 & 0.568 & EB & J051755.9+021111 & 0.586135 & 0.51 & EW & matches\\
50467272 & 0.389988 & 0.576 & EW & J051816.9+053720 & 0.389814 & 0.38 & EW & matches\\
50472102 & 0.286322 & 0.619 & EW & J051827.7+023451 & 0.250382 & 0.36 & EW & "\\
50480134 & 0.310499 & 0.842 & EW & J051846.0+005011 & 0.310496 & 0.71 & EW & matches\\
50480790 & 0.622294 & 0.232 & EW & J051848.8+001221 & 0.474302 & 0.14 & EW & "\\
50481359 & 0.382985 & 0.285 & EW & J051848.8+033355 & 0.382633 & 0.35 & EW & matches\\
50484048 & 7.648866 & 0.499 & EW & J051854.9+014017 & 1.5819831 & 0.44 & EW & "\\
50486089 & 0.260532 & 0.62 & EW & J051859.7+051351 & 0.260534 & 0.36 & EW & matches\\
50487171 & 0.267714 & 0.3 & EW & J051902.0+030152 & 0.309222 & 0.19 & EW & "\\
50488408 & 0.699606 & 0.729 & EA & J051904.8+051015 & 0.699606 & 0.53 & EA & matches\\
50491106 & 0.27748 & 0.411 & EW & J051910.9+031945 & 0.322326 & 0.29 & EW & "\\
50493040 & 0.386542 & 0.0 & EW & J051915.1+025606 & 0.38648 & 0.17 & EW & matches\\
50493050 & 2.248062 & 0.277 & EW & J051915.1-025408 & 2.24802 & 0.21 & EW & matches\\
50498753 & 0.367363 & 0.539 & EW & J051929.1+001258 & 0.310216 & 0.41 & EW & "\\
50499158 & 0.25607 & 0.785 & EW & J051925.2-004142 & 0.29379 & 0.57 & EW & "\\
50500557 & 0.346462 & 0.549 & EW & J051931.9+024051 & 0.346464 & 0.44 & EW & matches\\
50505329 & 0.384864 & 0.611 & EW & J051942.4+002051 & 0.322615 & 0.59 & EW & "\\
50508506 & 2.766943 & 0.472 & EW & J051946.2-021535 & 7.1426 & 0.27 & EW & "\\
50510289 & 0.620334 & 0.304 & EW & J051953.5+031807 & 0.620326 & 0.26 & EW & matches\\
50517261 & 0.852987 & 0.883 & EA & J052008.8+024545 & 0.597462 & 0.54 & EA & "\\
50527821 & 0.331654 & 0.768 & EW & J052028.0-003202 & 0.331654 & 0.51 & EW & matches\\
50529660 & 0.17806 & 0.569 & EW & J052036.1+003205 & 0.327004 & 0.62 & EW & "\\
50543256 & 0.437992 & 0.703 & EW & J052105.6+033600 & 0.359126 & 0.63 & EW & "\\
50544388 & 0.284569 & 0.456 & EW & J052109.3+001326 & 0.284568 & 0.16 & EW & matches\\
50545221 & 0.381176 & 0.703 & EW & J052109.7+033815 & 0.381178 & 0.62 & EW & matches\\
50545498 & 3.138798 & 0.303 & EA & J052110.3+013800 & 1.5693684 & 0.24 & EA & 1-day alias\\
50546307 & 0.40051 & 0.457 & EW & J052112.1+035710 & 0.333534 & 0.23 & EW & "\\
50552687 & 0.356636 & 0.395 & EW & J052125.8-024606 & 0.356638 & 0.4 & EW & matches\\
50557720 & 0.313152 & 0.196 & EW & J052132.8+011008 & 0.270658 & 0.15 & EW & "\\
50563048 & 0.273228 & 0.608 & EW & J052148.6+022644 & 0.27323 & 0.3 & EW & matches\\
50563367 & 0.321374 & 0.507 & EW & J052149.2+031851 & 0.321376 & 0.25 & EW & matches\\
50564011 & 0.538886 & 0.503 & EW & J052150.7-032647 & 0.349842 & 0.42 & EW & 1-day alias\\
50566490 & 0.540496 & 0.521 & EW & J052152.0+012122 & 0.425262 & 0.17 & EW & "\\
50569288 & 1.351627 & 0.485 & EA & J052202.1+014915 & 1.35164 & 0.4 & EA & matches\\
50571325 & 0.379842 & 0.537 & EW & J052202.5-020046 & 0.37984 & 0.31 & EW & matches\\
50571898 & 10.786122 & 0.212 & EW & J052209.0-040950 & 5.39375 & 0.15 & RS Cvn & k=2 harmonic\\
50574471 & 0.984894 & 0.485 & EW & J052213.1-024311 & 0.659321 & 0.45 & EW & "\\
50579339 & 0.251444 & 0.843 & EW & J052219.6-003747 & 0.251446 & 0.8 & EW & matches\\
50599532 & 2.071471 & 0.363 & EW & J052305.9+013851 & 2.07152 & 0.17 & EW & matches\\
50600809 & 0.275578 & 0.23 & EW & J052308.5+015332 & 0.31976 & 0.14 & EW & "\\
50607615 & 0.348568 & 0.65 & EW & J052323.8-040845 & 0.348566 & 0.42 & EW & matches\\
50607820 & 0.576858 & 0.45 & EW & J052323.1+051724 & 0.447677 & 0.66 & EW & 1/4-day alias\\
50611629 & 2.480004 & 0.488 & EW & J052330.8+015118 & 1.2397549 & 0.25 & RS Cvn & k=2 harmonic\\
50615100 & 1.420845 & 0.669 & EA & J052334.0-015619 & 1.4208 & 0.59 & EA & matches\\
50617224 & 0.489996 & 0.338 & EW & J052342.3+030656 & 0.49 & 0.25 & EA & matches\\
50620504 & 0.504927 & 0.498 & EW & J052348.7+004808 & 0.402922 & 0.36 & EW & "\\
50638865 & 0.267213 & 0.441 & EW & J052424.7+023851 & 0.267214 & 0.32 & EW & matches\\
50641455 & 0.272109 & 0.697 & EW & J052425.7+012525 & 0.315096 & 0.66 & EW & "\\
50650756 & 0.97408 & 0.35 & EW & J052447.7+013628 & 0.974024 & 0.18 & EW & matches\\
50653408 & 0.388638 & 0.274 & EW & J052452.7+054434 & 0.388464 & 0.24 & EW & matches\\
50653608 & 0.247476 & 0.565 & EW & J052449.0-010157 & 0.247476 & 0.47 & EW & matches\\
50656194 & 0.487314 & 0.486 & EW & J052458.2+002536 & 0.391636 & 0.35 & EW & "\\
50658547 & 1.286026 & 0.343 & EW & J052503.0+050152 & 0.7818883 & 0.24 & EW & 1/2-day alias\\
50664317 & 0.281642 & 0.589 & EW & J052514.5+030539 & 0.281642 & 0.43 & EW & matches\\
50666065 & 0.220862 & 0.222 & EW & J052518.0+003819 & 0.248364 & 0.15 & EW & "\\
50674665 & 9.984332 & 0.908 & EW & J052535.1+014340 & 4.99396 & 0.14 & RS Cvn & k=2 harmonic\\
50676364 & 0.690322 & 1.516 & EW & J052539.7+000941 & 0.2565863 & 0.36 & RRc & 1/2-day alias\\
50691067 & 1.129948 & 0.257 & EW & J052607.6+055249 & 0.721269 & 0.21 & EW & "\\
50694000 & 0.305808 & 0.211 & EW & J052613.7-032846 & 0.26515 & 0.17 & EW & "\\
50698135 & 0.282626 & 0.502 & EW & J052621.7+051755 & 0.247548 & 0.33 & EW & "\\
50703622 & 0.280871 & 0.558 & EW & J052632.7+034935 & 0.280867 & 0.54 & EW & matches\\
50729302 & 0.273402 & 0.829 & EW & J052721.9+023524 & 0.273402 & 0.77 & EW & matches\\
50735395 & 0.34603 & 0.743 & EW & J052733.4-033724 & 0.346028 & 0.65 & EW & matches\\
50737943 & 3.084968 & 0.391 & EW & J052738.2+002304 & 2.82098 & 0.16 & RS Cvn & "\\
50747963 & 0.413978 & 0.249 & EW & J052752.3+010134 & 0.342823 & 0.19 & EW & "\\
50756757 & 0.39778 & 0.492 & EW & J052815.1-000451 & 0.331636 & 0.21 & EW & "\\
50758840 & 0.286996 & 0.395 & EW & J052817.9-023202 & 0.286996 & 0.3 & EW & matches\\
50762725 & 0.615163 & 0.679 & EA & J052825.3+023907 & 0.615162 & 0.49 & EW & matches\\
50763713 & 0.254044 & 0.0 & EW & J052827.2+030612 & 0.340882 & 0.52 & EW & "\\
50765935 & 1.26327 & 0.439 & EW & J052831.4+004819 & 0.3866938 & 0.21 & RRd & 1/2-day alias\\
50787252 & 4.371379 & 0.971 & EA & J052912.9+040057 & 1.84385 & 0.32 & EA & "\\
50788205 & 0.356702 & 0.333 & EW & J052909.7-012507 & 0.356704 & 0.25 & EW & matches\\
50793950 & 0.296002 & 0.326 & EW & J052926.6+050408 & 0.347586 & 0.3 & EW & "\\
50797908 & 0.344865 & 0.532 & EW & J052934.4+040435 & 0.344866 & 0.6 & EW & matches\\
50798370 & 0.898687 & 0.453 & EA & J052935.3+035729 & 1.79738 & 0.43 & EA & k=1/2 harmonic\\
50798398 & 0.277574 & 0.715 & EW & J052935.4+040651 & 0.243664 & 0.66 & EW & "\\
50801428 & 1.019254 & 0.349 & EA & J052941.6+033844 & 0.33609 & 0.3 & EA & 1/2-day alias\\
50818997 & 0.269308 & 0.337 & EW & J053017.2+034843 & 0.269306 & 0.21 & EW & matches\\
50820059 & 0.331189 & 0.353 & EW & J053019.4+024036 & 0.397128 & 0.38 & EW & "\\
50822867 & 0.60706 & 0.238 & EW & J053025.1-023032 & 0.4654165 & 0.28 & EW & "\\
50823983 & 0.484094 & 0.365 & EW & J053027.4+034246 & 0.319626 & 0.3 & RRc & 1-day alias\\
50824981 & 0.2446 & 0.379 & EW & J053029.4+034652 & 0.27879 & 0.29 & EW & "\\
50829485 & 0.354527 & 0.261 & EW & J053038.3+003637 & 0.301022 & 0.19 & EW & "\\
50847483 & 0.468221 & 0.0 & EW & J053108.8+005800 & 0.468232 & 0.3 & EW & matches\\
50848129 & 0.252325 & 0.0 & EW & J053117.3+000051 & 0.288868 & 0.69 & EW & "\\
50860953 & 1.233148 & 0.489 & EW & J053141.9+002925 & 0.3810179 & 0.38 & EW & 1/2-day alias\\
50863250 & 0.372698 & 0.271 & EW & J053146.6+004926 & 0.3727 & 0.23 & EW & matches\\
50876465 & 0.327801 & 0.736 & EW & J053207.7+010412 & 0.281532 & 0.69 & EW & "\\
50879736 & 0.227755 & 0.462 & EW & J053214.6+010739 & 0.227756 & 0.53 & EW & matches\\
50891971 & 0.355848 & 0.697 & EB & J053246.8+033822 & 0.301972 & 0.58 & EW & "\\
50904287 & 0.3454 & 0.242 & EW & J053312.5+032921 & 0.3454 & 0.22 & EW & matches\\
50912009 & 0.353496 & 0.653 & EW & J053328.6+051553 & 0.353495 & 0.54 & EW & matches\\
50917935 & 0.474314 & 0.348 & EW & J053341.0-031328 & 0.382984 & 0.31 & EW & "\\
50924899 & 0.55331 & 0.626 & EW & J053355.6+031021 & 0.433146 & 0.53 & EW & 1/4-day alias\\
50928290 & 0.39011 & 0.449 & EB & J053404.0+000234 & 0.390112 & 0.37 & EW & matches\\
50939657 & 0.257598 & 0.662 & EW & J053425.3+050522 & 0.2576 & 0.68 & EW & matches\\
50952250 & 0.24115 & 0.487 & EW & J053450.5+050005 & 0.319612 & 0.41 & EW & "\\
50957494 & 0.48729 & 0.727 & EW & J053500.8+053353 & 0.391608 & 0.67 & EW & "\\
50960726 & 0.333189 & 0.519 & EW & J053500.4+012330 & 0.333188 & 0.31 & EW & matches\\
50961355 & 0.299252 & 0.482 & EW & J053508.7+050532 & 0.352082 & 0.38 & EW & "\\
50978560 & 0.353664 & 0.531 & EW & J053542.6+040151 & 0.300392 & 0.38 & EW & "\\
50982055 & 0.317424 & 0.526 & EW & J053549.7+021911 & 0.317426 & 0.42 & EW & matches\\
51000045 & 1.66799 & 0.428 & EW & J053626.1-031355 & 5.089475 & 0.3 & RS Cvn & k=1/3 harmoninc\\
51010242 & 0.481214 & 0.832 & EA & J053646.6+024651 & 0.481676 & 0.33 & EW & matches\\
51015973 & 0.377194 & 0.646 & EW & J053658.0+035420 & 0.377196 & 0.53 & EW & matches\\
51017040 & 0.352766 & 0.618 & EW & J053652.6+012836 & 0.352768 & 0.4 & EW & matches\\
51019368 & 0.414812 & 0.47 & EW & J053704.9+004445 & 0.523737 & 0.36 & EW & "\\
51022720 & 2.28257 & 0.467 & EW & J053713.6-040100 & 7.90483 & 0.3 & RS Cvn & "\\
51026720 & 0.45626 & 0.362 & EW & J053719.9+054853 & 0.420527 & 0.53 & RRc & "\\
51037363 & 0.272899 & 0.654 & EB & J053741.6+022903 & 0.272898 & 0.48 & EW & matches\\
51044826 & 2.02277 & 0.788 & EA & J053756.5+050226 & 0.676342 & 0.77 & EA & 1-day alias\\
51062956 & 0.257494 & 0.941 & EW & J053834.2+000821 & 0.257494 & 0.58 & EW & matches\\
51072869 & 0.40529 & 0.555 & EW & J053852.6+053706 & 0.336837 & 0.62 & EW & "\\
51073077 & 0.542084 & 0.322 & EW & J053853.0+003650 & 0.744406 & 0.29 & EW & "\\
51077029 & 0.464762 & 0.321 & EW & J053901.2+003919 & 0.464764 & 0.24 & EW & matches\\
51082306 & 0.387926 & 0.449 & EW & J053913.2-002044 & 0.324764 & 0.3 & EW & "\\
51085303 & 0.304641 & 0.808 & EW & J053919.1-040055 & 0.264276 & 0.7 & EW & "\\
51090576 & 6.555936 & 0.546 & EA & J053927.7+005239 & 3.2635 & 0.41 & EA & k=2 harmonic\\
51102994 & 0.501248 & 0.709 & EW & J053953.3-032841 & 0.400582 & 0.57 & EW & "\\
51111613 & 0.281162 & 0.856 & EW & J054012.8-001009 & 0.281162 & 0.59 & EW & matches\\
51121235 & 0.26659 & 0.378 & EW & J054021.6+012809 & 0.26659 & 0.21 & EW & matches\\
51121900 & 0.306746 & 0.585 & EW & J054031.9-044321 & 0.362492 & 0.58 & EW & "\\
51125983 & 0.366139 & 0.372 & EW & J054040.5+003218 & 0.448448 & 0.24 & EW & "\\
51142474 & 0.299966 & 0.604 & EW & J054115.7+022720 & 0.299964 & 0.43 & EW & matches\\
51151082 & 0.285984 & 0.555 & EB & J054134.4+033739 & 0.286262 & 0.44 & EW & matches\\
51155526 & 0.81525 & 0.407 & EW & J054144.0+003141 & 0.4076207 & 0.29 & RRc & k=2 harmonic\\
51164830 & 3.769318 & 0.565 & EA & J054206.4-001304 & 3.76931 & 0.59 & EA & matches\\
51173465 & 0.266494 & 0.544 & EW & J054212.6+011216 & 0.266496 & 0.46 & EW & matches\\
51178734 & 0.392646 & 0.839 & EW & J054235.2-034650 & 0.323518 & 0.38 & RRc & "\\
51185766 & 21.61681 & 0.822 & EA & J054247.6+035228 & 1.26828 & 0.63 & EA & 1-day alias\\
51189789 & 0.268334 & 0.643 & EW & J054255.7+033657 & 0.268336 & 0.48 & EW & matches\\
51198026 & 0.315734 & 0.391 & EB & J054312.5+052010 & 0.315722 & 0.22 & EW & matches\\
51207122 & 0.542304 & 0.852 & EW & J054321.2+011529 & 0.542305 & 0.91 & EW & matches\\
51211698 & 11.179158 & 0.825 & EW & J054340.4-032439 & 2.4273672 & 0.82 & EA & "\\
51217112 & 0.294318 & 0.617 & EW & J054351.2+002843 & 0.34527 & 0.41 & EW & "\\
51219660 & 0.338542 & 0.778 & EW & J054356.8+005318 & 0.338538 & 0.61 & EW & matches\\
51231455 & 0.320532 & 1.381 & EW & J054421.1+034722 & 0.381912 & 0.38 & EW & "\\
51235641 & 0.333922 & 0.599 & EW & J054429.6+035556 & 0.401066 & 0.33 & EW & "\\
51240102 & 0.490676 & 0.377 & EW & J054428.2+010004 & 0.39379 & 0.36 & EW & "\\
51242452 & 0.552998 & 0.613 & EW & J054432.9+010612 & 0.432957 & 0.62 & EW & 1/4-day alias\\
51259955 & 0.438044 & 0.289 & EW & J054508.4+010555 & 0.43805 & 0.31 & EW & matches\\
51260907 & 0.303644 & 0.682 & EW & J054510.4+011958 & 0.303642 & 0.6 & EW & matches\\
51264421 & 0.368086 & 0.374 & EW & J054517.5+012542 & 0.368088 & 0.29 & EW & matches\\
51271397 & 0.379268 & 0.245 & EW & J054543.5+023826 & 0.379262 & 0.19 & EW & matches\\
51274299 & 0.369856 & 0.486 & EB & J054549.7+051129 & 0.370006 & 0.25 & EW & matches\\
51287703 & 0.69964 & 0.673 & EW & J054618.1+033833 & 0.517966 & 0.7 & EW & "\\
51292247 & 0.417989 & 0.584 & EW & J054627.7+035840 & 0.34557 & 0.3 & EW & "\\
51297128 & 0.457484 & 0.443 & EW & J054638.1+050919 & 0.37213 & 0.39 & EW & "\\
51310859 & 0.35111 & 0.371 & EW & J054707.7+051611 & 0.344522 & 0.39 & EW & matches\\
51340891 & 0.448878 & 0.255 & EW & J054810.6+051558 & 0.366758 & 0.26 & EW & "\\
51343222 & 0.38899 & 0.462 & EW & J054815.3+024018 & 0.325502 & 0.39 & EW & "\\
51345608 & 0.280259 & 0.617 & EW & J054822.0-035124 & 0.32608 & 0.38 & EW & "\\
51347369 & 0.522042 & 0.638 & EW & J054823.7+051022 & 0.413554 & 0.55 & EW & "\\
51353765 & 9.98573 & 0.496 & EW & J054836.0+040313 & 0.8312 & 0.37 & RS Cvn & 1-day alias\\
51382182 & 0.329656 & 0.684 & EW & J054918.9+010716 & 0.32965 & 0.37 & EW & matches\\
51395714 & 0.28988 & 0.509 & EW & J054956.6-001833 & 0.28988 & 0.42 & EW & matches\\
51397444 & 2.084334 & 0.243 & EA & J054946.6-011439 & 1.46213 & 0.38 & EA & "\\
51409696 & 0.26897 & 0.466 & EW & J055008.8-012637 & 0.310892 & 0.3 & EW & "\\
51433825 & 1.062205 & 0.23 & EW & J055105.0-024613 & 1.06216 & 0.19 & EW & matches\\
51467049 & 1.065844 & 0.753 & EW & J055207.0-032923 & 0.694652 & 0.78 & EW & "\\
51483475 & 0.478032 & 0.645 & EW & J055239.0-024801 & 0.478028 & 0.5 & EW & matches\\
51499114 & 0.788348 & 0.435 & EW & J055309.2-024406 & 0.565468 & 0.4 & EW & 1/3-day alias\\
51510025 & 0.567512 & 0.584 & EB & J055330.0-023634 & 0.567511 & 0.52 & EW & matches\\
51526365 & 0.992569 & 0.651 & EW & J055403.4-001428 & 0.248729 & 0.34 & RRc & 1/3-day alias\\
51556152 & 0.214918 & 0.443 & EW & J055459.1+050419 & 0.278696 & 0.44 & EW & "\\
51558377 & 0.324344 & 0.629 & EW & J055505.2-000332 & 0.324344 & 0.41 & EW & matches\\
51589474 & 0.475041 & 0.585 & EW & J055602.1+001336 & 0.311764 & 0.32 & RRc & 1-day alias\\
51635765 & 0.42778 & 0.488 & EW & J055721.4+051438 & 0.544926 & 0.48 & EW & "\\
51637836 & 0.458783 & 0.551 & EW & J055725.0+035749 & 0.297917 & 0.41 & RRc & 1-day alias\\
51671374 & 0.450319 & 0.876 & EB & J055817.9-024547 & 0.450313 & 0.86 & EW & matches\\
51677757 & 0.90373 & 0.609 & EW & J055827.8-024416 & 0.451862 & 0.46 & RRc & 1-day alias\\
51714505 & 0.274214 & 0.898 & EW & J055924.5+011708 & 0.274216 & 0.85 & EW & matches\\
51719466 & 0.333328 & 0.37 & EW & J055933.7+001105 & 0.333174 & 0.35 & EW & matches\\
60046150 & 0.43239 & 0.693 & EW & J060130.8-031357 & 0.3553579 & 0.61 & EW & "\\
60097703 & 0.378 & 0.345 & EW & J060304.6-035423 & 0.377998 & 0.29 & EW & matches\\
60158615 & 0.385186 & 0.545 & EW & J060451.0-030834 & 0.385186 & 0.56 & EW & matches\\
60202242 & 0.33341 & 0.754 & EW & J060604.7-032414 & 0.33341 & 0.6 & EW & matches\\
60224749 & 0.274627 & 0.323 & EW & J060641.8-025541 & 0.24139 & 0.19 & EW & "\\
60247571 & 0.388248 & 0.67 & EW & J060721.0-033857 & 0.324988 & 0.44 & EW & "\\
60248515 & 0.448148 & 0.473 & EW & J060722.6-041028 & 0.365924 & 0.47 & EW & "\\
60262701 & 0.437439 & 0.593 & EW & J060748.1-035945 & 0.3587577 & 0.56 & EW & "\\
80114061 & 1.29415 & 0.608 & EW & J080546.5-015845 & 0.7849164 & 0.47 & EW & 1/2-day alias\\
80129138 & 0.374384 & 0.606 & EW & J080634.4-011910 & 0.31522 & 0.45 & EW & "\\
80194618 & 0.35212 & 0.826 & EW & J081009.1-011839 & 0.26024 & 0.52 & EW & 1-day alias\\
80213291 & 0.378357 & 0.332 & EW & J081112.8-021540 & 0.3045739 & 0.21 & RS Cvn & "\\
80235224 & 0.361266 & 0.877 & EW & J081228.7-020205 & 0.305872 & 0.69 & EW & "\\
80248581 & 0.291322 & 0.635 & EW & J081316.2-023821 & 0.29132 & 0.39 & EW & matches\\
80281680 & 0.386854 & 0.502 & EW & J081514.3-020638 & 0.386852 & 0.38 & EW & matches\\
80309940 & 0.337382 & 0.0 & EW & J081659.5-030021 & 0.337384 & 0.43 & EW & matches\\
80312834 & 0.690166 & 0.506 & EW & J081710.1-003845 & 0.3450909 & 0.43 & RRc & k=2 harmonic\\
80324778 & 0.486676 & 0.58 & EW & J081754.7-032900 & 0.391216 & 0.3 & EW & "\\
80337842 & 0.277439 & 0.674 & EW & J081845.1-033514 & 0.24364 & 0.5 & EW & "\\
80342868 & 10.269871 & 0.519 & EA & J081904.8-023045 & 0.247198 & 0.54 & EW & 1/2-day alias\\
80365166 & 0.268745 & 0.463 & EW & J082032.1-041612 & 0.2687441 & 0.39 & EW & matches\\
80375784 & 0.356022 & 0.509 & EB & J082115.0-060145 & 0.356026 & 0.47 & EW & matches\\
80383570 & 0.341059 & 0.259 & EW & J082147.0-024908 & 0.4116368 & 0.21 & EW & "\\
80398835 & 0.334695 & 0.229 & EW & J082250.0-033707 & 0.286598 & 0.25 & EW & "\\
80404115 & 0.320793 & 0.296 & EW & J082312.5-040323 & 0.3207893 & 0.17 & EW & matches\\
80411627 & 0.238116 & 0.412 & EW & J082344.5-033705 & 0.270396 & 0.32 & EW & "\\
80414589 & 0.74089 & 0.314 & EW & J082356.7-022705 & 0.425092 & 0.27 & EW & 1-day alias\\
80416105 & 0.772012 & 0.656 & EW & J082403.3-025524 & 0.3860133 & 0.51 & RRc & k=2 harmonic\\
80428018 & 0.312214 & 0.59 & EW & J082452.6-013102 & 0.312212 & 0.41 & EW & matches\\
80432262 & 0.334734 & 0.587 & EW & J082510.8-023754 & 0.40224 & 0.36 & EW & "\\
80444806 & 0.345034 & 0.534 & EW & J082603.8-032056 & 0.345032 & 0.5 & EW & matches\\
80453363 & 0.216779 & 0.318 & EW & J082639.5-024824 & 0.383313 & 0.23 & EW & "\\
80462097 & 0.327154 & 0.485 & EB & J082716.3-001146 & 0.327008 & 0.46 & EW & matches\\
80475567 & 0.381754 & 0.361 & EW & J082815.2-032308 & 0.381762 & 0.31 & EW & matches\\
80482415 & 0.401779 & 0.662 & EW & J082845.4-025328 & 0.334414 & 0.61 & EW & "\\
80482473 & 0.314988 & 0.405 & EA & J082845.6-023748 & 0.37406 & 0.37 & EA & "\\
80494973 & 0.480576 & 0.502 & EW & J082941.8-015938 & 0.38726 & 0.3 & EW & "\\
80496178 & 0.247964 & 0.886 & EW & J082947.4-031642 & 0.247962 & 0.51 & EW & matches\\
80499392 & 0.349196 & 0.23 & EW & J083002.0-040144 & 0.297168 & 0.16 & EW & "\\
80510152 & 0.451642 & 0.617 & EW & J083051.6-033102 & 0.368264 & 0.52 & EW & "\\
80515127 & 0.299404 & 0.329 & EW & J083114.7-014937 & 0.352286 & 0.22 & EW & "\\
80526300 & 0.437159 & 0.673 & EW & J083205.9-041730 & 0.23324 & 0.54 & EW & 1/2-day alias\\
80529680 & 0.214279 & 0.41 & EW & J083222.0-025135 & 0.27292 & 0.39 & EW & "\\
80538135 & 0.272902 & 0.548 & EW & J083302.0-025055 & 0.24006 & 0.3 & EW & "\\
80549180 & 0.481372 & 0.454 & EW & J083354.2-041452 & 0.481694 & 0.27 & EW & matches\\
80550396 & 0.491809 & 0.569 & EW & J083359.9-023452 & 0.394526 & 0.41 & EW & "\\
80562200 & 0.317451 & 0.267 & EW & J083453.7-002133 & 0.317448 & 0.21 & EW & matches\\
80563334 & 0.263678 & 0.451 & EW & J083458.9-031109 & 0.303722 & 0.21 & EW & "\\
80566476 & 0.496674 & 0.684 & EB & J083513.9-020858 & 0.496666 & 0.37 & EA & matches\\
80579393 & 0.459967 & 0.294 & EW & J083617.3-025129 & 0.314782 & 0.2 & EW & 1-day alias\\
80592473 & 0.31662 & 0.271 & EW & J083723.3-020900 & 0.316622 & 0.23 & EW & matches\\
80598558 & 0.518211 & 0.449 & EW & J083754.2-040618 & 0.411344 & 0.22 & EW & "\\
80604817 & 0.308152 & 0.276 & EW & J083826.4-012544 & 0.445944 & 0.25 & EW & "\\
80611793 & 0.243099 & 0.277 & EW & J083903.0-020735 & 0.321452 & 0.17 & EW & "\\
80612587 & 1.779399 & 0.496 & EA & J083907.1-040753 & 0.389496 & 0.38 & EW & 1/2-day alias\\
80640655 & 0.33652 & 0.37 & EW & J084129.7-031320 & 0.336524 & 0.38 & EW & matches\\
80654234 & 0.399126 & 0.421 & EW & J084235.1-040202 & 0.332574 & 0.33 & EW & "\\
80655851 & 0.419218 & 0.512 & EW & J084243.6-035021 & 0.41923 & 0.24 & EW & matches\\
80660959 & 0.365484 & 0.554 & EW & J084308.7-033836 & 0.365488 & 0.49 & EW & matches\\
80671001 & 1.162372 & 0.26 & EW & J084402.5-025257 & 0.536783 & 0.28 & EW & 1-day alias\\
80672147 & 0.244423 & 0.887 & EW & J084408.6-040639 & 0.217736 & 0.5 & Hump & "\\
80673891 & 0.262254 & 0.25 & EW & J084418.5-021038 & 0.301952 & 0.17 & EW & "\\
80679069 & 0.23912 & 0.827 & EW & J084448.4-020737 & 0.27169 & 0.57 & EW & "\\
80683482 & 1.291147 & 1.377 & EW & J084513.9-001533 & 0.2813594 & 0.46 & RRc & 1/3-day alias\\
80705613 & 0.553944 & 0.456 & EW & J084720.1-030832 & 0.433544 & 0.37 & EW & 1/4-day alias\\
80714634 & 0.801264 & 0.562 & EW & J084812.3-033521 & 0.4006423 & 0.4 & RRc & k=2 harmonic\\
80727469 & 0.244034 & 0.661 & EW & J084927.5-012337 & 0.244036 & 0.58 & EW & matches\\
80745967 & 0.257186 & 0.523 & EB & J085121.8-005436 & 0.257188 & 0.39 & EW & matches\\
80756751 & 0.27496 & 0.622 & EW & J085231.1-020802 & 0.274964 & 0.49 & EW & matches\\
80760463 & 0.38263 & 0.392 & EW & J085255.0-025137 & 0.38263 & 0.3 & EW & matches\\
80764204 & 0.405834 & 0.284 & EW & J085318.8-014826 & 0.509142 & 0.15 & EW & "\\
80765662 & 0.342998 & 0.433 & EW & J085328.1-014747 & 0.343002 & 0.37 & EW & matches\\
80802886 & 0.486016 & 0.831 & EW & J085732.6-030938 & 0.391004 & 0.38 & EW & "\\
80815591 & 0.280978 & 0.521 & EW & J085857.1-005020 & 0.327052 & 0.44 & EW & "\\
\hline
\end{tabular}
\end{table*}

